The Fence Complexity of Persistent Sets

We study the psync complexity of concurrent sets in the non-volatile shared memory model. Flush instructions are used in non-volatile memory to force shared state to be written back to non-volatile memory and must typically be accompanied by the use of expensive fence instructions to enforce ordering among such flushes. Collectively we refer to a flush and a fence as a psync. The safety property of strict linearizability forces crashed operations to take effect before the crash or not take effect at all; the weaker property of durable linearizability enforces this requirement only for operations that have completed prior to the crash event. We consider lock-free implementations of list-based sets and prove two lower bounds. We prove that for any durable linearizable lock-free set there must exist an execution where some process must perform at least one redundant psync as part of an update operation. We introduce an extension to strict linearizability specialized for persistent sets that we call strict limited effect (SLE) linearizability. SLE linearizability explicitly ensures that operations do not take effect after a crash which better reflects the original intentions of strict linearizability. We show that it is impossible to implement SLE linearizable lock-free sets in which read-only (or search) operations do not flush or fence. We undertake an empirical study of persistent sets that examines various algorithmic design techniques and the impact of flush instructions in practice. We present concurrent set algorithms that provide matching upper bounds and rigorously evaluate them against existing persistent sets to expose the impact of algorithmic design and safety properties on psync complexity in practice as well as the cost of recovering the data structure following a system crash.

==> unused/lb1.tex <==
\section{Redundant psync lower bound for durable linearizable sets}
\label{section:lb2}

After modifying a base object only a single psync is required to ensure that it is written to persistent memory. 
Performing multiple psyncs on the same base object is therefore unnecessary and wasteful.
We refer to these unnecessary psyncs as \textit{redundant} psyncs.
We show that for any durably linearizable lock-free set there must exist an execution in which $n$ concurrent processes are invoking $n$ concurrent update operations and $n$-1 processes each perform at least one redundant psync.
At first glance one may think that this result is implied by the lower bound of Cohen et al. \cite{cohen2018inherent}.
Cohen et al. show that for any lock-free durable linearizable object, there exists an execution wherein every update operation performs at least one persistence fence.
Cohen et al. make no claims regarding redundant psyncs. 
Our result demonstrates that durable linearizable lock-free objects cannot completely avoid redundant psyncs. 
\Cref{fig:lb2-executions} shows an example of an execution in which all but one process performs a redundant psync.
This execution is described in more detail in the proof sketch of \cref{theorem:redundant-psync}.

\begin{figure}[!t]
\begin{center}
    \includegraphics[width=0.6\linewidth]{diagrams/exec2.pdf}
\caption{An example of the execution described in \cref{theorem:redundant-psync}.
Operations $\pi_2-\pi_{n-1}$ rely on the durability of $\pi_1$ forcing.
Since none of these processes can know if the CPE of $\pi_1$ has occurred they are forced to perform a psync resulting each performing a redundant psync.} 
\label{fig:lb2-executions}
\end{center}
\end{figure}

\begin{definition}[Persistence Event]
Let $E$ be an execution of a durable linearizable set, we call any background flush, explicit flush or persistence fence a \textit{persistence event} in $E$. 
\end{definition}

\begin{definition}[Crash-Recovery Extension]
Consider an execution $E$ of a durable linearizable set.
Let $\bot$ denote a system crash event.
Let $E'$ be $E \cdot \bot \cdot E_R$ where $E_R$ is the sequential execution of the recovery procedure.
We refer to $E'$ as a \textbf{crash-recovery extension} of $E$.
\end{definition}

For a successful update operation $\pi$, we can identify a \textit{critical persistence event}~$e$.
Intuitively, if a crash event happens \textit{before} $e$, then the update $\pi$ will \textit{not be recovered}.
This means if we perform an identical update after recovery, it will \textit{succeed}.
On the other hand, if a crash happens \textit{after} $e$, then $\pi$ \textit{will be recovered}.
So, if we perform an identical update after recovery, it will \textit{fail}.

\begin{definition}[Critical Persistence Event (CPE)]
Consider an execution $E$ of a durable linearizable set and a pending operation $\pi$ in $E$ invoked by process $p$.
Let $r$ be the response of $\pi$ in a solo extension of $E$ wherein $p$ completes $\pi$ and no crash events occur.
Let $E'$ be the crash-recovery extension of $E$.
Consider a solo extension of $E'$ wherein $p$ invokes and completes a new operation $\pi'$ with the same arguments as $\pi$.
Let $r'$ be the response of $\pi'$.
For successful update operations, the persistence event $f$ in $E$ is the \textit{critical persistence event}, of $\pi$ if immediately before applying $f$, we have $r = r' = \texttt{true}$ and immediately after applying $f$ we have $r = \texttt{true}$ and $r' = \texttt{false}$.
\end{definition}

A CPE is defined for a successful update operation, and it represents the first point at which $\pi$ could, but is not guaranteed to, change the response of a different operation $\pi'$ where $\pi'$ is invoked after crashing and recovering. 
Crucially, $\pi$ and $\pi'$ are different operations, and $\pi'$ is the operation that completes in a solo extension after the crash. 
Note that immediately after recovering from a crash $\pi'$ has not yet started, so we cannot (and do not need to) argue that all extensions return the same response value.

Since the CPE is defined for successful update operations, if the CPE exists for an update $\pi$ in some execution $E$, then the CPE of $\pi$ exists at some point between when $\pi$ is decided and the response of $\pi$ (or a crash event). 
% The CPE of an update operation cannot be an explicit flush on a base object $b$ since an explicit flush requires a persistence fence to guarantee that that $b$ is written to persistent memory. 
% This means the CPE of an operation is either a background flush or a persistence fence. 
Recall that since explicit flushes are non-blocking, an explicit flush on a base object $b$ requires a persistence fence to guarantee that that $b$ is written to persistent memory.
It is possible that $b$ is written to persistent memory after an explicit flush on $b$ but prior any persistence fences.
In such a scenario the CPE of the operation can be the explicit flush on $b$.
% If $b$ is written to persistent memory after a persistence fence which followed an explicit flush on $b$ then the CPE of the operation is the persistence fence. 
If the CPE $\pi$ is a persistence fence by process $p$, then $p$ must have previously performed an explicit flush in $\pi$. 
We say that the base object $b$ is \textit{involved in the CPE} of $\pi$ if the CPE is a background flush or explicit flush on $b$ or if the CPE is a persistence fence where the corresponding explicit flush is on $b$.
% Unsuccessful update operations and read-only operations can be thought of as having a CPE.
% The CPE of an unsuccessful update operation or read-only operation corresponds to the CPE of some successful update operation.
% The corresponding CPE for an unsuccessful update operation or read-only operation can be prior to the invocation of the operation (this is easiest to see in the sequential case).

Our CPE definition is similar to the \textit{Persist Point} defined by Izraelevitz et al. \cite{izraelevitz2016linearizability} or the \textit{Durability Point} defined by Friedman et al \cite{QueueFriedman18}.
The \textit{Persist Point} of an operation is a point after the linearization point of the operation.
We have already mentioned two examples of implementations where the linearization point is after the point when the operation is persisted \cite{zuriel2019efficient,cohen2018inherent}.
The definition of a \textit{Durability Point} is not defined in terms of sets and lacks some necessary details which our definition of the CPE clarifies. 



\begin{definition}[Destructive Write]
A write to the base object $b$ is \textit{destructive} if it changes the value of $b$.
\end{definition}

\begin{definition}[Redundant-psync]
Consider an execution $E$ of a durable linearizable set. 
An explicit flush $f$ applied to the base object $b$, is redundant if $b$ was previously flushed by another explicit flush $f'$, and there does not exist a destructive write to $b$ between $f'$ and $f$ in $E$.
A persistence fence $f_p$ is redundant if there exists another persistence fence $f_p'$ prior to $f_p$ and there does not exist any non-redundant flush between $f_p'$ and $f_p$ in $E$.  
A psync which is a flush and a persistence fence, is redundant if the persistence fence redundant.
\end{definition}

\begin{theorem}
In an $n$-process system, for every durable linearizable lock-free set implementation $I$, there exists an execution of $I$ wherein $n$ processes are concurrently performing update operations and $n$-1 processes perform a redundant psync. 
\label{theorem:redundant-psync}
\end{theorem}

A proof of \Cref{theorem:redundant-psync} is included in the full version of the paper.

==> unused/lb2.tex <==
\section{SLE linearizable sets and persistence-free reads impossibility}
\label{section:lb1}

% \subsection{Strict limited effect linearizability}
% 
The key goal in Aguilera and Frølund was to enforce \textit{limited effect} by requiring operations to take effect before the crash or not at all. 
This is evident from the first paragraph of the abstract: "In such systems, an operation that crashes should either not happen or happen within some limited time frame—preferably before the process crashes. We define strict linearizability to achieve this semantics." 
The importance of limited effect is further emphasized in their own motivating example: “suppose that a military officer presses a button to launch a missile during war, but the missile does not come out. It might be catastrophic if the missile is suddenly launched years later after the war is over” \cite{AF03}. 
If the system can launch the missile during the execution of the recovery procedure (potentially many years later, when old systems are booted back up), this clearly contradicts the intentions of Aguilera and Frølund, however, in the full system crash-recovery model, strict linearizability admits this possibility.

% Aguilera and Frølund defined strict linearizability with the goal of enforcing \textit{limited effect} which requires that an operation takes effect within a limited amount of time after it is invoked.
Limited effect requires that an operation takes effect within a limited amount of time after it is invoked.
The point at which an operation takes effect is typically referred to as its \textit{linearization point} and we say that the operation \textit{linearizes} at that point.
Rephrasing the intuition, when crashes can occur, limited effect requires that operations that were pending at the time of a crash linearize prior to the crash or not at all.

\myparagraph{Strict linearizability does not satisfy limited effect in the full system crash-recovery model}
Strict linearizability is defined in terms of histories, which abstract away the real-time order of events.
As a result, strict linearizability does not allow one to argue anything about the ordering of linearization points of operations that were pending at the time of a crash relative to the crash event.
Thus, strict linearizability cannot and does not prevent operations from taking effect during the recovery procedure or even after the recovery procedure (which can occur for example in implementations that utilize linearization helping).
Strict linearizability only requires that at the time of a crash, pending operations \textit{appear} to take effect prior to the crash.
Although we are not aware of a formal proof of this, we conjecture in the full system crash-recovery model, durable linearizable objects are strict linearizable for some suitable definition of the recovery procedure.
This is because we can always have the recovery procedure \textit{clean-up} the state of the object returning it to a state such that the resulting history of any possible extension will satisfy strict linearizability.
We note this conjecture as further motivation towards re-examining the way in which the definition of strict linearizability has been adapted for the full system crash-recovery model.
The results in this paper do not rely on a proof of the conjecture.

\myparagraph{Limited effect matters}
It may be more accurate to say that strict linearizability enforces \textit{apparent limited effect}.
When the system can recover following a crash it is crucial that we distinguish between (1) requiring operations to actually \textit{take effect} before the crash and (2) requiring that operations simply \textit{appear to} take effect before the crash.
%This matters precisely because there is a difference between launching a missile years after 
% If this distinction were unimportant, then we should be satisfied with a recovery procedure launching a missile years after a conflict is over, as long as the operation that launches the missile is \textit{linearized} during the conflict. 

\myparagraph{Defining limited effect for sets}
%
In general arguing about an explicit point at which an operation takes effect is difficult. 
However, we are specifically interested in sets.
Update operations of a set are strongly non-commutative which is a useful property if we care about identifying an explicit point at which an update operation takes effect \cite{attiya2011laws}. 
% An operation $\pi_1$ is strongly non-commutative if there exists a configuration from which $\pi_1$ executed sequentially by process $p_1$ can alter the response of another operation $\pi_2$ executed sequentially by a different process $p_2$ \cite{attiya2011laws}.

In order to argue about the point at which an operation actually takes effect we need to identify specific event(s) at which operations can take effect.  
In our computational model, writes (or successful RMWs) are the only events with observable side effects since writes are the only events that change the states of shared objects.
Thus, for any implementation of a set, we argue that the linearization point of a successful update operation must be a write.
Specifically, the linearization point of a successful update operation is a \textit{key write} which we define as follows:
consider an execution $E$ of a durable linearizable set, ending with the write event $w$, on some base object $b$, as part of the successful update operation $\pi$, invoked by process $p$.
Let $E'$ be the prefix of $E$ ending just before $w$.
Consider a solo extension $EE$ of $E$ wherein some process $p'$ invokes and completes the operation $\pi'$ where $\pi'$ does not commute with $\pi$ and $\pi'$ is linearization help-free.
Similarly, consider the solo extension $EE'$ of $E'$ wherein process $p'$ invokes and completes the same operation $\pi'$ as previously defined.
The write event $w$ is the key write of $\pi$ iff the extensions $EE$ and $EE'$ exist and $\pi'$ has a different response in $EE$ and $EE'$. 
% 
% The write $w$ is the key write of $\pi$ iff there exists solo extensions $EE$ of $E$ and $EE'$ of $E'$ where in both $EE$ and $EE'$ process $p'$ invokes and completes the operation $\pi'$ where $\pi'$ does not commute with $\pi$ and $\pi'$ is linearization help-free and $\pi'$ has a different response in $EE$ and $EE'$. 

Intuitively, the key write is the event after which the operation can affect the response of some subsequent non-commutative, linearization help-free operation.
It is perhaps easier to imagine how a key write would exist for stacks or queues in which update operations typically contend on a single object (a top or head pointer) where it is clear that performing a write on that object will affect other operations. 

\myparagraph{Defining SLE linearizability}
We want to reason about when a key write occurs relative to a crash event. 
To do so we must lift the key write into histories. 
We utilize the concept of a key write to capture the intentions of Aguilera and Frølund in the context of sets by defining \textit{Strict limited effect} (SLE) linearizability for sets as follows:
an implementation $I$ of a set satisfies SLE linearizability iff all possible histories produced by $I$ satisfy SLE linearizability.
A history satisfies SLE linearizability iff the history satisfies strict linearizability and for all operations with a key write, if the operation is pending at the time of a crash, the key write of the operation must occur before the crash event.
In the strict completion of a history this is equivalent to requiring that the key write is always between the invocation and response of the operation. 
This is because the order of key writes relative to a crash event is fixed which means if the write occurs after the crash event then a strict completion of the history could insert a response for the operation only prior to the key write (at the crash) and this response cannot be reordered after the key write.
In this work we do not attempt to generalize SLE linearizability to other abstract types;
However, we note that it would not be difficult to generalize SLE linearizability for any type where we can define the concept of a key write for update operations.
For instance, \emph{stacks} and \emph{queues} are types where defining a key write is likely to be straightforward. 

We have already discussed some hand-crafted persistent sets which satisfy SLE linearizability.
In particular, the link-and-persist list of David et al. and the link-free list of Zuriel et al. both satisfy SLE linearizable.
% because these implementations ensure that the key write of any update operation always precedes the CPE of the operation. 

\myparagraph{Comparing with other correctness conditions}
%
SLE linearizability allows one to argue about the order of linearization points relative to crashes for sets.
SLE linearizability is stronger than durable linearizability and successfully captures the intuition that motivated strict linearizability.
One might say that SLE linearizability is similar to \textit{detectable executions} defined by Friedman et al. \cite{QueueFriedman18} in that ensuring SLE linearizability will often require identifying operations that were pending at the time of a crash in order to revert any effects of those pending operations whose key write did not occur prior to the crash. 
If the implementation is capable of identifying operations that were pending at the time of a crash then it provides detectable execution. 

\subsection{SLE Linearizable sets and persistence-free reads impossibility result}

We show that it is impossible to implement a SLE linearizable lock-free set for which read-only searches do no perform any explicit flushes or persistence fences. 
This result primarily follows from the fact that some operations will rely on the durability of other operations but persistence events have no visible side effects meaning from the perspective of a persistence-free search, a configuration in which the CPE of a particular operation has occur is not distinguishable from another configuration in which the CPE of said operation has occurred.
An example is depicted in \Cref{fig:lb1-executions}.

\begin{figure}[!t]
\begin{center}
    \includegraphics[width=0.6\linewidth]{diagrams/exec-pf-search-3.pdf}
\caption{A simplified example of the execution described in \cref{theorem:persistence-free-search-impossiblity}. 
Processes $p_2$ and $p_3$ cannot distinguish between configurations resulting after the last step of $p_1$ or $p_2$. 
$p_3$ and $p_4$ have no way to determine if the CPE of $\pi_1$ and $\pi_2$, respectively, have occurred.
$\pi_3$ and $\pi_4$ must return a specific value since an identical operation invoked after the crash has a fixed response but this response is not know a priori.}
\label{fig:lb1-executions}
\end{center}
\end{figure}

\begin{definition}[Persistence-Free Searches]
We say that a set offers persistence free searches if there is no execution of the set in which a process that invoked a read-only operation $\pi$ performs an explicit flush or persistence fence between the invocation and response of $\pi$. 
\end{definition}

\begin{definition}[Persistence Help-Freedom]
An execution of a set is persistence help-free if the following conditions hold.
If process $p$ performs an explicit flush on base object $b$ in an operation $\pi$, then $p$ must have previously written to $b$ in $\pi$. 
If $p$ performs a persistence fence in an operation $\pi$, then $p$ must have previously performed an explicit flush on some base object in $\pi$.
A set is persistence-help-free if all executions of the set are persistence-help-free.
\end{definition}

\begin{lemma}
A SLE linearizable lock-free set with read-only searches cannot linearize successful update operations after the CPE of the update.
\label{lemma:sle-lin-constraint}
\end{lemma}

\begin{theorem}
There exists no SLE linearizable lock-free set with persistence-free read-only searches.
\label{theorem:persistence-free-search-impossiblity}
\end{theorem}

A proof of \Cref{lemma:sle-lin-constraint} and \Cref{theorem:persistence-free-search-impossiblity} is included in the full version of the paper.

==> unused/refs-old.tex <==
@string{epfl             = "Ecole Polytechnique F\'ed\'erale de Lausanne"}
@string{cornell		= "Cornell University"}
@string{cornellcs	= "Department of Computer Science, 
                                  Cornell University"}
@string{gitics		= "School of Information and Computer Science,
				Georgia Institute of Technology"}
@string{ibmrl		= "IBM Research Laboratory"}
@string{mitlcs          = "Laboratory for Computer Science,
                  Massachusetts Institute of Technology"}
@string{mst             = "Mathematical Systems Theory"}
@string{gatech          = "College of Computing, Georgia Institute of Technology"}
@string{yalecs		= "Department of Computer Science, Yale University"}
%--------------------------------------------------------
@string{dc		= "Distributed Computing"}
@string{ic		= "Information and Computation"}
@string{surveys         = "ACM Computing Surveys"}
@string{lncs		= "LNCS"}
@string{springer	= "Springer-Verlag"}
%-------------------------------------------------------
@string{icalp		= "International Conference on Automata, Languages,
				and Programming"}
@string{focs		= "Symp. on Foundations of Computer Science"}
@string{ftcs		= "International Symp. on Fault-Tolerant Computing"}
@string{podc		= "ACM Symp. on Principles
				of Distributed Computing"}
@string{pods		= "Symp. on Principles of Database Systems"}
@string{proc		= "Proceedings of the"}
@string{stoc		= "ACM Symp. on Theory of Computing"}
@string{wdag		= "International Workshop on Distributed Algorithms"}
@string{disc		= "International Symp. on Distributed Computing"}
@string{icdcs		= "International   Conference on Distributed Computing Systems"}  
@string{srds            =" Symp. on Reliable Distributed Systems"}

%--------------------------


@string{inst-ibp	       = "Institut Blaise Pascal"}
@string{inst-litp	       = "LITP, " # inst-ibp}
@string{inst-masi	       = "MASI, " # inst-ibp}
@string{inst-igm	       = "Institut Gaspard Monge, Univer\-sit{\'e} de Marne-la-Vall{\'e}e"}
@string{inst-univp6	       = "Univer\-sit{\'e} Paris VI (France)"}
@string{inst-univp7	       = "Univer\-sit{\'e} Paris 7-Denis Diderot (France)"}
@string{inst-univp11	       = "Univer\-sit{\'e} Paris-Sud (France)"}
@string{inst-univp12	       = "Univer\-sit{\'e} Paris XII (France)"}
@string{inst-univbdx	       = "Univer\-sit{\'e} Bordeaux I (France)"}
@string{inst-UPxiLITP	       = "Univer\-sit{\'e} Paris-Sud et LITP (France)"}
@string{inst-univporto	       = "Universidade do Porto (Portugal)"}

@string{ibp	       = "Institut Blaise Pascal"}
@string{litp	       = "LITP, " # ibp}
@string{liafa	       = "LIAFA, "# inst-univp7} 
@string{masi	       = "MASI, " # ibp}
@string{igm	       = "Institut Gaspard Monge, Universit{\'e} de Marne-la-Vall{\'e}e"}
@string{univp6	       = "Univer\-sit{\'e} Paris VI (France)"}
@string{univp7	       = "Univer\-sit{\'e} Paris VII (France)"}
@string{univp11	       = "Univer\-sit{\'e} Paris-Sud (France)"}
@string{univp12	       = "Univer\-sit{\'e} Paris XII (France)"}
@string{univbdx	       = "Univer\-sit{\'e} Bordeaux I (France)"}
@string{UPxiLITP	       = "Univer\-sit{\'e} Paris-Sud et LITP (France)"}
@string{univporto	       = "Universidade do Porto (Portugal)"}
@string{polytechnique  = "{\'E}cole Polytechnique"}
				   ########
				   # TYPE #
				   ########


@string{tr		       = "Rapport de recherche"}
@string{trlitp		       = "Rapport {LITP}"}
@string{trliafa		       = "Rapport {LIAFA}"}
@string{trlix		       = "Rapport {LIX}"}
@string{trlri		       = "Rapport {LRI}"}
@string{trlabri		       = "Rapport {LaBRI}"}
@string{memo		       = "Research Memo"}


				   ########
				   # NOTE #
				   ########


@string{rlitp		       = "Rapport {LITP} n\No "}	# utilisation : rlitp # "92-31"
@string{rliafa		       = "Rapport {LIAFA} n\No "}	# utilisation : rlitp # "92-31"
@string{rmasi		       = "Rapport {MASI} n\No "}	# idem
@string{thlitp		       = "Rapport {LITP-TH} n\No "}	# idem
@string{prepa		       = "En pr{\'e}paration"}
@string{soumis		       = "Soumis"}
@string{soumisa		       = "Soumis {\`a} "}		# utilisation : soumisa # tcs
@string{ap		       = "{\`A} para{\^\i}tre"}
@string{apd		       = "{\`A} para{\^\i}tre dans "}	# idem
@string{invite		       = "Conf{\'e}rence invit{\'e}e"}
@string{invite+tutorial	       = "Conf{\'e}rence invit{\'e}e associ{\'e}e {\`a} un tutorial"}
@string{position-paper	       = "Position paper"}
@string{extended-abstract      = "Extended abstract"}
@string{available	       = "{\'E}galement disponible comme "}
@string{eng-translat-in	       = "Traduction anglaise dans "}
@string{in-french	       = "En fran{\c c}ais"}
@string{in-english	       = "En anglais"}
@string{in-japanese	       = "En japonais"}			# idem
@string{et		       = " et "}			# utilisation : ... # et # ...
@string{stop		       = ". "}				# pour separer deux notes


				   #########
				   # MONTH #
				   #########


@string{spring		       = "Printemps"}
@string{summer		       = "Et{\'e}"}
@string{fall		       = "Automne"}
@string{winter		       = "Hiver"}


@string{fev		       = feb}
@string{avr		       = apr}
@string{mai		       = may}

				  ###########
				  # PUBTYPE #
				  ###########

@string{numero_special	       = "Num{\'e}ro sp{\'e}cial"}
@string{art_avec_comite	       = "Article avec comit{\'e}"}
@string{art_sans_comite	       = "Article sans comit{\'e}"}
@string{coll_avec_comite       = "Colloque avec comit{\'e}"}
@string{coll_sans_comite       = "Colloque sans comit{\'e}"}
@string{seminaire	       = "S{\'e}minaire"}
@string{expose		       = "Expos{\'e}"}
@string{dea		       = "M{\'e}moire de {DEA}"}
@string{these		       = "Th{\`e}se de Doctorat"}
@string{these3		       = "Th{\`e}se de 3e cycle"}
@string{these_etat	       = "Th{\`e}se d'{\'E}tat"}
@string{habilitation	       = "Habilitation {\`a} diriger des recherches"}
@string{livre		       = "Livre"}
@string{edition		       = "{\'E}dition"}
@string{chapitre	       = "Chapitre"}
@string{rapport		       = "Rapport de recherche"}
@string{logiciel	       = "Logiciel"}
@string{autre		       = "Autre"}
@string{unpublished	       = "Non publi{\'e}"}
@string{see-also	       = "Voir aussi "}
@string{?		       = "???"}

@string{invited		       = invite}
@string{toappear	       = ap}
@string{research-memo	       = memo}
@string{research-report	       = tr}
@string{invited-assoc-tutorial = invite+tutorial}


				 #############
				 # PREAMBULE #
				 #############

@preamble{ "\def\noopsort#1{} "
	#  "\def\No{\kern-.25em\lower.2ex\hbox{\char'27}} "
	#  "\def\no#1{\relax} "
	#  "\def\http#1{{\\{\small\tt http://www-litp.ibp.fr:80/{$\sim$}#1}}}"
	}


%----------------------------------------------------------------------------
%A

@article{lamport-interprocess,
  author    = {Leslie Lamport},
  title     = {On Interprocess Communication. Part I: Basic Formalism},
  journal   = {Distributed Computing},
  volume    = {1},
  number    = {2},
  year      = {1986},
  pages     = {77-85},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{ABD95,
Author={Hagit Attiya and Amotz Bar-Noy and Danny Dolev},
Title={Sharing Memory Robustly in Message Passing Systems.},
Journal=jacm,
month=jan,
Year=1995,
Volume=42,
number=2,
pages="124-142",
}
@article{HS99,
 Author = {Maurice Herlihy and Nir Shavit},
 Title = {The topological structure of asynchronous computability},
 Journal = jacm,
 Volume = 46,
 number = 2,
 Year = 1999,
 pages = "858--923",
 }

@book{HS08-book,
  author    = {Maurice Herlihy and
               Nir Shavit},
  title     = {The art of multiprocessor programming},
  publisher = {Morgan Kaufmann},
  year      = {2008},
  isbn      = {978-0-12-370591-4},
  pages     = {I-XX, 1-508},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{Chaud93,
 Author = {Soma Chaudhuri},
 Title = {More choices allow more faults: Set consensus problems in totally asynchronous systems},
 Journal = ic,
 Volume = 105,
 number = 1,
 Year = 1993,
 pages = "132--158",
 }
 
@inproceedings{brown2020non,
  title={Non-blocking interpolation search trees with doubly-logarithmic running time},
  author={Brown, Trevor and Prokopec, Aleksandar and Alistarh, Dan},
  booktitle={Proceedings of the 25th ACM SIGPLAN Symp. on Principles and Practice of Parallel Programming},
  pages={276--291},
  year={2020}
}

@inproceedings{pelley2014memory,
  title={Memory persistency},
  author={Pelley, Steven and Chen, Peter M and Wenisch, Thomas F},
  booktitle={2014 ACM/IEEE 41st International Symp. on Computer Architecture (ISCA)},
  pages={265--276},
  year={2014},
  organization={IEEE}
}

@inproceedings{condit2009better,
  title={Better I/O through byte-addressable, persistent memory},
  author={Condit, Jeremy and Nightingale, Edmund B and Frost, Christopher and Ipek, Engin and Lee, Benjamin and Burger, Doug and Coetzee, Derrick},
  booktitle={Proceedings of the ACM SIGOPS 22nd Symp. on Operating systems principles},
  pages={133--146},
  year={2009}
}

@Article{Karp-NP,
  author = 	 {Richard M. Karp},
  title = 	 {Reducibility Among Combinatorial Problems},
  journal = 	 {Complexity of Computer Computations},
  year = 	 {1972},
  pages = 	 {85-103}
}

@inproceedings{ATD99,


 booktitle    = proc # " 13th International Symp. on Distributed Computing",

   author    = {Marcos Kawazoe Aguilera and
               Sam Toueg and
               Borislav Deianov},
  title     = {Revising the Weakest Failure Detector for Uniform Reliable
               Broadcast},
  series = {LNCS 1693},
  year     = {1999},
  pages     = {19-33},
 
}

@inproceedings{golab-strong,
  author    = {Wojciech M. Golab and
               Lisa Higham and
               Philipp Woelfel},
  title     = {Linearizable implementations do not suffice for randomized distributed
               computation},
  booktitle = {Proceedings of the 43rd {ACM} Symp. on Theory of Computing, {STOC}
               2011, San Jose, CA, USA, 6-8 June 2011},
  pages     = {373--382},
  year      = {2011},
  url       = {
  % https://doi.org/10.1145/1993636.1993687
  },
  doi       = {
  % 10.1145/1993636.1993687
  },
  timestamp = {Tue, 06 Nov 2018 11:07:04 +0100},
  biburl    = {https://dblp.org/rec/conf/stoc/GolabHW11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{AADGMS93,
  author    = {Yehuda Afek and
               Hagit Attiya and
               Danny Dolev and
               Eli Gafni and
               Michael Merritt and
               Nir Shavit},
  title     = {Atomic Snapshots of Shared Memory.},
  journal   = jacm,
  volume    = {40},
  number    = {4},
  year      = {1993},
  pages     = {873-890}
}

@article{Aw85,
  Author = "Awerbuch, Baruch",
  Title = "Complexity of Network Synchronization",
  Journal = jacm,
  month = oct,
  Year = 1985,
  volume = 32,
  number = 4,
  pages = "804--823"
  }

@inproceedings{bushkov2012,
 author = {Bushkov, Victor and Guerraoui, Rachid and Kapalka, Michal},
 title = {On the Liveness of Transactional Memory},
 booktitle = {Proceedings of the 2012 ACM Symp. on Principles of Distributed Computing},
 series = {PODC '12},
 year = {2012},
 isbn = {978-1-4503-1450-3},
 location = {Madeira, Portugal},
 pages = {9--18},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2332432.2332435},
 doi = {10.1145/2332432.2332435},
 acmid = {2332435},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {concurrent programming, liveness, transactional memory},
}

@inproceedings{IzraelevitzMS16,
  author    = {Joseph Izraelevitz and
               Hammurabi Mendes and
               Michael L. Scott},
  title     = {Linearizability of Persistent Memory Objects Under a Full-System-Crash
               Failure Model},
  booktitle = {Distributed Computing - 30th International Symp, {DISC} 2016,
               Paris, France, September 27-29, 2016. Proceedings},
  pages     = {313--327},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-662-53426-7\_23},
  doi       = {10.1007/978-3-662-53426-7\_23},
  timestamp = {Tue, 14 May 2019 10:00:54 +0200},
  biburl    = {https://dblp.org/rec/conf/wdag/IzraelevitzMS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{EllenFRB10,
  author    = {Faith Ellen and
               Panagiota Fatourou and
               Eric Ruppert and
               Franck van Breugel},
  title     = {Non-blocking binary search trees},
  booktitle = {Proceedings of the 29th Annual {ACM} Symp. on Principles of Distributed
               Computing, {PODC} 2010, Zurich, Switzerland, July 25-28, 2010},
  pages     = {131--140},
  year      = {2010},
  url       = {https://doi.org/10.1145/1835698.1835736},
  doi       = {10.1145/1835698.1835736},
  timestamp = {Tue, 06 Nov 2018 11:07:19 +0100},
  biburl    = {https://dblp.org/rec/conf/podc/EllenFRB10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ellen-dap,
 author = {Ellen, Faith and Fatourou, Panagiota and Kosmas, Eleftherios and Milani, Alessia and Travers, Corentin},
 title = {Universal Constructions That Ensure Disjoint-access Parallelism and Wait-freedom},
 booktitle = {Proceedings of the 2012 ACM Symp. on Principles of Distributed Computing},
 series = {PODC '12},
 year = {2012},
 isbn = {978-1-4503-1450-3},
 location = {Madeira, Portugal},
 pages = {115--124},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2332432.2332457},
 doi = {10.1145/2332432.2332457},
 acmid = {2332457},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {disjoint-access parallelism, impossibility result, universal construction, wait-freedom},
} 


@article{A90,
	Author = "Ahuja, Mohan",
	Title = "{\em Flush\/} Primitives for Asynchronous Distributed
                 Systems",
	Journal = ipl,
	Volume = 34,
	number = 1,
	month = feb,
	Year = 1990,
	pages = "5--12"
}

@techreport{ADGFT01a,
  author       = "Marcos Kawazoe Aguilera and Carole Delporte-Gallet and Hugues Fauconnier and Sam Toueg",
  title = "Stable Leader Election",
  institution= liafa,
  year = 2001,
number = {2001-4},
}

@techreport{ADFT03b,
  author       = "Marcos Kawazoe Aguilera and Carole Delporte-Gallet and Hugues Fauconnier and Sam Toueg",
  title = "On implementing {Omega} with weak reliability and synchrony assumptions",
  institution= liafa,
  year = 2003,
number = {2003-7},
}
@inproceedings{ADFT03,
  author    = {Marcos Kawazoe Aguilera and
               Carole Delporte-Gallet and
               Hugues Fauconnier and
               Sam Toueg},
  title     = {On implementing {0mega} with weak reliability and synchrony
               assumptions.},
  booktitle   = "22th " # podc,
  year      = {2003},
  pages     = {306-314},
}



@inproceedings{ADFT00,
  author       = "M.K. Aguilera and C. Delporte-Gallet and H. Fauconnier 
and S. Toueg",
  title        = " Thrifty generic broadcast",
 booktitle    = proc # " 14th International Symp. on Distributed Computing",
    year         = 2000,
  place        = "Toledo ,Spain",
  editor       = springer,
  series       = {LNCS 1914},
   pages        = {268-283},
}
@inproceedings{AMT10,
	title = {View Transactions: Transactional Model with Relaxed Consistency Checks},
	author = {Yehuda Afek and Adam Morrison and Moran Tzafrir},
	booktitle = {PODC},
	year = {2010},
}

@inproceedings{ADGFT01b,
  author       = "M.K. Aguilera and C. Delporte-Gallet and H. Fauconnier and S. Toueg",
  title        = "Stable Leader Election (extended abstract)",
  booktitle    = proc # " 15th International Symp. on Distributed Computing",
  year         = 2001,
  place        = "Lisboa, Portugal",
  publisher       = springer,
  series       = {LNCS  2180},
pages        = {108-122},
  }

@INPROCEEDINGS{FGG09,
  author = {Pascal Felber and Vincent Gramoli and Rachid Guerraoui},
  title = {Elastic Transactions},
  booktitle = {DISC},
  year = {2009},
  pages = {93--107},
}

@techreport{FGG09b,
   author = {Pascal Felber and Vincent Gramoli and Rachid Guerraoui},
   title = {Elastic Transactions},
   year = {2009},
   institution = {EPFL},
   number = {LPD-REPORT-2009-002},
}    

@inproceedings{GG11-poly,
  author    = {Vincent Gramoli and
               Rachid Guerraoui},
  title     = {Brief announcement: transaction polymorphism},
  booktitle = {SPAA},
  year      = {2011},
  pages     = {311-312}
}


@INPROCEEDINGS{Gadi-Bakery,
  author = {Gadi Taubenfeld},
  title = {The Black-White Bakery Algorithm and Related Bounded-Space, Adaptive, Local-Spinning and FIFO Algorithms},
  booktitle = {DISC '04: Proceedings of the 23rd International Symp. on Distributed Computing},
  year = {2004}	
}

@inproceedings{GK03,
  author    = "Rachid Guerraoui and
               Petr Kouznetsov",
  title     = "On Failure Detectors and Type Boosters",
  booktitle = proc # " 17th International Symp. on Distributed Computing",
  year      = 2003,
  place        = "Sorrento, Italy",
  publisher       = springer,
  series       = {LNCS  2848},
  pages     = {292-305},
}

@article{GK08,
  author    = {Rachid Guerraoui and
               Petr Kouznetsov},
  title     = {Failure detectors as type boosters},
  journal   = {Distributed Computing},
  volume    = {20},
  number    = {5},
  year      = {2008},
  pages     = {343-358}
}

@article{GKK08,
  author    = {Rachid Guerraoui and
               Michal Kapalka and
               Petr Kouznetsov},
  title     = {The weakest failure detectors to boost obstruction-freedom},
  journal   = {Distributed Computing},
  volume    = {20},
  number    = {6},
  year      = {2008},
  pages     = {415-433}
}




@article{DFGK05,
  author    = {Carole Delporte-Gallet and
               Hugues Fauconnier and
               Rachid Guerraoui and
               Petr Kouznetsov},
  title     = {Mutual exclusion in asynchronous systems with failure detectors.},
  journal   = {J. Parallel Distrib. Comput.},
  volume    = {65},
  number    = {4},
  year      = {2005},
  pages     = {492-505}
}



@proceedings{DBLP:conf/wdag/2003,
  editor    = {Faith E. Fich},
  title     = {Distributed Computing, 17th International Conference, DISC
               2003, Sorrento, Italy, October 1-3, 2003, Proceedings},
  booktitle = disc,
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {2848},
  year      = {2003},
  isbn      = {3-540-20184-X},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@InProceedings{per-determinism,
   affiliation = {EPFL},
   author      = {Guerraoui, Rachid and Henzinger, Thomas A. and Singh, Vasu},
   booktitle   = {Proceedings of the 19th {I}nternational {C}onference on
                 {C}oncurrency {T}heory},
   details     = {http://infoscience.epfl.ch/record/125895},
   documenturl = {http://infoscience.epfl.ch/getfile.py?recid=125895&mode=best},
   extra-id    = {000259487000002},
   oai-id      = {oai:infoscience.epfl.ch:125895},
   oai-set     = {conf; fulltext; fulltext-public},
   review      = {REVIEWED},
   status      = {PUBLISHED},
   title       = {Completeness and {N}ondeterminism in {M}odel {C}hecking
                 {T}ransactional {M}emories},
   unit        = {LPD},
   year        = 2008
}	
@inproceedings{AACMM93,

Author = "Amir, Y. and  Moser , L.E. and Melliar-Smith, P.M. and Agarwal, D.A. and
Ciarfella, P. ",
  Title = "Fast message ordering and membership using logical token-passing ring.",
   pages = "551-565", 
  crossref = "icdcs93",


}

@inproceedings{GHKLN07,
  author    = {Rachid Guerraoui and
               Maurice Herlihy and
               Petr Kouznetsov and
               Nancy A. Lynch and
               Calvin C. Newport},
  title     = {On the weakest failure detector ever},
  booktitle = {PODC},
  year      = {2007},
  month = aug,
  pages     = {235-243}
}

@inproceedings{Bayer,
 author = {Bayer, R. and Schkolnick, M.},
 title = {Concurrency of operations on B-trees},
 booktitle = {Readings in database systems},
 year = {1988},
 isbn = {0-934613-65-6},
 pages = {129--139},
 numpages = {11},
 url = {http://dl.acm.org/citation.cfm?id=48751.48760},
 acmid = {48760},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 

@techreport{GHKLN07-TR,
author  = {Rachid Guerraoui and
               Maurice Herlihy and
               Petr Kouznetsov and
               Nancy A. Lynch and
               Calvin C. Newport},
title = {On the weakest failure detector ever},
institution = {MPI-SWS},
type = {Technical Report},
note = {"http://www.mpi-sws.mpg.de/$\sim$pkouznet/pubs/wfd.pdf"},
month = dec,
year = 2007}

@inproceedings{harris-set,
 author = {Harris, Timothy L.},
 title = {A Pragmatic Implementation of Non-blocking Linked-Lists},
 booktitle = {DISC},
 year = {2001},
 pages = {300--314},
} 


@inproceedings{michael-set,
 author = {Michael, Maged M.},
 title = {High performance dynamic lock-free hash tables and list-based sets},
 booktitle = {SPAA},
 year = {2002},
 pages = {73--82},
} 

@inproceedings{HGKLN07-TR,
  author    = {Rachid Guerraoui and
               Maurice Herlihy and
               Petr Kouznetsov and
               Nancy A. Lynch and
               Calvin C. Newport},
  title     = {On the weakest failure detector ever},
  booktitle = {PODC},
  year      = {2007},
  pages     = {235-243}
}

@inproceedings{Maged-list,
 author = {Michael, Maged M.},
 title = {High Performance Dynamic Lock-free Hash Tables and List-based Sets},
 booktitle = {Proceedings of the Fourteenth Annual ACM Symp. on Parallel Algorithms and Architectures},
 series = {SPAA '02},
 year = {2002},
 isbn = {1-58113-529-7},
 location = {Winnipeg, Manitoba, Canada},
 pages = {73--82},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/564870.564881},
 doi = {10.1145/564870.564881},
 acmid = {564881},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{AGKLR05,
Author = " Attie,P. and  Guerraoui,R. and  Kouznetsov,P. and Lynch,N. and  Rajsbaum,S.",
  Title = "The Impossibility of Boosting Distributed Service Resilience",
 
  booktitle = proc # " 25th " # icdcs,

  month = jun,
  Year = 2005,
publisher = "IEEE Computer Society Press",
  }

@article{AMMSAC95,
  Author = "Amir, Y. and Moser , L.E. Melliar-Smith, P.M. and Agarwal, D.A and Ciarfella, P.",
  Title = "The {Totem} single-ring ordering and membership protocol",
  Journal = tocs,
  month = nov,
  Year = "95",
  volume = 13,
  number = 4,
  pages = "311-342",
  }

@Article{AAFFLMWZ94,
        author =       "Y. Afek and H. Attiya and A. D. Fekete and M.
Fischer and N. Lynch and
                       Y. Mansour and D. Wang and L. Zuck",
        title =        "Reliable Communication Over Unreliable Channels",
        journal =      "Journal of the ACM",
        volume =       "41",
        number =       "6",
        year =         "1994",
        pages =        "1267--1297",
      }


@inproceedings{CZZL07,
  author    = {Wei Chen and
               Jialin Zhang and
               Yu Chen and
               Xuezheng Liu},
  title     = {Weakening Failure Detectors for {\it k}-Set Agreement
               Via the Partition Approach},
  booktitle = {DISC},
  year      = {2007},
  pages     = {123-138}
}	


@INPROCEEDINGS{ABDKPR87,
	crossref = "focs87",
	AUTHOR = {Attiya, Hagit and {Bar-Noy}, Amotz and Dolev, Danny and Koller,
			Daphne and Peleg, David and Reischuk, R{\"{u}}diger},
	TITLE = {Achievable Cases in an Asynchronous Environment},
			PAGES = {337--346},
}


@Article{ABDPR90,
        author =       "H. Attiya and A. Bar-Noy and D. Dolev and D. Peleg and
                       R. Reischuk",
        title =        "Renaming in an Asynchronous Environment",
        journal =      "Journal of the ACM",
        volume =       "37",
        number =       "3",
        pages =        "524--548",
        publisher =    "ACM Press , New York, NY , USA",
        year =         "1990"
      }


@inproceedings{ABMM95,

  Author = "Agarwal, D.A and Moser, L.E. and Melliar-Smith, P.M. and Budhia, R.K. ",
  Title = "A reliable ordered delivery protocol for interconnected local-area networks",
  booktitle = "Proceedings of the International Conference on Network Protocol",
  month = nov,
  Year = 1995,
  pages = "365-374"
  }

  }

@techreport{ACBMT95,
author  = {Emmanuelle Anceaume and Charron-Bost, Bernadette  and
     Minet, Pascale and Toueg, Sam},
title = {On the formal specification of group membership services},
institution = {INRIA, Rocquencourt},
type = {Technical Report},
month = jul,
year = 1995}

@inproceedings{ACDS85,
  crossref = "ftcs85",
  Author = "Cristian, Flaviu and Houtan Aghili and H. Raymond Strong
		and Danny Dolev",
  Title = "Atomic Broadcast:  From Simple Message Diffusion
		to {Byzantine} Agreement",
  pages = "200--206",
  note = "A revised version appears as IBM Research Laboratory Technical
		Report RJ5244 (April 1989)"
  }


@inproceedings{ACS86,
  crossref = "ftcs86",
  Author = "Cristian, Flaviu and Houtan Aghili and H. Raymond Strong",
  Title = "Approximate Clock Synchronization despite Omission and
               Performance Faults and Processor Joins"
  }

@inproceedings{ACT97,  
	AUTHOR = "Aguilera, Marcos Kawazoe and Chen, Wei and Toueg, Sam",
	TITLE = {Heartbeat: a timeout-free failure detector for
                  quiescent reliable communication},
	BOOKTITLE = proc # " 11th " # wdag,
	YEAR = {1997},
	PUBLISHER = springer,
	MONTH = sep,
        series = {LNCS 1320},
}

@techreport{ACT97b,
        author = "Aguilera, M. K. and Chen, W. and Toueg, S.",
        title = "Quiescent reliable communication and quiescent
                  consensus in partitionable networks",
	institution = "Cornell University",
        number = "TR 97-1632",
        year = "1997",
	month = jun,
        address = "Dept. of Computer Science, Cornell University, Ithaca, NY
		14853"
}
@article{ACT99,
         author = "Aguilera, Marcos Kawazoe and Chen, Wei and Toueg, Sam",
         title = "Using the {Heartbeat} Failure Detector for 
                 Quiescent Reliable Communication and Consensus
                 in Partitionable Networks",
         journal = "Theoretical Computer Science",
         year = 1999,
         month = jun,
         volume = 220,
         number = 1,
         pages = "3-30",
}

@inproceedings{ACT00,
  author = "Aguilera, Marcos Kawazoe and Chen, Wei and Toueg, Sam",
  title = "On the Quality of Service of Failure Detectors",
  year = "2000",
  booktitle = "International Conference on Dependable Systems and Networks (DSN 2000)",
  pages =  "191-200", 
  month = Jun,
  address = "New York",
}

@article{ACT00b,
	author = "Aguilera, Marcos Kawazoe and Chen, Wei and Toueg, Sam",
	title = "Failure Detection and Consensus in the Crash-Recovery Model",
        journal = "Distributed Computing", 
	publisher = springer,
        year = 2000,
        volume = 13,
        number = 2,
        month = apr,
        pages="99-125",
}
@article{AT98,
	author = "Aguilera, Marcos Kawazoe and Toueg, Sam",
	title = "Failure Detection and Randomization : a Hybrid Approach to Solve Consensus",
        journal = "Siam Journal of Computing", 
	
        year = 1998,
        volume = 28,
        number = 3,
        
        pages="890--903",
}



@article{ADLS94,
  Author = "Attiya, Hagit and Dwork, Cynthia and Lynch, Nancy and
     Stockmeyer, Larry",
  Title = "Bounds on the Time to Reach Agreement in the Presence of
                  Timing Uncertainty",
  Journal = jacm,
  month = jan,
  Year = 1994,
  volume = 41,
  number = 1,
  pages = "122--152"
  }

% note="aussi reference comme Membership algorithm in broadcast domain"
@inproceedings{ADKM92a,
  author  = {Amir, Yair and Dolev, Danny and Kramer, Shlomo and Malki, Dalia},
  title = {Membership algorithms for multicast communication groups},
  crossref = "wdag92",
  pages = {292--312},
  }


@INPROCEEDINGS{ADKM92b,
  crossref = "ftcs92",
  AUTHOR = "Amir, Yair and Danny Dolev and Shlomo Kramer and Dalia Malki",
  Title = "Transis: A communication sub-system for high availability",
  Year = "1992",
  Pages = "76-84",
   }

@inproceedings{ADS89,
  crossref = "podc89",
  Author = "Attiya, Hagit and Danny Dolev and Nir Shavit",
  Title = "Bound Polynomial Randomized Consensus (preliminary version)",
  pages = "281--293",
  }
	  
@Article{AE86,
        author =       "B. Awerbuch and S. Even",
        title =        "Reliable Broadcast Protocols in Unreliable Networks",
        journal =      "Networks: An International Journal",
        volume =       "16",
        year =         "1986",
      }


		  
@InProceedings{AGH90,
        author =       "B. Awerbuch and O. Goldreich and A. Herzberg",
        title =        "A Quantitative Approach to Dynamic Networks",
        crossref =     "podc90",
        pages =        "189--204",
      
      }

@inproceedings{AHR92,
	AUTHOR = {Attiya, Hagit and Herlihy, Maurice and Rachman, Ophir},
	TITLE = {Efficient Atomic Snapshots Using Lattice Agreement},
	crossref = "wdag92",
	
}  

@Article{ALS94,
  author = 	 { Attiya, Hagit and Lynch, Nancy and Shavit, Nir},
  title = 	 {Are wait-free algorithms fast?},
  journal = 	 "jacm",
  year = 	 {94},
  volume = 	 {41},
  number = 	 {1},
  pages = 	 {725--763},
  month = 	 jul,
 }

@Article{shavit-moir,
author = {Moir, Mark and Shavit, Nir},
 title ={Concurrent data structures},
 author = {Moir, Mark and Shavit, Nir},
 title = {Handbook Of Data Structures And Applications, Mehta, Dinesh P. and Sahni, Sartaj eds.},
 year = {2004},
 isbn = {1584884355},
 publisher = {Chapman \& Hall/CRC},
} 

@article{shavit11-ds,
  author    = {Nir Shavit},
  title     = {Data structures in the multicore age},
  journal   = {Commun. ACM},
  volume    = {54},
  number    = {3},
  year      = {2011},
  pages     = {76-84},
  ee        = {http://doi.acm.org/10.1145/1897852.1897873},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DiceLMN09,
 author = {Dice, Dave and Lev, Yossi and Moir, Mark and Nussbaum, Daniel},
 title = {Early Experience with a Commercial Hardware Transactional Memory Implementation},
 booktitle = {Proceedings of the 14th International Conference on Architectural Support for Programming Languages and Operating Systems},
 series = {ASPLOS XIV},
 year = {2009},
 isbn = {978-1-60558-406-5},
 location = {Washington, DC, USA},
 pages = {157--168},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/1508244.1508263},
 doi = {10.1145/1508244.1508263},
 acmid = {1508263},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {hardware, synchronization, transactional memory},
} 

@inproceedings{DragojevicMLM11,
 author = {Dragojevi\'{c}, Aleksandar and Herlihy, Maurice and Lev, Yossi and Moir, Mark},
 title = {On the Power of Hardware Transactional Memory to Simplify Memory Management},
 booktitle = {Proceedings of the 30th Annual ACM SIGACT-SIGOPS Symp. on Principles of Distributed Computing},
 series = {PODC '11},
 year = {2011},
 isbn = {978-1-4503-0719-2},
 location = {San Jose, California, USA},
 pages = {99--108},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1993806.1993821},
 doi = {10.1145/1993806.1993821},
 acmid = {1993821},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {hardware, memory management, synchronization, transactional memory},
} 

@inproceedings{AlistarhEMMS14,
 author = {Alistarh, Dan and Eugster, Patrick and Herlihy, Maurice and Matveev, Alexander and Shavit, Nir},
 title = {StackTrack: An Automated Transactional Approach to Concurrent Memory Reclamation},
 booktitle = {Proceedings of the Ninth European Conference on Computer Systems},
 series = {EuroSys '14},
 year = {2014},
 isbn = {978-1-4503-2704-6},
 location = {Amsterdam, The Netherlands},
 pages = {25:1--25:14},
 articleno = {25},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/2592798.2592808},
 doi = {10.1145/2592798.2592808},
 acmid = {2592808},
 publisher = {ACM},
 address = {New York, NY, USA},
} 



@Article{MMA93,
  author = 	 {Moser, Louise E. and Melliar-Smith P.M. and Agrawala, Vivek},
  title = 	 {Asynchronous fault-tolerant total ordering algorithms},
  journal = 	 {SIAM J. COMPUT},
  year = 	 {93},
  volume = 	 {22},
  number = 	 {4},
  pages = 	 {727--750},
  month = 	 aug,
 }

@Article{AMM94,
  author = 	 {Moser, Louise E. and Melliar-Smith P.M. and Agrawala, Vivek},
  title = 	 {Processor membership in asynchronous distributed systems},
 journal = 	 {IEEE Transactions on Parallel and Distribued Systems },
  year = 	 {94},
  volume = 	 {5},
  number = 	 {5},
  pages = 	 {459-473},
  month = 	 may,
 }

@ARTICLE{AHCAS,
author={Attiya, H. and Hendler, D.},
journal={Parallel and Distributed Systems, IEEE Transactions on}, title={Time and Space Lower Bounds for Implementations Using k-CAS},
year={2010},
month={feb. },
volume={21},
number={2},
pages={162 -173},
keywords={k-CAS synchronization primitives;k-compare amp;swap synchronization primitives;lower bound;space complexity;time complexity;computational complexity;concurrency theory;data structures;},
doi={10.1109/TPDS.2009.60},
ISSN={1045-9219},}


@article{AR97,

  Author = "Attiya Hagit and Rappoport, Rinat",
  Title = "The level of Handshake required for managing a connection
		",
  Journal = dc,
  volume = 11,
  Year = 1997,
pages = "41--57",
  }


@article{AS85,
	Author = "Alpern, Bowen and Schneider, Fred B.",
	Title = "Defining Liveness",
	Journal = ipl,
	Volume = 21,
	number = 4,
	month = oct,
	Year = 1985,
	pages = "181--185"
}	



@article{AWH92,
  Author = "Amdur, Eugene and Sam Weber and Vassos Hadzilacos",
  Title = "On the Message Complexity of Binary Byzantine Agreement
                under Crash Failures" ,
  Journal = dc,
  Year = 1992,
  volume = 5,
  number = 2,
  pages = "175--186"
  }


%B-----------------------------------------------------------------------
@inproceedings{Ben83,
  crossref = "podc83",
  Author = "Ben{-}Or, Michael",
  Title = "Another advantage of free choice:  Completely asynchronous
		agreement protocols",
  pages = "27--30"
  }
@article{Bir93,
author  = {Birman, Kenneth P.},
journal = {Communication of the ACM},
title = {The process group approach to reliable distributed computing},
volume = {9},
number = 12,
pages = {36--53},
month = dec,
year = 1993}

@book{BvR94,
  author  = {Birman, Kenneth P. and van Renesse, Robbert},
  title = { Reliable Distributed Computing with the ISIS Toolkit},
publisher = {IEEE Computer Society Press},
year = 1994}

@InProceedings{Bir85,
        author =       "K. Birman",
        title =        "Replication and Fault-Tolerance in the {ISIS} System",
        booktitle =    "Proceedings of the 10th ACM Symp. on Operating
                       Systems Principles",
        pages =        "79--86",
        address =      "Orcas Island, WA USA",
        year =         "1985"
}
	

@article{Bra87a,
  Author = "Bracha, Gabriel",
  Title = "Asynchronous {Byzantine} Agreement Protocols",
  Journal = ic,
  month = nov,
  Year = 1987,
  volume = 75,
  number = 2,
  pages = "130--143"
  }

@article{Bra87b,
  Author = "Bracha, Gabriel",
  Title = "An {$O(\log n)$} Expected Rounds Randomized
		{Byzantine} Generals Protocol",
  Journal = jacm,
  month = oct,
  Year = 1987,
  volume = 34,
  number = 4,
  pages = "910--920"
  }



@InProceedings{BMS02,
  author = 	 {Bertier, Marin and Marin, Olivier and Sens, Pierre},
  title = 	 {Implementation and Performance Evaluation of an Adaptable Failure Detector},
  booktitle = 	 {Proceedings of the 2002 International Conference on Dependable Systems and Networks },
  year = 	 {2002},
  month = 	 jun,
place ={Washington, DC},
page={345--364}
}



@article{GK99-undecidable,
  author    = {Eli Gafni and
               Elias Koutsoupias},
  title     = {Three-Processor Tasks Are Undecidable},
  journal   = {SIAM J. Comput.},
  volume    = {28},
  number    = {3},
  year      = {1999},
  pages     = {970-983},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}




@article{BBD97,
author = {Babao\u{g}lu, \"{O}zalp and Bartoli Alberto and Dini Gianluca},
title = { Enriched View Synchrony: A Programming Paradigm for Partitionable Asynchronous Distributed Systems},
journal = {IEEE Transactions on computers},
volume = 46,
number = 6,
month = jun,
year = 1997,
}

@inproceedings{BCGRS93,
author  = {Van Renesse, Robbert and Birman, Kenneth P. and Cooper,
Robert and Glade, Bradford
				  and Stephenson, Patrick},
title = {The Horus system},
booktitle = {Reliable Distributed Computing with the Isis Toolkit},
editor = {Birman, Kenneth P. and van Renesse, Robbert},
publisher = {IEEE Computer Society Press, Los Alamitos, CA},
pages = {133--147},
year = 1993}

}

@MANUAL{BCJKS90,
	TITLE = {Isis - A Distributed Programming Environment},
	AUTHOR = {Birman, Kenneth P. and Cooper, Robert and Joseph, Thomas A. and
		Kane, Kenneth P. and Schmuck, Frank Bernhard},
	MONTH = jun,
	YEAR = 1990
}

@InProceedings{BCT96,
  Author = "A. Basu and B. Charron-Bost and S. Toueg",
  Title = "Simulating Reliable Links with Unreliable Links in the
Presence of Process Crashes",
  pages = "105--122",
  booktitle = proc # " Tenth " # wdag,
  editor = "{Babao{\u{g}}}lu, {\"{O}}. and K. Marzullo",
  confaddress = "Bologna, Italy",
  series = lncs,
  volume = 1151,
  month = oct,
  Year = 1996,
  publisher = springer,
  }

@techreport{BD85a,
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Rog{\'{e}}rio Drummond},
  Title = "Communication-Time Tradeoffs for Reliable Broadcast Protocols",
  Institution = cornellcs,
  month = jun,
  Year = 1985,
  number = "85-687"
  }
@article{BD85b,
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Rog{\'{e}}rio Drummond},
  Title = "Streets of {Byzantium}:  Network Architectures
		for Fast Reliable Broadcasts",
  Journal = ieeese,
  month = jun,
  Year = 1985,
  volume = 11,
  number = 6,
  pages = "546--554"
  }
  
@inproceedings{BD87,
  crossref = "ftcs87",
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Rog{\'{e}}rio Drummond},
  Title = "({Almost}) No Cost Clock Synchronization",
  pages = "42--47"
  }

@incollection{BD88,
  Author = "Bar{-}Noy, Amotz and Danny Dolev",
  Title = "Families of Consensus Protocols",
  booktitle = "Proceedings of the Third Aegean Workshop on Computing:
  		VLSI Algorithms and Architectures",
  editor = "J. H. Reif",
  series = lncs,
  month = jul,
  Year = 1988,
  volume = 319,
  publisher = springer,
  pages = "380--390"
  }



@book{BDGB94,
  author  = {Babao\u{g}lu, \"{O}zalp and Davoli, Renzo and Giachini,
    Luigi-Alberto and Baker, Mary Gray},
  title = {RELACS: a communications infrastructure for constructing
   reliable applications in large-scale distributed systems},
  publisher = {BROADCAST Project deliverable report},
  note = {Department of Computing Science, University of Newcastle upon
                  Tyne, UK},
  year = 1994,
}


@techreport{BDM95,
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Davoli, R. and Montresor, A.},
  Title = "Failures Detectors, Group Membership and 
           View-Synchronous Communication in Partitionable 
            Asynchronous Systems",
  Institution = "Department of Computer Science, University of Bologna",
  month = nov,
  Year = 1995,
  number = "TR UBLCS95-18",
  }

@techreport{BDM97,
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Davoli, R. and Montresor, A.},
  Title = "Partitionable Group Membership: Specifications and Algorithms",
  Institution = "Department of Computer Science, University of Bologna",
  month = jan,
  Year = 199,
  number = "TR UBLCS97-1"
  }



@incollection{BG89,
  Author = "Berman, Piotr and Juan A. Garay",
  Title = "Asymptotically Optimal Consensus",
  booktitle = proc # " Sixteenth " # icalp,
  pages = "80--94",
  Volume = "372",
  publisher = springer,
  series = lncs,
  Year = 1989
  }
@incollection{BG93,
  Author = "Berman, Piotr and Bharali, Anupam A.",
  Title = "Quick Atomic Broadcast",
  booktitle =" " ,
  pages = "189-203",
  Volume = " ",
  publisher = " ",
  series = " ",
  Year = 93,
  }
@inproceedings{BG93b,
    Author = {Elizabeth Borowsky and Eli Gafni},
  Title = "Generalized {FLP} impossibility result for $t$-resilient asynchronous computations  ",

  booktitle = {STOC},

  month = may,
  Year = 1993,
  confaddress = "San Diego, California",
  confeditor = "Alok Aggrawal",
  publisher = "ACM Press",
 
  pages = "91--100"
  }

@article{BGLR01,
  author    = {Elizabeth Borowsky and
               Eli Gafni and
               Nancy A. Lynch and
               Sergio Rajsbaum},
  title     = {The {BG} distributed simulation algorithm},
  journal   = {Distributed Computing},
  volume    = {14},
  number    = {3},
  year      = {2001},
  pages     = {127-146}
}

@inproceedings{vechev08,
  author    = {Martin T. Vechev and
               Eran Yahav},
  title     = {Deriving linearizable fine-grained concurrent objects},
  booktitle = {PLDI},
  year      = {2008},
  pages     = {125-135},
  ee        = {http://doi.acm.org/10.1145/1375581.1375598},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@techreport{BGP89a,
  Author = "Berman, Piotr and Juan A. Garay and Kenneth J. Perry",
  Title = "Recursive Phase King Protocols for Distributed Systems",
  number = "89-24",
  Institution = "Department of Computer Science, The Pennsylvania State
		University",
  month = aug,
  Year = 1989
  }

@inproceedings{BGP89b,
  crossref = "FOCS89",
  Author = "Berman, Piotr and Juan A. Garay and Kenneth J. Perry",
  Title = "Towards Optimal Distributed Consensus",
  pages = "410--415"
  }

@article{BG86a,
  Author = "Bernstein, Philip A. and Nathan Goodman",
  Title = "A Proof Technique for Concurrency Control and Recovery
		Algorithms for Replicated Databases",
  Journal = dc,
  volume = 1,
  Year = 1986
  }

@article{BG86b,
  Author = "Bernstein, Philip A. and Nathan Goodman",
  Title = "Serializability Theory for Replicated Databases",
  Journal = jcss,
  volume = 31,
  number = 3,
  month = dec,
  Year = 1986,
  pages = "355--374"
  }

@book{BHG87,
  Author = "Bernstein, Philip A. and Vassos Hadzilacos and Nathan Goodman",
  Title = "Concurrency Control and Recovery in Database Systems",
  Publisher = "Addison-Wesley",
  Year = 1987
  }



@inproceedings{BJ87a,
  Author = "Birman, Kenneth P. and Thomas A. Joseph",
  Title = "Exploiting Virtual Synchrony in Distributed Systems",
  booktitle = "Proceedings of the 11th ACM Symp. on Operating
		Systems Principles",
  month = nov,
  Year = 1987,
  pages = "123--138"
  }

@article{BJ87b,
  Author = "Birman, Kenneth P. and Thomas A. Joseph",
  Title = "Reliable Communication in the Presence of Failures",
  Journal = tocs,
  month = feb,
  Year = 1987,
  volume = 5,
  number = 1,
  pages = "47--76"
  }
  
@techreport{BJ88,
  Author = "Birman, Kenneth P. and Thomas A. Joseph",
  Title = "Exploiting Replication",
  number = "88-917",
  Institution = cornellcs,
  month = may,
  Year = 1988,
  note = "To appear in {\em An Advanced Course in Distributed Computing
		(Lecture Notes from the Arctic '88 Short Course)},
		Addison-Wesley, July 1989"
  }

@incollection{BJ89a,
  Author = "Birman, Kenneth P. and Thomas A. Joseph",
  Title = "Reliable Broadcast Protocols",
  Editor = "Mullender, Sape J.",
  booktitle = "An Advanced Course in Distributed Computing",
  Publisher = "Addison-Wesley",
  Year = "1989",
  Chapter = 14
  }

@incollection{BJ89b,
  Author = "Birman, Kenneth P. and Thomas A. Joseph",
  Title = "Exploiting Replication in Distributed Systems",
  Editor = "Mullender, Sape J.",
  booktitle = "An Advanced Course in Distributed Computing",
  Publisher = "Addison-Wesley",
  Year = "1989",
  Chapter = 15
  }

@inproceedings{BMZ88,
	crossref = "podc88",
	Author = "Biran, Ofer and Moran, Shlomo and Zaks, Shmuel",
	Title = "A combinatorial characterization of the distributed tasks
		that are solvable in the presence of one faulty processor",
	pages = "263--275"
}
@techreport{BN92,
  Author = "Burns, James E. and Gil Neiger",
  Title = "Fast and Simple {Byzantine} Agreement",
  Institution = gatech,
  month = mar,
  Year = 1992,
  number = "92/12"
  }
@TECHREPORT{BSS90,
	AUTHOR = {Birman, Kenneth P. and Schiper, Andre and Stephenson, Pat},
	TITLE = {Fast Causal Multicast},
	INSTITUTION = cornellcs,
	YEAR = {1990},
	NUMBER = {90-1105},
	MONTH = apr
}

@article{BSS91,
	AUTHOR = {Birman, Kenneth P. and Schiper, Andre and Stephenson, Pat},
	TITLE = {Lightweight Causal and Atomic Group Multicast},
	Journal = tocs,
	YEAR = {1991},
        Month = aug,
        Volume = 9,
	NUMBER = 3,
	pages = "272--314"
}


@incollection{BT93,
  Author = {Babao{\u{g}}lu, {\"{O}}zalp and Sam Toueg},
  Title = "Non-Blocking Atomic Commitment",
  Editor = "Mullender, Sape J.",
  booktitle = "Distributed Systems",
  Publisher = "Addison-Wesley",
  Year = "1993",
  Chapter = 6
  }

@article{BT85,
  Author = "Bracha, Gabriel and Sam Toueg",
  Title = "Asynchronous Consensus and Broadcast Protocols",
  Journal = jacm,
  month = oct,
  Year = 1985,
  volume = 32,
  number = 4,
  pages = "824--840"
  }

  
@article{BT87,
  Author = "Bracha, Gabriel and Sam Toueg",
  Title = "Distributed Deadlock Detection",
  journal = dc,
  year = 1987,
  volume = 2,
  pages = "127--138"
  }


@article{BNP97,
author={Rida A. Bazzi and Gil Neiger and Gary L. Peterson},
title={ On the Use of Registers in Achieving Wait-Free Consensus},
journal=dc,
volume=10,
number=3,
pages={117--127},
year=1997,
}

@inproceedings{BG93a,
  author =     {Elizabeth Borowsky and Eli Gafni},
  title =     {Immediate atomic snapshots and fast renaming},
  booktitle =     {PODC},
  year =     {1993},
  isbn =     {0-89791-613-1},
  pages =     {41--51},
  location =     {Ithaca, New York, United States},
  doi =         {http://doi.acm.org/10.1145/164051.164056},
  publisher =     {ACM Press},
  address =     {New York, NY, USA},
}

@inproceedings{KS06,
  author =     {Idit Keidar and Alex Shraer},
  title =     {Timeliness, Failure Detectors and Consensus Peformance},
  booktitle =     {PODC '06: Proceedings of the annual ACM Symp.
on
                  Principles of distributed computing},
  year =     {2006},
  location =     {Denver, Colorado, United States},
  publisher =     {ACM Press},
  address =     {New York, NY, USA},
}



@inproceedings{DG02a,
  author    = {Partha Dutta and
               Rachid Guerraoui},
  title     = {The inherent price of indulgence.},
  booktitle = {PODC '02: Proceedings of the  annual ACM Symp. on Principles of distributed computing},
  year      = {2002},
  pages     = {88-97},
  ee        = {http://doi.acm.org/10.1145/571825.571838},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}




@inproceedings{BG97,
  author =     {Elizabeth Borowsky and Eli Gafni},
  title =     {A simple algorithmically reasoned characterization of
                  wait-free computation (extended abstract)},
  booktitle =     {PODC '97: Proceedings of the sixteenth annual ACM Symp.                   on Principles of distributed computing},
  year =     {1997},
  isbn =     {0-89791-952-1},
  pages =     {189--198},
  location =     {Santa Barbara, California, United States},
  doi =         {http://doi.acm.org/10.1145/259380.259439},
  publisher =     {ACM Press},
  address =     {New York, NY, USA},
}


%----------------------------------------------------------------
%C

@techreport{Crit89,
  Author = "Critchlow, Carol",
  Title = "On Inhibition and Atomicity in Asynchronous Consistent-Cut
		Protocols",
  Institution = cornellcs,
  month = dec,
  Year = 1989,
  number = "90-1069"
  }

		 
@InProceedings{Cha90,
        author =       "Soma Chaudhuri",
        title =        "Agreement is Harder than Consensus: Set Consensus
                       Problems in Totally Asynchronous Systems",
        booktitle =     proc # " 9th " # podc,
        month =        aug,
        year =         "1990",
        pages = "311--324",
        address =      "Qu\'ebec City, Qu\'ebec, Canada",
      }
@article{Cha93,
   Author =       "Soma Chaudhuri",
   title =        "More {\em choices} allow more {\em faults}:
              Set consensus      Problems in Totally Asynchronous Systems",
   
  Journal = "Information and Computation",
  Year = 1993,
  volume = 105,
  Number = 1,
  pages = "132--158"
      }

@inproceedings{CHLT93,
  crossref = "focs93",
   Author =       "Chaudhuri, Soma and Herlihy, Maurice and Lynch, Nancy A. and Tuttle, Mark",
   title =        "A tight lower-bound for {$k$-set} agreement",
    pages = "206--215",
         }

@InProceedings{CHJT94,
 author = {Tushar D. Chandra and Vassos Hadzilacos and Prasad Jayanti and Sam Toueg},
 title = {Wait-freedom vs. $t$-resiliency and the robustness of wait-free hierarchies},
 booktitle = podc,
 year = {1994},
 pages = {334-343},
 location = {Los Angeles, California, United States},
 OPTpublisher = {ACM Press}
 }
        
@inproceedings{JT08,
  author    = {Prasad Jayanti and
               Sam Toueg},
  title     = {Every problem has a weakest failure detector},
  booktitle = {PODC},
  year      = {2008},
  pages     = {75-84}
}

@InProceedings{Zie08,
 author = {Piotr Zieli\'nski},
 title = {Anti-Omega: the weakest failure detector for set agreement},
 booktitle = {PODC},
 month = aug, 
year = {2008},
  
 OPTpublisher = {ACM Press}
 }






@article{Chu98,
  Author = "Chu, F.",
  Title = "Reducing {$\Omega$} to {$\Diamond W$}",
  Journal = "Information Processing Letters",
  Volume = " 67 ",
  Number = 6,
  Pages = "298-293",
  year = 1998,
  month = sep,
}

@techreport{CBS00,
author =       "Bernadette Charron-Bost  and
                 {Andr\'e} Schiper",
title = "Uniform consensus is harder than consensus (extended abstract)",
institution= EPFL,
year = "2000",
type={Technical Report},
month = may,
number= "DSC/2000/028",
}  


@article{CD89,
  Author = "Chor, Benny and  Cynthia Dwork",
  Title = "Randomization in Byzantine Agreement",
  Journal = "Advances in Computer Research",
  Year = 1989,
  volume = 5,
  pages = "443--497"
  }




@article{CHM83,
  Author = "Chandy, K. Mani and Laura M. Haas and Jayadev Misra",
  Title = "Distributed Deadlock Detection",
  Journal = tocs,
  month = may,
  Year = 1983,
  volume = 1,
  number = 2,
  pages = "144--156"
  }

@inproceedings{CHTCB96,
  Author  = {Chandra, Tushar Deepak and  Hadzilacos, Vassos and Toueg,
                  Sam and Charron-Bost, Bernadette},
  Title = {On the Impossibility of Group Membership},
  booktitle =     proc # " 15th " # podc,
  month = may,
  year = "1996",
  pages = "322--330",
  confaddress =  "Philadelphia, Pennsylvania, USA",
  }



@InProceedings{CHT92a,
  author = 	"Chandra, Tushar Deepak and Hadzilacos, Vassos and Toueg, Sam",
  title = 	"The Weakest Failure Detector for Solving Consensus",
  pages = 	"147--158",
crossref =   "podc92",
 }

@article{CHT96,
  Author = " Chandra, Tushar Deepak and Hadzilacos, Vassos and Toueg, Sam",
  Title = "The weakest failure detector for solving consensus ",
  Journal = jacm,
  month = jul,
  Year = 1996,
  volume = 43,
  number = 4,
  pages = "685--722"
  }
@INPROCEEDINGS{CT91,
	Author = "Chandra, Tushar Deepak and Toueg, Sam",
	Title = "Unreliable Failure Detectors for Asynchronous Systems
(Preliminary Version)",
	crossref = "podc91",
	PAGES = "325--340",
	}

@techreport{CT94,
  Author = {Charron-Bost, B. and Tel, G.},
  Title = {Approximation d'une borne inf\'erieure r\'epartie},
  number = {LIX/RR/94/06},
  Institution = {Laboratoire d'Informatique LIX, \'Ecole Polytechnique},
  month = sep,
  Year = 1994
  }


@article{CT96,
  Author = " Chandra, Tushar Deepak and Toueg, Sam",
  Title = "Unreliable Failure Detectors for Reliable Distributed Systems",
  Journal = jacm,
  month = mar,
  Year = 1996,
  volume = 43,
  number = 2,
  pages = "225--267"
  }



@inproceedings{CM91,
  author = " R. Cooper and K. Marzullo",
  title = "Consistent Detection of Global Predicates",
  booktitle = "Proceedings of the ACM/ONR Workshop on Parallel and 
             Distributed Debugging",
  publisher = "ACM, New York",
  year = 1991,
  pages = " 163--173"
  }



@article{CL85,
  Author = "Chandy, K. Mani and Leslie Lamport",
  Title = "Distributed Snapshots:  Determining Global States of Distributed
  		Systems",
  Journal = tocs,
  month = feb,
  Year = 1985,
  volume = 3,
  number = 1,
  pages = "63--75"
  }
  
@article{CM86,
  Author = "Chandy, K. Mani and Jayadev Misra",
  Title = "How Processes Learn",
  Journal = dc,
  Year = 1986,
  volume = 1,
  number = 1,
  pages = "40--52"
  }

@book{CM88,
  Author = "Chandy, K. Mani and Jayadev Misra",
  Title = "Parallel Program Design: A foundation",
  Publisher = {Addison-Wesley},
  Address = {Reading Massachusetts},
  Year = 1988
  }

@article{CM84,
  author = "Chang, Jo-Mei and N.F. Maxemchuk",
  title = "Reliable broadcast protocols",
  journal = tocs,
  year = 1984,
  volume = 2,
  number = 3,
  month = aug,
  pages = "251--273"
}

@INPROCEEDINGS{CAA90,
	  AUTHOR = {S. Y. Cheug and M. Ahamad and M. H. Amnar},
	  TITLE = {The grid protocol: A high performance scheme for
maintaining replicated data},
	  BOOKTITLE = {Proceedings of the sixth IEEE conference on Data
Engineering},
	  YEAR = {1990},
	  PAGES = {438--445},
	  MONTH = Jan
}

@inproceedings{CIL87,
  crossref = "podc87",
  Author = "Chor, Benny and Amos Israeli and Ming Li",
  Title = "On Processor Coordination Using Asynchronous Hardware",
  pages = "222--231"
  }

@inproceedings{Coa86,
  crossref = "podc86",
  Author = "Coan, Brian A.",
  Title = "A Communication-Efficient Canonical Form for Fault-Tolerant
		Distributed Protocols",
  pages = "63--72",
  note = "A revised version appears in Coan's Ph.D.\ dissertation~\cite{Coa87}"
  }

@phdthesis{Coa87,
  Author = "Coan, Brian A.",
  Title = "Achieving Consensus in Fault-Tolerant Distributed
		Computer Systems:  Protocols, Lower Bounds, and Simulations",
  School = "Massachusetts Institute of Technology",
  month = jun,
  Year = 1987
  }

@article{Coa88a,
  Author = "Coan, Brian A.",
  Title = "A Compiler that Increases the Fault-Tolerance of Asynchronous
		Protocols",
  Journal = ieeetc,
  volume = 37,
  number = 12,
  month = dec,
  year = 1988,
  pages = "1541--1553"
  }

@inproceedings{Coa88b,
  Author = "Coan, Brian A.",
  Title = "Efficient Agreement using Fault Diagnosis",
  booktitle = "Proceedings of the Twenty-Sixth Annual Allerton Conference
		on Communication, Control, and Computing",
  month = sep,
  Year = 1988
  }


@article{CDDS89,
  Author = "Coan, Brian A. and Danny Dolev and Cynthia Dwork
		and Larry Stockmeyer",
  Title = "The Distributed Firing Squad Problem",
  Journal = sicomp,
  month = oct,
  Year = 1989,
  volume = 18,
  number = 5,
  pages = "990--1012"
  }

@INPROCEEDINGS{CW86,
	crossref = "podc86",
	AUTHOR = {Coan, Brian A. and Jennifer L. Welch},
	TITLE = {Transaction Commit in a Realistic Fault Model},
	PAGES = {40--51}
}

@inproceedings{CW89,
  crossref = "podc89",
  Author = "Coan, Brian A. and Jennifer L. Welch",
  Title = "Modular Construction of Nearly Optimal {Byzantine} Agreement
  		Protocols",
  pages = "295--306"
  }

@article{CW92,
  Author = "Coan, Brian A. and Jennifer L. Welch",
  Title = "Modular Construction of a {Byzantine} Agreement Protocol
with Optimal Message Bit Complexity",
  Journal = ic,
  Volume = 97,
  Number = 1,
  Year = 1992,
  Month = mar,
  pages = "61--85"
  }


@INPROCEEDINGS{Cri87,
	AUTHOR = {Cristian, Flaviu},
	TITLE = {Issues in the Design of Highly Available Computing Services},
	BOOKTITLE = {Annual Symp. of the Canadian Information
Processing Society},
	YEAR = {1987},
	PAGES = {9--16},
	MONTH = jul,
	Note = "Also IBM Research Report RJ5856, July 1987"
}


@article{Cri91,
author  = {Cristian, Flaviu},
journal = {Distributed Computing},
title = {Reaching agreement on processor group membership in
synchronous distributed systems},
volume = {4},
number = 4,
pages = {175--187},
month = apr,
year = 1991}


@techreport{Cri88,
  Author = "Cristian, Flaviu",
  Title = "Probabilistic Clock Synchronization",
  Institution = ibmrl,
  month = oct,
  Year = 1988,
  number = "RJ6432"
  }

@article{Cri89a,
  Author = {Flaviu Cristian},
  Title = "Probabilistic Clock Synchronization",
  Journal = dc,
  Year = 1989,
  volume = 3,
  pages = "146--158"
  }


@TECHREPORT{Cri89,
	AUTHOR = {Cristian, Flaviu},
	TITLE = {Synchronous Atomic Broadcast for Redundant Broadcast Channels},
	INSTITUTION = ibmrl,
	YEAR = {1989},
	NUMBER = {RJ7203},
	MONTH = dec,
	NOTE = {Revised April 1990}
}


@article{Cri90b,
  Author = {Cristian, Flaviu},
  Title = {Synchronous Atomic Broadcast for Redundant Broadcast Channels},
  Journal = "Real-Time Systems",
  Year = 1990,
  Month= sep,
  volume = 2,
  number = 3,
  pages = "195--212",
  Note = "Also IBM Research Report RJ7203, December 1989 (revised April 1990)."
  }

@techreport{CDD90,
  Author = "Cristian, Flaviu and Robert D. Dancey and Jon Dehn",
  Title = "Fault-Tolerance in the Advanced Automation System",
  Institution = ibmrl,
  month = apr,
   title     = {Fail-Awareness: An Approach to Construct Fail-Safe Applications},
   booktitle = {Proceedings of the 27th Annual International Symp. on Fault-Tolerant Computing},
   year      = {1997},
   month     = jun,
   address   = {Seattle},
   abstract  = {We present a framework for building fail-safe hard real-time 
                applications on top of an asynchronous distributed system 
                subject to communication partitions, i.e. using processors 
                and communication facilities whose real-time delays cannot 
                be guaranteed. The basic assumption behind our approach is 
                that each processor has a local hardware clock that proceeds 
                within a linear envelope of real-time. This allows to compute 
                an upper bound on the actual delays incurred by a particular 
                processing sequence or message transmission. Services and 
                applications can use these computed bounds to detect when 
                they cannot guarantee all their standard properties because 
                of excessive delays. This allows an application to detect 
                when to switch to an exception fail-safe mode.},
   URL       = {http://www.research.att.com/\~christof/FAPS},
}


@inproceedings{CF97b,
   author    = {Fetzer, C. and Cristian, F.},
   title     = {A Fail-Aware Membership Service},
   booktitle = {SRDS' 97: Proceedings of the 16th Symp. on IEEE Reliable Distributed Systems},
   year      = {1997},
   month     = oct,
   pages     = {157--164},
   abstract  = {We propose a new protocol that can be used to implement 
                majority-partition and partitionable membership services 
                for timed asynchronous systems. The protocol is fail-aware 
                in the sense that a process p knows at all times if its 
                approximation of the set of processes in its partition 
                is up-to-date or out-of-date. The protocol minimizes
                wrong suspicions of processes by giving processes a 
                second chance to stay in the membership before they 
                are removed. Our measurements show that the exclusion 
                of alive processes is rare and the crash detection 
                times are good. The protocol guarantees that the 
                memberships of two partitions never overlap. },
   URL       = {http://www.research.att.com/\~christof/FAMS},
}




@article{CF99,
   author    = {Cristian, F. and Fetzer, C.},
   title     = {The Timed Asynchronous Distributed System Model},
   journal   = {IEEE Transactions on Parallel and Distributed Systems},
   abstract  = {We propose a formal definition for the timed asynchronous 
                system model, we describe extensive measurements of actual 
                message and process scheduling delays and hardware clock 
                drifts that confirm that this model adequately 
                describes current distributed 
                systems built from networked workstations, and we give an 
                explanation of why practically needed services, such as 
                consensus or leader election, which are not implementable 
                in the time-free asynchronous system model, are implementable 
                in the timed model. },
   URL       = {http://www.research.att.com/\~christof/MODEL},
   year      = {1999},
   month     = jun,
   volumne   = {10},
   pages     = {642-657},
   issue     = {6}
}

@TECHREPORT{CS95,
	AUTHOR = {Cristian, F. and Schmuck, F.},
	TITLE = {Agreeing on processor-group membership in
                  asynchronous distributed systems},
	INSTITUTION = {UCSD},
	YEAR = {1995},
	NUMBER = {CSE95-428}
}

@TECHREPORT{fraser,
	AUTHOR = {Fraser, K.},
	TITLE = {Practical lock-freedom},
	INSTITUTION = {Cambridge University Computer Laborotory},
	YEAR = {2003}

}
@inproceedings{nztm,
 author = {Tabba, Fuad and Moir, Mark and Goodman, James R. and Hay, Andrew W. and Wang, Cong},
 title = {NZTM: Nonblocking Zero-indirection Transactional Memory},
 booktitle = {Proceedings of the Twenty-first Annual Symp. on Parallelism in Algorithms and Architectures},
 series = {SPAA '09},
 year = {2009},
 isbn = {978-1-60558-606-9},
 location = {Calgary, AB, Canada},
 pages = {204--213},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1583991.1584048},
 doi = {10.1145/1583991.1584048},
 acmid = {1584048},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {hardware support, nonblocking synchronization, transactional memory},
} 

@inproceedings{CT90,
  crossref = "podc90",
  Author = "Critchlow, Carol and Kim Taylor",
  Title = "The Inhibition Spectrum and the Achievement of Causal Consistency",
  note = "An expanded version appears as Cornell University Department of
		Computer Science Technical Report 90-1101"
  }

@inproceedings{ CL99,
    author = "Castro, Miguel   and Barbara Liskov",
    title = "Practical Byzantine Fault Tolerance",
    booktitle = "{OSDI}: Symp. on Operating Systems Design and Implementation",
    publisher = "USENIX Association, Co-sponsored by IEEE TCOS and ACM SIGOPS",
    year = "1999",
    month = feb,
}


@Article{CL02,
  author = 	 { Castro, Miguel and Barbara Liskov},
  title = 	 {Practical byzantine fault tolerance and proactive recovery },
  journal = 	 {ACM Transactions on Computer Systems (TOCS)},
  year = 	 {2002},
  volume = 	 {20},
  number = 	 {4},
  pages = 	 {398--461},
  month = 	 nov,

}

@inproceedings{Lee05,
  author    = {Hyonho Lee},
  title     = {Transformations of Mutual Exclusion Algorithms from the Cache-Coherent
               Model to the Distributed Shared Memory Model},
  booktitle = {25th International Conference on Distributed Computing Systems {(ICDCS}
               2005), 6-10 June 2005, Columbus, OH, {USA}},
  year      = {2005},
  pages     = {261--270},
  
  url       = {http://doi.ieeecomputersociety.org/10.1109/ICDCS.2005.83},
  doi       = {10.1109/ICDCS.2005.83},
  timestamp = {Wed, 12 Nov 2014 22:50:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icdcs/Lee05},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{AlistarhAGG11,
  author    = {Dan Alistarh and
               James Aspnes and
               Seth Gilbert and
               Rachid Guerraoui},
  title     = {The Complexity of Renaming},
  booktitle = {{IEEE} 52nd Annual Symp. on Foundations of Computer Science, {FOCS}
               2011, Palm Springs, CA, USA, October 22-25, 2011},
  year      = {2011},
  pages     = {718--727},
  
  url       = {http://dx.doi.org/10.1109/FOCS.2011.66},
  doi       = {10.1109/FOCS.2011.66},
  timestamp = {Wed, 12 Nov 2014 22:43:16 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/focs/AlistarhAGG11},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{damien-vw,
  author    = {Damien Imbs and
               Jos{\'e} Ram{\'o}n Gonz{\'a}lez de Mend\'{\i}vil and
               Michel Raynal},
  title     = {Brief announcement: virtual world consistency: a new condition
               for STM systems},
  booktitle = {PODC},
  year      = {2009},
  pages     = {280-281},
  ee        = {http://doi.acm.org/10.1145/1582716.1582764},
 
}

@inproceedings{cond-04,
 author = {Fich, Faith and Hendler, Danny and Shavit, Nir},
 title = {On the Inherent Weakness of Conditional Synchronization Primitives},
 booktitle = {Proceedings of the Twenty-third Annual ACM Symp. on Principles of Distributed Computing},
 series = {PODC '04},
 year = {2004},
 isbn = {1-58113-802-4},
 location = {St. John's, Newfoundland, Canada},
 pages = {80--87},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1011767.1011780},
 doi = {10.1145/1011767.1011780},
 acmid = {1011780},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {compare-and-swap, load-linked, lower bounds, store-conditional, synchronization primitives, test-and-set, wait-freedom},
} 


@techReport{DFKM96,
   author =      {Dolev, D. and Friedman, R. and Keidar, I. and Malki, D.},
   title =       {Failure detectors in omission failure environments},
   institution = {Cornell University},
   address = "Dept. of Computer Science, Cornell University, Ithaca, NY
		14853",
   year =        "1996",
   number = "TR 96-1608",
   
}


@Article{DS80,
    Author = "Dijkstra, E.~W. and  Scholten, C.~S.",
    Title = "Termination detection for diffusing computations",
    Journal = ipl,
    volume = 11,
    Number = 1,
    Year = 1980,
    month = Aug,
    Pages = "1--4"
       }

@Article{DFG83,
    Author = "Dijkstra, E.~W. and Feijen, W. H. and van Gasteren, A. J.",
    Title = "Derivation of a termination detection algorithm for distributed
  computations",
    Journal = ipl,
    volume = 16,
    Number = 5,
    Year = 1983,
    month = Jun,
    Pages = "217--219"
       }






@InProceedings{DT00,
  author = 	 {Deianov, Boris and Toueg, Sam},
  title = 	 {Failure detector service for dependable computing},

  booktitle = 	{Proceedings of the 2000 International Conference on Dependable Systems and Networks (ICDSN/FTCS-30)},
  year = 	 {2000},
       PUBLISHER = {IEEE computer society press},
  month = 	 jun,
  pages = 	 {B14--B15},
}

@techreport{DMS94,
author  = {Dolev, Danny and Malki, Dalia and Strong, Ray},
title = {An asynchronous membership protocol that tolerates partitions},
institution = {Institute of Computer Science, The Hebrew University of Jerusalem},
type = {Technical Report},
number = {CS94-6},
year = 1994}

@techreport{DMS95,
author  = {Dolev, Danny and Malki, Dalia and Strong, Ray},
title = {A Framework for Partitionable Membership Service},
institution = {Institute of Computer Science, The Hebrew University of Jerusalem},
type = {Technical Report},
month= mar,
number = "TR 95-4",
year = 1995}



@inproceedings{ DMY94,
  author = "De Prisco, R.and Mayer, A. J. and Yung, M.",
  title = "Time-Optimal Message-Efficient Work Performance in the Presence of Faults (Extended Summary)",
  booktitle = "in Proceedings of the 13th ACM Symp. on Principles of Distributed Computing(PODC94)",
  pages = "161-172",
  year = "1994",

}

@article{G05,
  author    = {Faith Ellen and
               Danny Hendler and
               Nir Shavit},
  title     = {On the Inherent Sequentiality of Concurrent Objects},
  journal   = {SIAM J. Comput.},
  volume    = {41},
  number    = {3},
  year      = {2012},
  pages     = {519-536},
  ee        = {http://dx.doi.org/10.1137/08072646X},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DPLL97,
  year      =   {1997},
   title     =   {Revisiting the {Paxos} Algorithm},
  author    =   {De Prisco, R. and Lampson , B. and Lynch, N. A.},
  booktitle =   {Proceedings of the 11th Workshop on Distributed Algorithms},
  month     =       sep,
  pages     = "11-125",
publisher = springer,
  series =  {LNCS 1320},
 }

@article{DPLL00,
   title     =   {Revisiting the {Paxos} Algorithm},
  author    =   {De Prisco, R. and Lampson , B. and Lynch, N. A.},
 
  Journal = tcs,
  Year = 2000,
  volume = 243,
}

  @techreport{DSS99,
  Author = {Sergent, Nicole and Defago, Xavier and Schiper, Andr\'e},
  Title = "Failure Detectors: implementation issues and impact on consensus performance",
  Institution = epfl,
  month = "?",
  Year = "1999?",
  number = "?"
}



@inproceedings{DLA88,
  crossref = "icdcs88",
  Author = "Dasgupta, Partha and Richard J. LeBlanc and William F. Appelbe",
  Title = "The {Clouds} Distributed Operating System:  A Functional
		Description, Related Work and Implementation Details",
 
   }
@inproceedings{DPMR99,
	crossref = "podc99",
	Author ="De Prisco, Roberto and  Malkhi, Dahlia and Reiter, Michael K.",
	Title =  "On k-set Consensus Problems in Asynchronous Systems",
	pages = "257--265",
}
	
@article{Dol82,
  Author = "Dolev, Danny",
  Title = "The {Byzantine} Generals Strike Again",
  Journal = "Journal of Algorithms",
  Year = 1982,
  volume = 3,
  number = 1,
  pages = "14--30"
  }

@article{DDS87,
  Author = "Dolev, Danny and Cynthia Dwork and Larry Stockmeyer",
  Title = "On the Minimal Synchronism Needed for Distributed Consensus",
  Journal = jacm,
  month = jan,
  Year = 1987,
  volume = 34,
  number = 1,
  pages = "77--97"
  }

@article{DHS86,
  Author = "Dolev, Danny and Joseph Y. Halpern and H. Raymond Strong",
  Title = "On the Possibility and Impossibility of Achieving Clock
		Synchronization",
  Journal = jcss,
  volume = 22,
  number = 2,
  month = apr,
  Year = 1986,
  pages = "230--250"
  }

@inproceedings{DK96,
	crossref = "podc96",
	Author = "Dolev, Danny and Keidar, Idit.",
	Title = "Efficient Message Ordering in Dynamic Networks",
	pages = "68--76"
 
}
@inproceedings{DG02,
  year =        {2002},
   title =       {Fast Indulgent Consensus with Zero Degradation},
  author =      {Partha Dutta and Rachid Guerraoui},
  booktitle =   {Proceedings of the 4th European Dependable Computing
Conference},
confadress= {Toulouse, France},
month= oct,
 
}

@article{DLPSW86,
  Author = "Dolev, D. and N. A. Lynch and S. S. Pinter and
		E. W. Stark and W. E. Weihl",
  Title = "Reaching Approximate Agreement in the Presence of Faults",
  Journal = jacm,
  month = jul,
  Year = 1986,
  volume = 33,
  number = 3,
  pages = "499--516"
  }

@article{DR85,
  Author = {Dolev, Danny and R{\"{u}}diger Reischuk},
  Title = "Bounds on Information Exchange for {Byzantine} Agreement",
  Journal = jacm,
  month = jan,
  Year = 1985,
  volume = 32,
  number = 1,
  pages = "191--204"
  }

@techreport{DRS86,
  Author = {Dolev, Danny and R{\"{u}}diger Reischuk and H. Raymond Strong},
  Title = "Early Stopping in {Byzantine} Agreement",
  Institution = ibmrl,
  month = dec,
  Year = 1986,
  number = "RJ5406"
  }

@article{DRS90,
  Author = {Dolev, Danny and R{\"{u}}diger Reischuk and H. Raymond Strong},
  Title = "Early Stopping in {Byzantine} Agreement",
  Journal = jacm,
  month = oct,
  Year = 1990,
  volume = 37,
  number = 4,
  pages = "720--741"
  }


@article{DS83,
  Author = "Dolev, Danny and H. Raymond Strong",
  Title = "Authenticated Algorithms for {Byzantine} Agreement",
  Journal = sicomp,
  month = nov,
  Year = 1983,
  volume = 12,
  number = 4,
  pages = "656--666"
  }

@phdthesis{Dru86,
  Author = "Drummond, Rog{\'{e}}rio",
  Title = "Impact of Communication Networks on Fault-Tolerant Distributed
		Computing",
  School = cornell,
  month = jun,
  Year = 1986,
  note = "Department of Computer Science Technical Report 86-748"
  }

@techreport{DHPW92,
  Author = {Dwork, Cynthia and Herlihy, Maurice and Plotkin, Serge and
Waarts, Orli},
  Title = {Time-Lapse Snapshots},
  number = {STAN-CS-92-1423},
  Institution = {Department of Computer Science, Stanford University},
  month = apr,
  Year = 1992
  }

@inproceedings{DHW92,
  crossref = "podc92",
  Author = "Dwork, Cynthia and Joseph Y. Halpern and Orli Waarts",
  Title = "Performing Work Efficiently in the Presence of Faults",
  pages = "91--102"
  }
@article{ DHW98,
  author = "Dwork, C. and Halpern, J. Y. and Waarts, O.",
  title = "Performing Work Efficiently in the Presence of Faults",
  journal = "SIAM Journal on Computing",
  volume = "27",
  number = "5",
  pages = "1457--1491",
  year = "1998",
}




@article{DLS88,
  Author = "Dwork, Cynthia and Nancy A. Lynch and Larry Stockmeyer",
  Title = "Consensus in the Presence of Partial Synchrony",
  journal = jacm,
  volume = 35,
  number = 2,
  month = apr,
  year = 1988,
  pages = "288--323"
  }


@article{DM90,
  Author = "Dwork, Cynthia and Yoram Moses",
  Title = "Knowledge and Common Knowledge in a {Byzantine} Environment:
  		Crash Failures",
  Journal = ic,
  volume = 88,
  number = 2,
  month = oct,
  Year = 1990,
  pages = "156--186"
  }
@INPROCEEDINGS{DKM93,
  crossref = "ftcs93",
  AUTHOR = " Danny Dolev and Shlomo Kramer and Dalia Malki",
  Title = "Early Delivery Totally Ordered Multicast in Asynchronous Environments",
 BOOKTITLE = {Proceedings of the 23nd Annual International  Symp. on
              Fault},
  Year = "1993",
  Pages = "544-553",
  }

@article{DM96,
  Author = "Dolev, D. and Lalkihi, D.",
  Title = "The {Transis} approach to high availability cluster communication",
  Journal = cacm,
  month = apr,
  Year = "96",
  volume = 39,
  number = 4,

  }



@InProceedings{DPFLS98,  
	crossref = "podc98",
        author =       "De Prisco, R. and Fekete, A. and Lynch, N. and Shvartsman, A.",
        title =        "A  dynamic view-oriented group communication service",
pages = "227--236",
     }


@InProceedings{DPFLS99,  
	crossref = "disc99",
        author =       "De Prisco, R. and Fekete, A. and Lynch, N. and Shvartsman, A.",
        title =        "A  dynamic primary configuration group communication service",
     }

@inproceedings{DPPU86,
  crossref = "stoc86",
  Author = "Dwork, Cynthia and D. Peleg and N. Pippenger and Eli Upfal",
  Title = "Fault Tolerance in Networks of Bounded Degree",
  pages = "370--379"
  }

@INPROCEEDINGS{DwSk83,
        CROSSREF = "podc83",
        AUTHOR = {Dwork, C. and Skeen, D.},
        TITLE = {The Inherent Cost of Nonblocking Commitment},
        PAGES = {1--11},
       }
@article{DS87,
  Author = "Dolev, D. and  Strong, R.",
  Title = "A Simple Model For Agreement in Distributed Systems",
  booktitle={Fault-Tolerant Distributed Computing},
  pages="42--50",
  Year = 1987,
  editor       = { B. Simons and A. Spector},
  publisher= springer,
  series       = {LNCS 448},
   }


%E

@inproceedings{ESS89,
  crossref= "wdag89",
  Author  = {Schiper, A. and Eggli, J. and Sandoz, A.},
  Title = { A New Algorithm to Implement Causal Ordering},
   pages = "219--232"
  }
%verif
@inproceedings{EMS95,
author  = {Ezhilchelvan, Paul D. and Mac\^edo, Raimundo A. and
Shrivastava, Santosh K.},
title = {Newtop: a fault-tolerant group communication protocol},
booktitle = {Proceedings of the 15th International Conference on
Distributed Computing Systems},
confaddress = {Vancouver, BC, Canada},
month = jun,
year = 1995,
}
@INPROCEEDINGS{Ezh87,
        AUTHOR = {Paul D. Ezhilchelvan},
        TITLE = {Early Stopping algorithms for Distributed agreement under
		fail-stop, omission, and timing fault types},
        BOOKTITLE = {IEEE 1987 Sixth Symp. on Reliability in Distributed
		Software and Database Systems},
        YEAR = {1987},
        PAGES = {201-212},
        PUBLISHER = {IEEE computer society press},
        ADDRESS = {Computing Laboratory, The university, Newcastle upon Tyne,
		England},
}

%F
@techreport{FH86,
  Author = "Fagin, Ronald and Joseph Y. Halpern",
  Title = "Belief, Awareness, and Limited Reasoning",
  Institution = ibmrl,
  month = may,
  date = 23,
  Year = 1986,
  number = "RJ4657",
  note = "Also appears in the 1985 {\em Proceedings of IJCAI}"
  }

@inproceedings{FH87,
  Author = "Fagin, Ronald and Joseph Y. Halpern",
  Title = "I'm {OK} if You're {OK}:  On the Notion of Trusting Communication",
  Booktitle = "Proceedings of the Symp. on Logic in Computer Science",
  month = jun,
  Year = 1987,
  confaddress = "Ithaca, New York",
  pages = "280--292",
  note = "Also appears as IBM Research Laboratory Technical Report RJ5600"
  }


@inproceedings{Fek86,
  crossref = "podc86",
  Author = "Fekete, A. D.",
  Title = "Asymptotically Optimal Algorithms for Approximate Agreement",
  pages = "73--87"
  }


@inproceedings{BenOr83,
  author    = {Michael Ben-Or},
  title     = {Another Advantage of Free Choice: Completely Asynchronous
               Agreement Protocols (Extended Abstract).},
  booktitle = {PODC '83: Proceedings of the annual ACM Symp.
on     Principles of distributed computing},
  year      = {1983},
  pages     = {27-30}
}

@inproceedings{Skeen81,
  author    = {Dale Skeen},
  editor    = {Y. Edmund Lien},
  title     = {Nonblocking Commit Protocols},
  booktitle = {SIGMOD},
  year      = {1981},
  pages     = {133-142}
}


@inproceedings{Fek87,
  crossref = "podc87",
  Author = "Fekete, A. D.",
  Title = "Asynchronous Approximate Agreement",
  pages = "64--76"
  }
  
@article{Fek90,
  Author = "Fekete, Alan D.",
  Title = "Asymptotically Optimal Algorithms for Approximate Agreement",
  Journal = dc,
  Year = 1990,
  volume = 4,
  number = 1,
  pages = "9--30"
  }

@article{Fek94,
  Author = "Fekete, Alan D.",
  Title = "Asynchronous Approximate Agreement",
  Journal = ic,
  Year = 1994,
  pages="95--124",
volume= 115,
number= "1",
month= nov,
  }




@Article{GR04,
  author    = {Rachid Guerraoui and
               Michel Raynal},
  title     = {The Information Structure of Indulgent Consensus.},
  journal   = {IEEE Trans. Computers},
  volume    = {53},
  number    = {4},
  year      = {2004},
  pages     = {453-466},
}

@Article{FLMS93,
        author =       "A. D. Fekete and N. Lynch and Y. Mansour and J. Spinelli",
        title =        "The Impossibility of Implementing Reliable
                       Communication in the Face of Crashes",
        journal =      "Journal of the ACM",
        volume =       "40",
        number =       "5",
        year =         "1993",
        pages =        "1087--1107",
      }
  

@techreport{FM90,
  Author = {Feldman, Paul and Silvio Micali},
  Title = "An Optimal Algorithm for Synchronous {Byzantine} Agreement",
  Institution = mitlcs,
  month = jun,
  Year = 1990,
  number = "MIT/LCS/TM-425"
  }


@inproceedings{HLM03,
  author    = {Maurice Herlihy and
               Victor Luchangco and
               Mark Moir},
  title     = {Obstruction-Free Synchronization: Double-Ended Queues as
               an Example},
  booktitle = {ICDCS},
  year      = {2003},
  pages     = {522-529}
}

@article{AGHK09,
  author    = {Hagit Attiya and
               Rachid Guerraoui and
               Danny Hendler and
               Petr Kuznetsov},
  title     = {The complexity of obstruction-free implementations},
  journal   = {J. ACM},
  volume    = {56},
  number    = {4},
  year      = {2009}
}


@inproceedings{FLMS05,
  author    = "Faith Ellen Fich and
               Victor Luchangco and
               Mark Moir and
               Nir Shavit",
  title     = "Obstruction-Free Algorithms can be Practically Wait-Free",
  booktitle = "Proceedings of the International Symp. on Distributed Computing",
  year      = "2005",
  pages     = "493-494"
}


@inproceedings{MRT04,
  Author = "Moustefaoui, Achour and Raynal, Michel and Travers, Corentin",
  Title = "Crash-Resilient Time-Free Eventual Leadership",
  booktitle = "SRDS' 04: Proceedings of the IEEE International Symp. on Reliable Distributed Systems",
  publisher = "IEEE",
  Year = "2004",
  pages = "208--217"
  }

@inproceedings{Fid90,
  Author  = "Fidge, Colin",
  Title = "A simple run-time concurrency measure",
  booktitle = "The Transputer in Australia",
  editor = "Bossomaier, T. and  Hintz, T and Hulskamp J.",
  publisher = "IOS Press",
  year = 1990,
  pages = "92--101"
  }



@inproceedings{Fid88,
  Author = "Fidge, Colin",
  Title = "Timestamps in Message-Passing Systems that Preserve the Partial
		Ordering",
  booktitle = "Proceedings of the 11th Australian Computer Science
		Conference",
  mon = Feb,
  Year = 1988,
  address = "University of Queensland, Australia"
  }

@techreport{Fis83,
  Author = "Fischer, Michael J.",
  Title = "The Consensus Problem in Unreliable Distributed Systems
		(a Brief Survey)",
  institution = yalecs,
  month = jun,
  Year = 1983,
  number = 273
  }

@inproceedings{FC96,
  Author  = "Christof Fetzer and Flaviu Christian",
  Title = "Fail-Aware Failure Detectors",
  crossref= "srds96",
  pages = "200--209",
  }
@inproceedings{F99,
  Author  = "Christof Fetzer",
  Title = "A Comparaison of Timed Asynchronous Systems and asynchronous Systems with Failure Detectors",
  booktitle="Proceedings of ERSADS99",
  pages = "200--209",
year = 1999,
  }


@inproceedings{FIMR98,
  year =        {1998},
  confaddress =     {West Lafayette, Indiana},
  pages =       {578-585},
  title =       {Fault-tolerant total order multicast to asynchronous groups},
  author =      {U. Fritzke and Ph. Ingels and A. Most\'efaoui and M. Raynal},
  booktitle =   {Proceedings of the 17th IEEE Symp. on Reliable Distributed Systems},
  month =       Oct
,
}

@incollection{FS86,
  Author = "Shavit, N. and Francez, N.",
  Title = "A new approach to the detection of locally indicative stability",
  booktitle = proc # " Thirteenth " # icalp,
  pages = "344--358",
  Volume = "226",
  publisher = springer,
  series = lncs,
  Year = 1986
  }
@article{FL82,
  Author = "Fischer, Michael J. and Nancy A. Lynch",
  Title = "A Lower Bound for the Time to Assure Interactive Consistency",
  Journal = ipl,
  Year = 1982,
  volume = 14,
  pages = "183--186"
  }

@article{FLM86,
  Author = "Fischer, Michael J. and Nancy A. Lynch and Michael Merritt",
  Title = "Easy Impossibility Proofs for Distributed Consensus Problems",
  Journal = dc,
  month = jan,
  Year = 1986,
  volume = 1,
  pages = "26--39"
  }

@article{FLP85,
  Author = "Fischer, Michael J. and Nancy A. Lynch and Michael S. Paterson",
  Title = "Impossibility of Distributed Consensus with one Faulty Process",
  Journal = jacm,
  volume = 32,
  number = 2,
  month = apr,
  Year = 1985,
  pages = "374--382"
  }
@InProceedings{FLS97,  
        author =       "Fekete, A. and Lynch, N. and Shvartsman, A.",
        title =        "Specifying and using a partionable group communication service",
        booktitle =    proc # " 16th " # podc,
        pages =        "53--62", 
        year =         "1997",
        month =         aug,
        confaddress = 	"Toronto, Ontario, Canada",        
}

@techreport{FRT00, 
author = "C. Fetzer and M. Raynal and F. Tronel", 
title = "A Failure Detection Protocol Based on a Lazy Approach", 
institution = "IRISA", 
year = 2000, 
month = nov, 
number = 1367, 
type = "Research Report"
} 

@InProceedings{FRT01, 
author = "C. Fetzer and M. Raynal and F. Tronel", 
title = "A Failure Detection Protocol Based on a Lazy Approach",
booktitle = "IEEE 8th Pacific Rim Symp. on Dependable Computing",
year = 2001, 
pages = "146-153"
} 



@InProceedings{F01,  
        crossref = "icdcs01"  ,
        author =       "Christof Fetzer",
        title =        "Enforcing Perfect  Failure Detection",
        pages =        "350--357", 
        
   }
@techreport{FvR95,
Author ={ Roy Friedman and Robbert van Renesse},
Title={Strong and Weak Virtual Synchrony in {Horus}}, 
Institution = cornellcs,
   number = "95-1537",
month= aug,
year="1995",
}

@INPROCEEDINGS{GMS89,
CROSSREF = "icdcs89",
	AUTHOR = {Hector Garcia-Molina and Annemarie Spauster},
	TITLE = {Message Ordering in a Multicast Environment},
	
	PAGES = {354--361},
	
}
@Article{GMS91,
	AUTHOR = {Hector Garcia-Molina and Annemarie Spauster},
title = "Reliable and Reliable Multicast Communication",
  journal = 	 tocs,
  year = 	 {91},
  volume = 	 {9},
  number = 	 {3},
  pages = 	 {242-271},
  month = 	 aug,
 }                                                                                  

@inproceedings{GRH06,
  author    = {Eli Gafni and
               Sergio Rajsbaum and
               Maurice Herlihy},
  title     = {Subconsensus Tasks: Renaming Is Weaker Than Set Agreement.},
  booktitle = disc,
  year      = {2006},
  pages     = {329-338}
}


%G
@InProceedings{GA88,  
        author =       "Eli Gafni and Yehuda Afek",
        title =        "End-to-End Communication in Unreliable Networks",
        booktitle =    proc # " Seventh " # podc,
        pages =        "131--148", 
        year =         "1988",
        month =        aug,
        address = 	"Toronto, Ontario, Canada",        
}

@InProceedings{GL00,  
        author =       "Eli Gafni and Leslie Lamport",
        title =        "Disk Paxos",
        booktitle    = proc # " 14th International Symp. on Distributed Computing",
        year         = 2000,
        place        = "Toledo ,Spain",
        publisher    = springer,
        series       = {LNCS 1914},
        pages="330--344",
     }

	
  
@InProceedings{GG98,  
        crossref= "icdcs98",
        author =       "Gouda, M.G. and Mc Guire, T. M.",
        title =        "Accelerated heartbeat protocols",
              pages =        "", 
}
@article{GS91,
  Author = {Garcia-Molina, Hector and Annemarie Spauster},
  Title = "Ordered and Reliable Multicast Communication",
  Journal = tocs,
  month = aug,
  Year = 1991,
  volume = 9,
  number = 3,
  pages = "242--271"
  }

@article{GHS83,
  Author = " Gallager, R. G. and Humblet, P. A. and Spira, P. M.",
  Title = "A distributed algorithm for minimum-weight spanning trees",
  Journal = toplas,
  month = jan,
  Year = 1983,
  volume = 5,
  number = 1,
  pages = "66--77"
  }
@incollection{Gri90,
  Author = "Gribomont, E.P.",
  Title = "From Synchronous to Asynchronous Communication",
  Booktitle = "Specification and Verification of Concurrent Systems",
  publisher = springer,
  editor = "Rattray, C.",
  Year = 1990,
  pages = "368--383"
  }
@inproceedings{GRS98,
  Author = "Rodrigues, L. and Guerraoui, R. and Schiper, A.", 
  title = {Scalable Atomic Multicast},
  booktitle = {IEEE International Conference Computer Communication and Networks(IC3N'98)},
 year = 1998,
place=Louisiana,
   }

@Article{GL90,
  author = 	 { S.W. Luan and V.D.Gligor},
  title = 	 {A fault tolerant protocole for atomic broadcast },
  journal = 	 {IEEE Transactions on Parallel and Distribued Systems },
  year = 	 {90},
  volume = 	 {1},
  number = 	 {3},
  pages = 	 {271-285},
  month = 	 jul,
 }
@InProceedings{GHM89,
        author =       "O. Goldreich and A. Herzberg and Y. Mansour",
        title =        "Source to Destination Communication in the Presence of
                       Faults",
        booktitle =    "Proceedings of the 8th ACM Symp. on Principles of
                       Distributed Computing (PODC)",
        pages =        "85--102",
        publisher =    "ACM Press , New York, NY , USA",
        address =      "Edmonton, AL CDN",
        year =         "1989",
      }
		  

@INPROCEEDINGS{GSTC90,
        crossref = " podc90",
	AUTHOR = {Gopal, Ajei and Strong, Ray and Toueg, Sam and Cristian, Flaviu},
       	TITLE = {Early-Delivery Atomic Broadcast},
	PAGES = {297--310}
}

@techreport{GT91a,
  Author = "Gopal, Ajei and Sam Toueg",
  Title = "Fault-Tolerant Broadcasts and Multicasts.
	The Problem of Inconsistency and Contamination.
	Part 1: Specifications",
  Institution = cornellcs,
  month = feb,
  Year = 1991,
  number = "91-1189"
  }


@incollection{GT89,
  crossref = "wdag89",
  Author = "Gopal, Ajei and Sam Toueg",
  Title = "Reliable Broadcast in Synchronous and Asynchronous
		Environments (Preliminary Version)",
  pages = "110--123",
  }

@inproceedings{GT91b,
  crossref = "podc91",
  Author = "Gopal, Ajei and Sam Toueg",
  Title = "Inconsistency and Contamination",
  pages = "257--272",
 
  }
@inproceedings{Gue95,
  crossref = "wdag95",
  title =       {Revisiting the relation between non-blocking atommic 
                 commitment and consensus},
  author =      {Rachid Guerraoui },
}

@inproceedings{FSS05,
  author    = "Christof Fetzer and
               Ulrich Schmid and
               Martin Susskraut",
  title     = "On the Possibility of Consensus in Asynchronous Systems
               with Finite Average Response Times",
  booktitle = "International Conference on Distributed Computing Systems",
  publisher = "ieee",
  year      = "2005",
  pages     = "271-280"
}


@inproceedings{GLS95,
  crossref= "srds95",
   title =       {Non Blocking Atomic Commitment with an Unreliable Failure Detector},
  author =      {Rachid Guerraoui and Mikel Larrea and {Andr} Schiper},

}
@inproceedings{GS95,
  year =        {1995},
   title =       {The decentralized Non blocking AtomicCommitment},
  author =      {Rachid Guerraoui and {Andr\'e} Schiper},
  booktitle =   {Proceedings of the 7th IEEE Symp. on Parallel and Distributed Processing},
 
}
@inproceedings{GS96,
  crossref = "wdag96",
  title =      " {$\Gamma$-Accurate} Failure Detectors.",
  author =      {Rachid  Guerraoui and {Andr\'e} Schiper},
}

@inproceedings{GS97,
  year =        {1997},
  address =     {Saarbr\"ucken, Germany},
  title =       {Genuine Atomic Multicast},
  author =      {Rachid Guerraoui and {Andr\'e} Schiper},
  booktitle =   {Proceedings of the 11th International Workshop on Distributed Algorithms },
  keywords =    {IMPORTANT; FT_principles},
  month =       sep,
  series =  {LNCS 1320},
publisher = springer,
}

@inproceedings{GS97f,
  crossref= "icdcs97",
  pages =       {578-585},
  title =       {Total order multicast to multiple groups},
  author =      {Rachid Guerraoui and {Andr} Schiper},
  
}

@article{Gue01,
  Author = "Guerraoui, Rachid ",
  Title = "On the Hardness of Failure Sensitive Agreement Problems",
  Journal = ipl,
  Year = 2001,
  volume = "79 ",
  } 


@Unpublished{GK09,
  author = 	 {Eli Gafni and Petr Kuznetsov},
  title = 	 {The Weakest Failure Detector for Solving $k$-Set Agreement},
  note =         {In submission}, 
  month = 	 {February},
  year = 	 {2009}
}

@inproceedings{GK09-wfd,
  author    = {Eli Gafni and
               Petr Kuznetsov},
  title     = {The weakest failure detector for solving k-set agreement},
  booktitle = {PODC},
  year      = {2009},
  pages     = {83-91}
}



@inproceedings{GK09-setcon,
  author    = {Eli Gafni and
               Petr Kuznetsov},
  title     = {On Set Consensus Numbers},
  booktitle = {DISC},
  year      = {2009},
  pages     = {35-47}
}



@Unpublished{Gaf08-concurrency,
  author = 	 {Eli Gafni},
  title = 	 {Free-for-All Execution: Unifying Resiliency, Set-Consensus, and Concurrency},
  note =         {Unpublished manuscript}, 
  month = 	 {February},
  year = 	 {2008}
}


@Unpublished{Gaf08-EBG,
  author = 	 {Eli Gafni},
  title = 	 {{The extended {BG}-Simulation}},
  note =         {Unpublished manuscript},
  month = 	 {May},
  year = 	 {2008}
}

@inproceedings{Gaf09-EBG,
  author    = {Eli Gafni},
  title     = {The extended {BG}-simulation and the characterization of t-resiliency},
  booktitle = {STOC},
  year      = {2009},
  pages     = {85-92}
}



@article{Gue02,
  author    = {Rachid Guerraoui},
  title     = {Non-blocking atomic commit in asynchronous distributed systems
               with failure detectors.},
  journal   = {Distributed Computing},
  volume    = {15},
  number    = {1},
  year      = {2002},
  pages     = {17-25},
}


@phdthesis{Go92,
  Author = "Gopal, A.",
  Title = "Fault-Tolerant Broadcasts and Multicasts: The Problem of Inconsistency and Contamination",
  School = cornell,
  month = jan,
  Year = 1992
  }

%H
@techreport{Had83,
  Author = "Hadzilacos, Vassos",
  Title = "Byzantine Agreement Under Restricted Types of Failures
		(Not Telling the Truth is Different from Telling Lies)",
  Institution = "Department of Computer Science, Harvard University",
  Year = 1983,
  number = "18-83",
  note = "A revised version appears in Hadzilacos's
		Ph.D.\ dissertation~\cite{Had84}"
  }
@article{Had87,
  Author = "Hadzilacos, Vassos",
  Title = "On the relationship between the atommic commitment and 
            consensus problems",
  Journal = {Fault-Tolerant Distributed Computing},
  pages="201--208",
  Year = {1987},
  Editor   = { B. Simons and A. Spector},
  Publisher= springer,
  Series   = {LNCS 448},
  }


@misc{H02,
  author       = "Hadzilacos, Vassos",
  year = 2002,
  note = "Comparison between {$\Diamond S$} and {$\Diamond P$}, personal communication",
}

@misc{Ray07,
  author       = "Michel Raynal",
  year = 2007,
  title = {{$K$-anti-Omega}},
  note = {Rump session at PODC 2007},
  month = {August}
}


@inproceedings{RT06,
  author    = {Michel Raynal and
               Corentin Travers},
  title     = {In Search of the Holy Grail: Looking for the Weakest Failure
               Detector for Wait-Free Set Agreement},
  booktitle = {OPODIS},
  year      = {2006},
  pages     = {3-19}
}

@inproceedings{CZCL07,
  author    = {Wei Chen and
               Jialin Zhang and
               Yu Chen and
               Xuezheng Liu},
  title     = {Weakening Failure Detectors for {\it } -Set Agreement
               Via the Partition Approach},
  booktitle = {DISC},
  year      = {2007},
  pages     = {123-138}
}

@inproceedings{AGRRT06,
  author    = {Yehuda Afek and
               Eli Gafni and
               Sergio Rajsbaum and
               Michel Raynal and
               Corentin Travers},
  title     = {Simultaneous Consensus Tasks: A Tighter Characterization
               of Set-Consensus},
  booktitle = {ICDCN},
  year      = {2006},
  pages     = {331-341}
}

@article{Her91,
  title={Wait-free synchronization},
  author={Herlihy, Maurice},
  journal={ACM Transactions on Programming Languages and Systems},
  volume={13},
  number={1},
  pages={124--149},
  year={1991},
  publisher={ACM New York, NY, USA}
}

@inproceedings{HR97,
  author    = {Maurice Herlihy and
               Sergio Rajsbaum},
  title     = {The Decidability of Distributed Decision Tasks (Extended
               Abstract)},
  booktitle = {STOC},
  year      = {1997},
  pages     = {589-598}
}


@article{HW90,
author="Maurice Herlihy and  Jeannette M. Wing",
title="Linearizability: A Correctness Condition for Concurrent Objects",
journal=" ACM Trans. Program. Lang. Syst.",
volume= 12,
number=3,
pages="463--492",
year= 1990
}

@inproceedings{GHW11,
 author = {Golab, Wojciech and Higham, Lisa and Woelfel, Philipp},
 title = {Linearizable implementations do not suffice for randomized distributed computation},
 booktitle = {Proceedings of the 43rd annual ACM Symp. on Theory of computing},
 series = {STOC '11},
 year = {2011},
 pages = {373--382},
 numpages = {10}
} 

@inproceedings{AFHHT07,
  author    = {Marcos Kawazoe Aguilera and
               Svend Fr{\o}lund and
               Vassos Hadzilacos and
               Stephanie Lorraine Horn and
               Sam Toueg},
  title     = {Abortable and query-abortable objects and their efficient
               implementation},
  booktitle = {PODC},
  year      = {2007},
  pages     = {23-32}
}



@TechReport{AF03,
  author = 	 {Aguilera, Marcos K. and Frolund, Svend},
  title = 	 {Strict Linearizability and the Power of Aborting},
  institution =  {HP Laboratories Palo Alto},
  year = 	 {2003},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTnumber = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}


@inproceedings{HS95,
author  = {Hiltunen, Matti A. and Schlichting, Richard D.},
title = {Properties of membership services},
booktitle = {Proceedings of the 2nd International Symp. on
				  Autonomous Decentralized Systems},
address = {Phoenix, AZ},
month = apr,
year = 1995}

@phdthesis{Had84,
  Author = "Hadzilacos, Vassos",
  Title = "Issues of Fault Tolerance in Concurrent Computations",
  School = "Harvard University",
  month = jun,
  Year = 1984,
  note = "Department of Computer Science Technical Report 11-84"
  }
 

 
@article{Had87a,
  Author = "Hadzilacos, Vassos",
  Title = "Connectivity Requirements for {Byzantine} Agreement
		under Restricted Types of Failures",
  Journal = dc,
  volume = 2,
  number = 2,
  Year = 1987,
  pages = "95--103"
  }

}

@article{HH93,
  Author = "Hadzilacos, Vassos and Joseph Y. Halpern",
  Title = "Message and Bit-Optimal Protocol for {Byzantine} Agreement",
  Journal = mst,
  Year = 1993,
  Volume = 26,
  Number = 1,
  pages = "41--102"
}

@book{HJT99,
  Author = "Hadzilacos, Vassos and Prasad Jayanti and Sam Toueg",
  Title = "Fundamentals of Fault-Tolerant Distributed Computing",
  Note = "Forthcoming"
  }




@inproceedings{HMW90,
  crossref = "podc90",
  Author = "Halpern, Joseph Y. and Yoram Moses and Orli Waarts",
  Title = "A Characterization of Eventual {Byzantine} Agreement",
  pages = "333--346"
  }


@inproceedings{HS93,
  
  Author = {Maurice Herlihy and Nir Shavit},
  Title = "The Asynchronous Computability Theorem for $t$-Resilient Tasks",
  pages = "111--120",
  booktitle = proc # " 25th " # stoc,
  month = may,
  Year = 1993,
  confaddress = "San Diego, California",
  confeditor = "Alok Aggrawal",
   }
 @inproceedings{HR94,
  
  Author = {Herlihy, Maurice and Rajsbaum, Sergio},
  Title = "Set consensus using arbitrary objects",
    booktitle = proc # " 13th" # podc,
  month = aug,
  Year = 1994,
 pages = "324--333",
  }
   

@inproceedings{HSSD84,
  crossref = "podc84",
  Author = "Halpern, Joseph Y. and Barbara Simons and Ray Strong
			and Danny Dolev",
  Title = "Fault-Tolerant Clock Synchronization",
  pages = "89--102"
  }
    


@incollection{HT93,
  Author = "Hadzilacos, Vassos and Toueg, Sam",
  Title = "Fault-tolerant broadcasts and related problems",
  Editor = "Mullender, Sape J.",
  booktitle = "Distributed Systems",
  Publisher = "Addison-Wesley",
  Year = "1993",
  Chapter = 5,
  Pages = {97--145}
  }

@techreport{HT94,
        author = "Hadzilacos, V. and Toueg, S.",
        title = "A modular approach to
        	fault-tolerant broadcasts and related problems",
	institution = cornellcs,
        number = "TR 94-1425",
        year = "1994",
	month = may,
     
}





@inproceedings{HV86,
  crossref = "stoc86",
  Author = "Halpern, Joseph Y. and Moshe Y. Vardi",
  Title = "The Complexity of Reasoning about Knowledge and Time:
		Extended Abstract",
  pages = "304--315",
  note = "A revised version appears as IBM Research Laboratory
Technical Report RJ5764"
  }

@techreport{HV87,
  Author = "Halpern, Joseph Y. and Moshe Y. Vardi",
  Title = "The Complexity of Reasoning about Knowledge and Time, {I}:
		Lower Bounds",
  month = aug,
  Institution = ibmrl,
  Year = 1987,
  Number = "RJ5764"
  }
 

@inproceedings{HLvR99,
author = { Jason Hickey and Nancy Lynch and Robbert van Renesse},
title ={Specifications and proofs for ensemble layers},
 booktitle = proc # " Fifth" # "International Conference on Tools and Algorithms for the Construction and Analysis of Systems",
  confaddress = "Amsterdam, Netherlands",
  series = lncs,
  month = mar,
  Year = 1999,
  publisher = springer,
}


@inproceedings{SB05,
  Author = "Livia Sampaio and Francisco Brasileiro",
  Title = "Adaptive Indulgent Consensus",
 booktitle = proc # " International Conference on Dependable Systems and Networks (DSN)",
  pages = "422-431",
  Year = "2005",
  publisher = ieee,
  }


@inproceedings{T07,
  Author = "Gadi Taubenfeld",
  Title = "Computing in the Presence of Timing Failures",
 booktitle = proc # "IEEE International Conference on Distributed Computing Systems (IDCS)",
  Year = "2007",
  publisher = ieee,
  }


@inproceedings{VR02,
  Author = "Pedro Vicente and Luis Rodrigues",
  Title = "An indulgent uniform total order broadcast algorithm with optimistic delivery",
  booktitle = proc # "IEEE International Symp. on Reliable Distributed Systems (SRDS)",
  pages = "92-80",
  Year = "2002",
  publisher = ieee,
  }



@inproceedings{HZ87,
  crossref = "podc87",
  Author = "Halpern, Joseph Y. and Lenore D. Zuck",
  Title = "A Little Knowledge Goes a Long Way:
	Simple Knowledge-Based Derivations and Correctness Proofs
	for a Family of Protocols",
  pages = "269--280",
  note = "A revised version appears as IBM Research Laboratory Technical
		Report RJ5857"
  }

@techreport{HW86,
  Author = "Herlihy, Maurice P. and Jeannette M. Wing",
  Title = "Axioms for Concurrent Objects",
  Institution = "Department of Computer Science, Carnegie-Mellon University",
  month = oct,
  Year = 1986,
  number = "86-154"
  }

@inproceedings{HLvR99,
author = { Jason Hickey and Nancy Lynch and Robbert van Renesse},
title ={Specifications and proofs for ensemble layers},
 booktitle = proc # " Fifth" # "International Conference on Tools and Algorithms for the Construction and Analysis of Systems",
  confaddress = "Amsterdam, Netherlands",
  series = lncs,
  month = mar,
  Year = 1999,
  publisher = springer,
}

@techreport{HA89,
  Author = "Hutto, Phillip W. and Mustaque Ahamad",
  Title = "Slow Memory:  Weakening Consistency to Enhance Concurrency
		in Distributed Shared Memories",
  Institution = gitics,
  month = oct,
  Year = 1989,
  number = "89/39"
  }

@inproceedings{HA90,
  crossref = "icdcs90",
  Author = "Hutto, Phillip W. and Mustaque Ahamad",
  Title = "Slow Memory:  Weakening Consistency to Enhance Concurrency
		in Distributed Shared Memories",
 
  }



@techReport{HHMRT99,
   author =      {Helary, Jean-Michel and Hurfin M. and Mostefaoui Achour and 
                  Raynal, Michel and Tronel,F},
   title =       {Computing Global Functions in Asynchrous Distributed 
                  Systems with crashes},
   institution = {IRISA and accepte a ICDCS2000},
   address = "Campus Universitaire de Beaulieu, Rennes",
   year =        "1999",
   number = "1243",
   
}

@techReport{HMR98,
   author =      {Hurfin, Michel and Mostefaoui Achour and 
                  Raynal, Michel },
   title =       {Consensus in asynchronous systems where processe can crash and recover},
   crossref =" srds98",

   pages= "280--286",
   
}

@article{HR99,
   author =      {Hurfin, Michel and 
                  Raynal, Michel },
   title =       {A simple and fast asynchronous consensus based on a weak failure detector},
  
journal= dc,
volume =12,
number =4,
year=1999,
 }	

@article{IL93,
author={ A. Israeli and M. Li},
title={Bounded time-stamps},
journal=dc,
volume= 6,
number=4,
month=jul,
year="1993",
}

%J
@Article{J95,
  author = 	 {X. Jia},
  title = 	 {A Total Ordering Multicast Protocol Using Propagations trees},
  journal = 	 {IEEE Transactions on Parallel and Distributed Systems },
  year = 	 {95},
  volume = 	 {6},
  number = 	 {6},
  pages = 	 {617-627},
  month = 	 jun,
 }

@Article{Jay97,
  author = 	 {Prasad Jayanti},
  title = 	 {Robust wait-free hierarchies},
  journal = 	 {Journal of the ACM},
  year = 	 {1997},
  volume = 	 {44},
  number = 	 {4},
  pages = 	 {592-614}
}


@inproceedings{JV96,
	crossref = "podc96",
	Author = "Jayaram, M. and Varghese, G.",
	Title = "Crash Failures can Drive Protocols to Arbitrary States",
	pages = "247--256"
}


@inproceedings{JFR93,
    author  = {Jahanian, Farnam and Fakhouri, Sameh and Rajkumar, Ragunathan},
    title = {Processor group membership protocols: 
            specification, design and implementation},
    booktitle = {Proceeding of the Twelfth IEEE Symp. on Reliable
				  Distributed Systems},
    pages = {2--11},
   address = {Princeton},
   month = oct,
   year = 1993
}



@article{Jef85,
  Author = "Jefferson, David R.",
  Title = "Virtual Time",
  Journal = toplas,
  month = jul,
  Year = 1985,
  volume = 7,
  number = 3,
  pages = "404--425"
  }
%K

@techreport{KK99,
author = {Idit Keidar and Roger Khazan},
title= {A client-server approach to virtually synchronous group multicast: Specifications and Algorithms},
 Institution = mitlcs ,
  Year = 1999,
  number = "",
   }

@techreport{KSMD00R,
author = {Idit Keidar and Jeremy Sussman and Keith Marzull and Danny Dolev},
title= {Moshe: A Group Membership Service for WANs.},
 Institution = mitlcs ,
  Year = 2000,
  number = "MIT-LCS-TM-593a",
   }    
@inproceedings{KSMD00,
  crossref= "icdcs00",
author = {Idit Keidar and Jeremy Sussman and  Keith Marzullo and Danny Dolev},       
title = {      A Client-Server Oriented Algorithm for Virtually Synchronous Group Membership in WANs.},
     pages = {356--365},
}
      
@article{KR01,
 author = {Idit Keidar and Sergio Rajsbaum},       
title = {On the cost of Fault-Tolerant Consensus when There Are No Faults-A tutorial},
     pages = {45--63},
journal ="SIGACT News",
volume = 32,
number=2,
editor="Distributed Computing column",
month = jun,
year = "2001",
}

  @techreport{KR01a,
 author = {Idit Keidar and Sergio Rajsbaum},       
title = {On the cost of Fault-Tolerant Consensus when There Are No Faults-A tutorial},
     pages = {45--63},
 Month = may,
  Year = 2001,
institution = mitlcs ,
type = {Technical Report},
  number = "MIT-LCS-TR-821"
    }
@inproceedings{KR02,
 author = {Idit Keidar and Sergio Rajsbaum},       
title = {On the cost of Fault-Tolerant Consensus when There Are No Faults-A tutorial},
 booktitle   = "Tutorial  21th " # podc,
  month = jul,
  Year = 2002,
  confaddress = "Monterey, California"
  }

    
 
@inproceedings{KK00, 
crossref= "icdcs00",
author= {Idit Keidar and Roger Khazan},
title = {       A Client-Server Approach to Virtually Synchronous 
        Group Multicast: Specifications and Algorithms},
pages = {344--355},
} 

@article{KR81,
author={Kung, H. T. and Robinson, J. T. },
title={An optimistic methos for concurrency control},
journal={ACM Transaction on Darabase Systems},
year= 1981,
month= jun,
number=2,
volume=6,
pages="213--226",
}

@techreport{VKCD99,
author ={ Roman Vitenberg and Idit Keidar and Gregory V. Chockler and  Danny Dolev},
title= {Group Communication Specifications: A Comprehensive Study.},
  
  Month = sep,
  Year = 1999,
  number = "MIT-LCS-TR-790",
notes= "ACM Computing surveys.To appear."
    }


@inproceedings{KT91,
  crossref= "icdcs91",
  author  = {Kaashoek, M. Frans and Tanenbaum, Andrew S.},
  title = {Group communication in the {Amoeba} distributed operating system},
   pages = {222--230},
 }

@inproceedings{KT96,
  crossref = "icdcs96",
  author  = {Kaashoek, M. Frans and Tanenbaum, Andrew S.},
  title = {An Evaluation of the {Amoaba} Group Communication System},
  pages = {436--447},
}

@PhDthesis{Ka92,
  Author = "Kaashoek, M. Frans",
  Title = "Group Communication in Distributed Computer Systems",
  School = "Vrije Universiteit",
  month = dec,
  Year = 1992
}

@ARTICLE{KT88,
	AUTHOR = {Koo, Richard and Toueg, Sam},
	TITLE = {Effects of Message Loss on the Termination of Distributed
		Protocols},
	JOURNAL = ipl,
	YEAR = {1988},
	VOLUME = {27},
	NUMBER = {4},
	PAGES = {181--188},
	MONTH = apr
}

@article{KO87,
  Author = "Kopetz, Hermann and Wilhelm Ochsenreiter",
  Title = "Clock Synchronization in Distributed Real-Time Systems",
  Journal = ieeetc,
  month = aug,
  Year = 1987,
  volume = "C-36",
  number = 8,
  pages = "933--940"
  }
%L
@article{L01,
author = {Leslie Lamport},       
title = {Paxos Made Simple},
     pages = {18--25},
journal ="SIGACT News",
volume = 32,
number=4,
editor="Distributed Computing column",
month = dec,
year = "2001",
}

@article{Lam77,
author = {Leslie Lamport},       
title = {Proving the correctness of multiprocessor programs},
     pages = {125--143},
journal ="Transactions on software engineering",
volume = 3,
number = 2,
editor="IEEE",
month = mar,
year = "1977",
}


 @Article{LA87,
  author = 	 {Loui, M.C. and Abu-Amara, H.H.},
  title = 	 {Memory requirements for agreement among unreliable asynchronous processes},
 journal = 	 {Advances in Computing Research},
  year = 	 {1987},
  volume = 	 {4},
  pages = 	 {163--183},
 
 }





@inproceedings{LAF99,
  year =        {1999},
  confaddress =     {Bratislava},
  title =       {Efficient Algorithms to Implement Unreliable Failure Detectors in Partially Synchronous Systems },
  author =      {Larrea, M. and Ar\'evalo, S. and Fern\'andez, A.},
  booktitle =   {Proceedings of the 13th International Symp. on Distributed Algorithms},
  month =       sep,
  pages = "34-48",
series = {LNCS 1693},
}

@inproceedings{LFA00,
  year =        {2000},
  address =     {Toledo},
  title =       {Eventually Consistent Failure Detectors},
  author =      { Larrea, M.  and Fern\'andez, A. and Ar\'evalo, S. },
  booktitle =   { Brief Annoucement  the 14th International Symp. on Distributed Algorithms},
  month =       oct,
}

@inproceedings{LFA00b,
  crossref = "srds00",
   title =       {Optimal Implementation of the Weakest Failure Detector for Solving Consensus},
  author =      "Larrea, M.  and Fern\'andez, A. and Ar\'evalo, S. ",
    pages = "52-59",
}



@inproceedings{ LFA01,
    author = "Mikel Larrea and Antonio Fernandez and Sergio Arevalo",
    title = "Eventually consistent failure detectors",
    booktitle = "{ACM} Symp. on Parallel Algorithms and Architectures",
    pages = "326-327",
    year = "2001" }










@inproceedings{ LO88,

  author = "Oki, B. M. and Liskov, B.",
  title = "Viewstamped Replication: A General Primary Copy",
  booktitle = "Proceedings of the 7th ACM Symp. on Principles of Distributed Computing(PODC 88)",
  pages = "8-17",
  year = "1988",
  address = "Toronto",
  month = aug,

}













@techreport{LT88,
author  = {Lynch, Nancy A. and Tuttle Mark R.},
title = {An Introduction to input/output automata},
institution = mitlcs ,
type = {Technical Report},
number = {MIT/LCS/TM-373},
year = 1988}

@article{Lam94,
  Author = "Lamport, Leslie",
  Title = "The temporal logic of actions",
  Journal = toplas,
  month = may,
  Year = 1994,
  volume = 16,
  number = 3,
  pages = "872--923"
  }
@article{Lam98,
  Author = "Lamport, Leslie",
  Title = "The {Part-Time} Parliament",
  Journal = "ACM Transactions on Computer Systems",
  Volume = " 16 ",
  Number = 2,
  Pages = "133-169",
  year = 1998,
month= may,
}

@INPROCEEDINGS{LLS90,
	crossref = "podc90",
	AUTHOR = {Ladin, Rivka and Liskov, Barbara and Shrira, Liuba},
	TITLE = {Lazy replication: Exploiting the semantics of Distributed
		Services},
	PAGES = {43--58}
}

@article{Lam78a,
  Author = "Lamport, Leslie",
  Title = "Time, Clocks, and the Ordering of Events in a Distributed System",
  Journal = cacm,
  month = jul,
  Year = 1978,
  volume = 21,
  number = 7,
  pages = "558--565"
  }

@ARTICLE{Lam78b,
	AUTHOR = {Lamport, Leslie},
	TITLE = {The Implementation of Reliable Distributed Multiprocess
		Systems},
	JOURNAL = {Computer Networks},
	YEAR = {1978},
	VOLUME = {2},
	PAGES = {95--114}
}

@article{Lam79,
  Author = "Lamport, Leslie",
  Title = "How to Make a Multiprocessor Computer that Correctly Executes
		Multiprocess Programs",
  Journal = ieeetc,
  month = sep,
  Year = 1979,
  volume = "C-28",
  number = 9,
  pages = "690--691"
  }

@InProceedings{Lam83,
  author =      "Lamport, L.",
  title =       "What good is temporal logic?",
  pages =       "657--668",
  booktitle =   "Information Processing 83: proceedings of the IFIP Ninth
                 World Congress",
  month = sep,
  Year = 1983,
  confaddress = "Paris",
  publisher = "IFIP, North-Holland",
  editor = "R. E. A. Mason",
  
}



@article{Lam84,
  Author = "Lamport, Leslie",
  Title = "Using Time Instead of Timeout for Fault-Tolerant
		Distributed Systems",
  Journal = toplas,
  month = apr,
  Year = 1984,
  volume = 6,
  number = 2,
  pages = "254--280"
  }

@article{Lam86a,
  Author = "Lamport, Leslie",
  Title = "On Interprocess Communication; Part {I}:  Basic Formalism",
  Journal = dc,
  volume = 1,
  number = 2,
  pages = "77--85",
  Year = 1986
  }

@article{Lam86b,
  Author = "Lamport, Leslie",
  Title = "On Interprocess Communication; Part {II}:  Algorithms",
  Journal = dc,
  volume = 1,
  number = 2,
  pages = "86--101",
  Year = 1986
  }

@article{Lam86,
  Author = "Lamport, Leslie",
  Title = "On Interprocess Communication; Part {I} and {II}",
  Journal = dc,
  volume = 1,
  number = 2,
  pages = "77--101",
  Year = 1986
  }


@incollection{Lam87,
  Author = "Lamport, Leslie",
  Title = "A Formal Basis for the Specification of Concurrent Systems",
  booktitle = "Distributed Operating Systems.  Theory and Practice",
  series = "NATO Advanced Study Institute Series",
  Year = 1987,
  volume = "F28",
  editor = "Y. Paker et al.",
  publisher =  springer,
  pages = "3--47"
  }

@techreport{Lam88,
  Author = "Lamport, Leslie",
  Title = "A Theorem on Atomicity in Distributed Algorithms",
  Institution = "DEC Systems Research Center",
  month = may,
  Year = 1988,
  Number = 28
  }
@InProceedings{LeL77,
  author =      "Le Lann, G.",
  title =       "Distributed Systems--towards a formal approach",
  pages =       "155--160",
  booktitle =   "Information Processing 77: proceedings of the IFIP
                 Congress",
  month = aug,
  Year = 1977,
  confaddress = "Toronto",
  publisher = "IFIP, North-Holland",
  editor = "R. E. A. Mason",
  
}
@InProceedings{LeL98,
  author =      "Le Lann, G.",
  title =       "Proof-based system engeneering and embedded systems",
  pages =       "208--248",
  booktitle =   "Proceedings of the european School on embedded Systems, nov 96 ",
  month = oct,
  Year = 1998,
  publisher = "",
series = {LNCS 1494 },
  publisher =  springer,
  
}
@techreport{LF82,
  Author = "Lamport, Leslie and Michael Fischer",
  Title = "Byzantine Generals and Transaction Commit Protocols",
  number = 62,
  Institution = "SRI International",
  month = apr,
  Year = 1982
  }

@article{LM-S85,
  Author = "Lamport, Leslie and P. M. Melliar{-}Smith",
  Title = "Synchronizing Clocks in the Presence of Faults",
  Journal = jacm,
  month = jan,
  Year = 1985,
  volume = 32,
  number = 1,
  pages = "52--78"
  }

@article{LSP82,
  Author = "Lamport, Leslie and Robert Shostak and Marshall Pease",
  Title = "The {Byzantine} Generals Problem",
  Journal = toplas,
  month = jul,
  Year = 1982,
  volume = 4,
  number = 3,
  pages = "382--401"
  }

@TECHREPORT{LG90,
	  AUTHOR = {T. V. Laxmanan and D. Ghoshal},
	  TITLE = {A new $\sqrt{N}$ multiple copy update algorithm and
its performance evaluation},
	  INSTITUTION = {University of Maryland at College Park},
	  YEAR = {1990},
	  NUMBER = {CS-TR-2502},
	  MONTH = jul
}

@article{LD87,
  Author = "Lee, Insup and Susan B. Davidson",
  Title = "Adding Time to Synchronous Process Communications",
  Journal = ieeetc,
  month = aug,
  Year = 1987,
  volume = "C-36",
  number = 8,
  pages = "941--948"
  }

@inproceedings{Leh84,
  crossref = "podc84",
  Author = "Lehmann, Daniel",
  Title = "Knowledge, Common Knowledge, and Related Puzzles",
  pages = "62--67"
  }

@techreport{LS88,
  Author = "Lipton, Richard J. and Jonathan S. Sandberg",
  Title = "{PRAM}:  A Scalable Shared Memory",
  institution = "Princeton University, Department of Computer Science",
  Number = "180-88",
  month = sep,
  Year = 1988
  }

@inproceedings{Jay93,
Author={ P. Jayanti},
Title={ On the Robustness of Herlihy's Hierarchy},
 booktitle   = "12th " # podc,
year=1993,
pages={145--157}
}

@inproceedings{Li91,
  Author = "Liskov, Barbara",
  Title = "Practical Uses of Synchronized Clocks in Distributed Systems",
  pages = "1--9",
  booktitle = proc # " Tenth " # podc,
  month = aug,
  Year = 1991,
  confaddress = "Montreal, Qu\'{e}bec",
  confeditor = "Richard Ladner"
  }
@book{Lyn96,
  Author = "Lynch, Nancy A.",
  Title = " Distributed Algorithms",
  Publisher = "Morgan Kaufmann",
  Year = 1996
  }

@book{AW98,
Author={ Hagit Attiya and Jennifer Welch},
Title= {Distributed Computing. Fundamentals, Simulations, and Advanced Topics.},
Publisher={McGraw-Hill},
Year= "1998",
}



@inproceedings{LS92,
  Author  = {Lynch, N. and Shavit, N},
  Title = { Timing-based mutual exclusion},
  booktitle = {Proceedings of the 13th Real-Time Systems Symp.},
  confaddress = "Los Alamitos, Calif.",
  month = dec,
  year = "1992",
  pages = "2--11"
  }

@inproceedings{LH94,
	AUTHOR = {Lo, Wai-Kau and Hadzilacos, Vassos},
	TITLE = {Using failure detectors to solve consensus in
                  asynchronous shared memory systems},
	BOOKTITLE = {WDAG},
        SERIES = {LNCS 857},
       
	YEAR = {1994},

	month = sep,
        pages = "280--295"
}

%M


@article{Mat89,
	Author = "Mattern, F.",
	Title = "Global quiescence detection based on credit
                  distribution and recovery",
	Journal = ipl,
	Volume = 30,
	number = 4,
	Year = 1989,
	pages = "195--200"
}

@article{Mat87,
  Author = "Mattern, F.",
  Title = "Algorithms for distributed termination detection",
  Journal = dc,
  Volume = 2,
  number = 3,
  Year = 1987,
  pages = "161--175",
  }

@inproceedings{MAMSA94,

  Author = "Moser, L.E. and Amir, Y. and Melliar-Smith, P.M. and Agarwal, D.A. ",
  Title = "Extended Virtual Synchrony",
   pages = "56-65", 
  crossref = "icdcs94",


}

@inproceedings{MFSW95,

  Author = "Malloth, C.P. and Felber P. and Schiper A. and Wilhelm",
  Title = "Phoenix: a toolkit for building fault-tolerant, distributed applications in large scale",
  booktitle = {Workshop on Parallel and Distributed Platforms in Industrial Products},
year= "1995",
mont= oct,



}


@inproceedings{MPS91, 
author = {Mishra, Shivakant and Peterson, Larry L. and Schlichting,
  Richard D.}, 
title = {A membership protocol based on partial order}, 
booktitle = {Proceedings of the IEEE International Working
Conference on Dependable Computing For Critical Applications}, 
address = {Tucson, AZ}, 
month = feb, 
pages = {137--145}, 
year = 1991,
}

@article{MPS93, 
author = {Mishra, Shivakant and Peterson, Larry L. and Schlichting,
  Richard D.}, 
title = {Consul: a Communication Substrate for Fault tolerant Distributed Programs}, 
Journal = {Distributed Systems Engineering},
pages = {87--103}, 
year = 1993,
}

@article{MMSALP96,
   Author = " Moser , L.E. and Melliar-Smith, P.M. and Agarwal, D.A and Budhia, R.K. and Lingley-Papadopoulos, C. A.",
  Title = "Totem: A Fault Tolerant Multicast Group Communication System",
  Journal = cacm,
  month = apr,
  Year = "96",
  volume = 39,
  number = 4,
  pages = "54--63",

  }
@Article{MMA90,
  author = 	 { Melliar-Smith P.M. and Moser, Louise E. and Agrawala, Vivek},
  title = 	 {Broadcast protocols for distributed systems},
  journal = 	 {IEEE Transactions on Parallel and Distribued Systems },
  year = 	 {90},
  volume = 	 {1},
  number = 	 {1},
  pages = 	 {17-25},
  month = 	 jan,
 }

@article{MMA94,
author  = {Melliar-Smith, P.M. and Moser, Louise and Agrawala, Vivek},
title = {Processor membership in asynchronous distributed systems},
journal = {IEEE Transactions on Parallel and Distributed Systems},
volume = {5},
number = 5,
month = may,
pages = {459--473},
year = 1994}

@article{ MR01, 
  author = "Most\'efaoui, A. and Raynal, M.", 
  title = "Leader-based consensus", 
   Journal = "Parallel Processing Letters",
  Volume = " 11 ",
  Number = 1,
  Pages = "95-107",
  year = 2001
}








@inproceedings{MRR01,
  crossref = "podc01",
  Author = "Achour Most\'efaoui and Sergio Rajbaum and Michel Raynal",
  Title = "Conditions on input vectors for consensus solvability in asynchronous distributed systems",
  year =2001,

  }

@inproceedings{MS85,
  crossref = "podc85",
  Author = "Mahaney, Stephen R. and Fred B. Schneider",
  Title = "Inexact Agreement:  Accuracy, Precision, and Graceful Degradation",
  pages = "237--249"
  }
@article{MR98,
  Author = "Malkhi, Dahlia and Reiter, Michael",
  Title = "Byzantine quorum systems",
  Journal = dc,
  Year = 1998,
  volume = "11?",
  number = "?",
  pages = "203--213"
  }


@inProceedings{MMT91,
   author =    {Merritt, M. and  Modugno, F. and Tuttle, M.},
   title =     {Time constrained automata},
   booktitle = {Proceedings of CONCUR'91},
   year =      1991, 
   publisher = springer,   
   series = {LNCS 527},
   pages = "408--423",
}


@inproceedings{MR99a,
  Author = "Most\'efaoui, Achour and Raynal, Michel", 
  title = {Solving Consensus Using {C}handra-{T}oueg's Unreliable Failure
                  detectors: A General Quorum Based Approach},  
 booktitle = proc # " 13th International Symp. on Distributed Computing",
  series = "LNCS 1693",
  month = sep,
  publisher = springer,
  pages = "49--63",
  year = 1999,
   }

@inProceedings{MR99b,
   author =    "Most\'efaoui, Achour and Raynal, Michel",
   title =     {Unreliable Failure Detectors with Limited Scope Accuracy and 
Application to Consensus},
     year =      1999, 
   publisher = springer,   
   series = {LNCS 1738},
   pages = "329--340",
booktitle = proc # " 19th " # "FST-TCS",
 
 month = dec,

}



@inproceedings{ MR00b, 
  author = "Most\'efaoui, Achour and Raynal, Michel", 
  title = "$k$-set agreement with limited accuracy failure detectors", 
  
crossref="podc00",
pages="143--152",

} 

@inproceedings{Mat88,
  crossref = "bonas",
  Author = "Mattern, Friedemann",
  Title = "Virtual Time and Global States of Distributed Systems",
  pages = "215--242"
  }

@techreport{MS94,
author={ Malloth, C. and Schiper, A.},
title={View synchronous communication in large scale networks},
 Institution = epfl,
  month = oct,
  Year = "1994",
  number = "94/84"
  }
}

@inproceedings{MSF83,
  crossref= "podc83",
  Author = "Mohan, C. and R. Strong and S. Finkelstein",
  Title = "Methods for Distributed Transaction Commit and Recovery
		Using {Byzantine} Agreement within Clusters of Processors",
  pages = "89--103"
  }

@INPROCEEDINGS{MT89,
	crossref = "wdag89",
	  AUTHOR = {Moran, Shlomo and Taubenfeld, Gadi},
	  TITLE = {Possibility and Impossibility Results in a Shared
Memory Environment},
	  PAGES = {254--267}
}

@article{Mor85,
  Author = "Morgan, Carroll",
  Title = "Global and Logical Time in Distributed Algorithms",
  Journal = ipl,
  month = may,
  Year = 1985,
  volume = 20,
  number = 4,
  pages = "189--194"
  }
  

%N
@inproceedings{Neig95,
author={ Gil Neiger},
title={Failure Detectors and the Wait-Free Hierarchy},
booktitle   = {Proceedings of the 14th ACM Symp. on Principles of Distributed Computing},
year={1995}
} 


@inproceedings{NT87,
  Crossref = "podc87",
  Author = "Neiger, Gil and Sam Toueg",
  Title = "Substituting for Real Time and Common Knowledge in
  		Asynchronous Distributed Systems (preliminary version)",
  pages = "281--293",
  booktitle = proc # " Sixth " # podc,
  month = aug,
  Year = 1987,
  confaddress = "Vancouver, British Columbia",
  confeditor = "Fred B. Schneider",
  note = "A revised and expanded version appears as:
	Simulating Synchronized Clocks and Common Knowledge in Distributed Systems.
	{\em Journal of the ACM}, 40(2):334--367, April 1993."
  }

@inproceedings{NT88,
  crossref = "bonas",
  Author = "Neiger, Gil and Sam Toueg",
  Title = "Providing Design Abstractions in Distributed Systems",
  pages = "227--242"
  }

@article{NT90a,
  Author = "Neiger, Gil and Sam Toueg",
  Title = "Automatically Increasing the Fault-Tolerance
		of Distributed Algorithms",
  Journal = "Journal of Algorithms",
  month = sep,
  Year = 1990,
  volume = 11,
  number = 3,
  pages = "374--419"
  }

@techreport{NT90b,
  Author = "Neiger, Gil and Sam Toueg",
  Title = "Simulating Synchronized Clocks and Common Knowledge in Distributed
		Systems",
  institution = gitics,
  Number = "90/05",
  month = jan,
  Year = 1990
  }
  
@inproceedings{dstm-contention,
 author = {Scherer,III, William N. and Scott, Michael L.},
 title = {Advanced Contention Management for Dynamic Software Transactional Memory},
 booktitle = {Proceedings of the Twenty-fourth Annual ACM Symp. on Principles of Distributed Computing},
 series = {PODC '05},
 year = {2005},
 isbn = {1-58113-994-2},
 location = {Las Vegas, NV, USA},
 pages = {240--248},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/1073814.1073861},
 doi = {10.1145/1073814.1073861},
 acmid = {1073861},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {contention management, obstruction-freedom, synchronization, transactional memory},
} 

@inproceedings{rmr-mutex,
 author = {Attiya, Hagit and Hendler, Danny and Woelfel, Philipp},
 title = {Tight RMR Lower Bounds for Mutual Exclusion and Other Problems},
 booktitle = {Proceedings of the Twenty-seventh ACM Symp. on Principles of Distributed Computing},
 series = {PODC '08},
 year = {2008},
 isbn = {978-1-59593-989-0},
 location = {Toronto, Canada},
 pages = {447--447},
 numpages = {1},
 url = {http://doi.acm.org/10.1145/1400751.1400843},
 doi = {10.1145/1400751.1400843},
 acmid = {1400843},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {bounded counter, information theory, lower bound techniques, mutual exclusion, shared-memory, store/collect object},
} 

@article{TM-WF14,
  author    = { Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On Partial Wait-Freedom in Transactional Memory},
  journal   = {CoRR},
  volume    = {abs/1407.6876},
  year      = {2014},
  ee        = {http://arxiv.org/abs/1407.6876},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Owi93,
  crossref = "podc93",
  Author = "Owicki, Susan S.",
  Title = "A Perspective on {AN2}: Local Area Network as Distributed System",
  pages = "1--12",
  }
@inproceedings{OFTM,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {On obstruction-free transactions},
 booktitle = {Proceedings of the twentieth annual Symp. on Parallelism in algorithms and architectures},
 series = {SPAA '08},
 year = {2008},
 isbn = {978-1-59593-973-9},
 location = {Munich, Germany},
 pages = {304--313},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1378533.1378587},
 doi = {http://doi.acm.org/10.1145/1378533.1378587},
 acmid = {1378587},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {consensus number, impossibility, obstruction-freedom, transactional memory},
} 


%Author = "Oliveira and  Guerraoui and Schiper",
%Title = "Consensus in the crash recovery model",
%Year = 1997



%P
@article{PSL80,
  Author = "Pease, Marshall and Shostak, Robert and Lamport, Leslie",
  Title = "Reaching Agreement in the Presence of Faults",
  Journal = jacm,
  month = apr,
  Year = 1980,
  volume = 27,
  number = 2,
  pages = "228--234"
  }
  
  
@inproceedings{PS98,
 author  = {Pedone, Fernando and Schiper, {Andr\'e}},
  title = {Optimistic Atomic Broadcast},
  booktitle = proc # " 12th " # wdag,
  series = {LNCS 1499},
  month = sep,
  publisher = "Springer Verlag",
  pages = {318--332},
  year = 1998,
}
@phdthesis{Per85,
  Author = "Perry, Kenneth J.",
  Title = "Early Stopping Protocols for Fault-Tolerant Distributed Agreement",
  School = cornell,
  month = feb,
  Year = 1985,
  note = "Department of Computer Science Technical Report 85-662"
  }



@TECHREPORT{PT84,
        AUTHOR = {Perry, Kenneth J. and Toueg, Sam},
        TITLE = {An authenticated {B}yzantine Generals algorithm with
early stopping},
        INSTITUTION = {Department of Computer Science, Cornell University},
        YEAR = {1984},
        NUMBER = {84-620},
        MONTH = Jun
}

@article{PT86,
  Author = "Perry, Kenneth J. and Sam Toueg",
  Title = "Distributed Agreement in the Presence of Processor and
		Communication Faults",
  Journal = ieeese,
  month = mar,
  Year = 1986,
  volume = 12,
  number = 3,
  pages = "477--482"
  }

@article{PBS89,
	AUTHOR = {Peterson, Larry L. and Bucholz, Nick C. and
Schlichting, Richard D.},
	TITLE = {Preserving and using context information in
interprocess communication},
	Journal = tocs,
	YEAR = 1989,
	MONTH = Aug,
	Volume = 7,
        Number = 3,
	PAGES = "217--246"
}
@article{dwork97,
 author = {Dwork, Cynthia and Herlihy, Maurice and Waarts, Orli},
 title = {Contention in Shared Memory Algorithms},
 journal = {J. ACM},
 issue_date = {Nov. 1997},
 volume = {44},
 number = {6},
 month = nov,
 year = {1997},
 issn = {0004-5411},
 pages = {779--805},
 numpages = {27},
 url = {http://doi.acm.org/10.1145/268999.269000},
 doi = {10.1145/268999.269000},
 acmid = {269000},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {contention, counting networks, mutual exclusion},
} 


@inproceedings{Rab83,
  crossref = "focs83",
  Author = "Rabin, Michael",
  Title = "Randomized {Byzantine} Generals",
  pages = "403--409"
  }


@ARTICLE{RST90,
	AUTHOR = {Raynal, Michel and Schiper, {Andr} and Toueg, Sam},
	TITLE = {The Causal Ordering Abstraction and a Simple Way to
		Implement it},
	JOURNAL = ipl,
	YEAR = {1991},
	VOLUME = 39,
        PAGES = " 343--350"
}

@TECHREPORT{Rei82,
	AUTHOR = {Reischuk, R{\"{u}}diger},
	TITLE = {A new solution for the {B}yzantine general's problem},
	INSTITUTION = {IBM Research Laboratory},
	YEAR = {1982},
	NUMBER = {RJ 3673},
	MONTH = Nov
}


@inproceedings{PS99,
 author  = {Pedone, Fernando and Schiper, {Andr\'e}},
  title = {Generic Broadcast},
  booktitle = proc # " 13th " # wdag,
  series = {LNCS 1693},
  month = sep,
  publisher = "Springer Verlag",
  pages = {94-108},
  year = 1999,
}




@INPROCEEDINGS{RiBi91,
	AUTHOR = {Ricciardi, Aleta and Birman, Ken},
	TITLE = {Using Process Groups to Implement Failure Detection in
		Asynchronous Environments},
	CROSSREF = "podc91",
	PAGES = "341--351",
	
}

@article{RSA78,
  Author = "Rivest, Ronald L. and Adi Shamir and Leonard Adleman",
  Title = "A Method for Obtaining Digital Signatures and {Public-Key}
		Cryptosystems",
  Journal = cacm,
  month = feb,
  Year = 1978,
  volume = 21,
  number = 2,
  pages = "120--126"
  }


@inproceedings{HS11-progress,
  author    = {Maurice Herlihy and
               Nir Shavit},
  title     = {On the Nature of Progress},
  booktitle = {OPODIS},
  year      = {2011},
  pages     = {313-328}
}


@article{RT99,
Author = "Michel Raynal and {Frdric} Tronel",
Title = "Group membership failure detection a simple protocol and its probabilistic analysis",
Journal = "Distributed Systems Engineering Journal",
volume= 6,
number= "3",
pages= "95--102",
year= 1999,
}
@techreport{RV92,
author={Rodrigues, L and Verissimo, P},
title={xAMp, a protocol suite for group communication},
number="RT/43-92",
institution="INESC",
mont="January",
year=1992,
}
%S
@techreport{ SM95,
    author = "Laura S. Sabel and Keith Marzullo",
    title = "Election Vs. Consensus in Asynchronous Systems",
    number = "TR95-1488",
    month = "17,",
    pages = "9",
    year = "1995",
    url = "citeseer.nj.nec.com/sabel95election.html" }

@InProceedings{SM99,  
	crossref = "disc99",
        author =       "Jeremy Sussman and Keith Marzullo",
        title =        "The Bancomat Problem: An example of resource 
                   allocationin a partitionable asynchronous system",
pages="363--388",
     }

@article{Sch97,
  Author = "Schiper, {Andr\'e}",
  Title = "Early consensus in an asynchronous system with a weak failure detector",
  Journal = dc,
  Year = 1997,
  volume = 10,
  number = 3,
  pages = "149-157",
  }

@article{Ennals05,
  Author = "Ennals, Robert",
  Title = "Software Transactional Memory should not be Obstruction-free",
  Journal = http://www2.berkeley.intel-research.net/~rennals/pubs/052RobEnnals.pdf,
  Year = 2005,
  
  }

@article{Sch93,
  Author = {M. Schneider},
  Title = "Self-Stabilization",
  Journal = surveys,
   Year = 1993,
  volume = 25,
  number = 1,
  }



@article{Sch90,
  Author = {Fred B. Schneider},
  Title = "Implementing Fault-Tolerant Services Using the State Machine
Approach: A Tutorial",
  Journal = surveys,
  month = dec,
  Year = 1990,
  volume = 22,
  number = 4,
  pages = "299--319"
  }


@ARTICLE{SGS84,
	AUTHOR = {Schneider, Fred B. and Gries, David and Schlichting, Richard
		D.},
	TITLE = {Fault-Tolerant Broadcasts},
	JOURNAL = {Science of Computer Programming},
	YEAR = {1984},
	VOLUME = {4},
	NUMBER = 1,
	MONTH = apr,
	PAGES = {1--15}
}


@article{SS83,
  Author = "Schlichting, Richard D. and Fred B. Schneider",
  Title = "Fail-Stop Processors: an Approach to Designing
Fault-Tolerant Computing Systems",
  Journal = tocs,
  month = aug,
  Year = 1983,
  volume = 1,
  number = 3,
  pages = "222--238"
  }
@inproceedings{SS93,

Author = "Schiper, {Andr} and Sandoz, A. ",
  Title = "Uniform reliable multicast in a virtually synchronous environment",
   pages = "561-568", 
  crossref = "icdcs93",


}
@inproceedings{SR93,

Author = "Schiper, {Andr\'e} and Ricciardi, A.M. ",
  Title = "Virtually Synchronous Communication based on a Weak Failure Susupector",
   pages = "534-543", 
  note= "Digest of Papers FTCS 23",
place = Toulouse,
month=  jun ,
year=93,


}
@inproceedings{SS94,

Author = "Schiper, {'Andr\'e} and Sandoz, A. ",
  Title = {Primary Partition "Virtually-Synchronous Communication" harder 
            than Consensus},
   pages = "38-52", 
  crossref = "wdag94",


}
@phdthesis{Sch88,
  Author = "Schmuck, Frank Bernhard",
  Title = "The Use of Efficient Broadcast Protocols in Asynchronous
		Distributed Systems",
  School = cornell,
  month = aug,
  Year = 1988,
  note = "Department of Computer Science Technical Report 88-928"
  }
  
@article{Sch82,
  Author = "Fred B. Schneider",
  Title = "Synchronization in Distributed Programs",
  Journal = toplas,
  month = apr,
  Year = 1982,
  volume = 4,
  number = 2,
  pages = "125--148"
  }

@article{Sch84,
  Author = "Fred B. Schneider",
  Title = "Byzantine Generals in Action:  Implementing Fail-Stop Processors",
  Journal = tocs,
  month = may,
  Year = 1984,
  volume = 2,
  number = 2,
  pages = "145--154"
  }

@techreport{Sch86,
  Author = "Fred B. Schneider",
  Title = "The State Machine Approach:  a Tutorial",
  number = "86-800",
  institution = cornellcs,
  month = dec,
  Year = 1986,
  note = "Revised June 1987"
  }

@unpublished{SY89,
  Author = "Shanbhogue, Vasant and Moti Yung",
  Title = "Distributed Consensus in the Presence of Byzantine Edges
  		in Asynchronous Networks",
  month = dec,
  Year = 1989,
  note = "Unpublished manuscript"
  }

@PHDTHESIS{Sk82,
	AUTHOR = {Skeen, Dale},
	TITLE = {Crash Recovery in a Distributed Database System},
	SCHOOL = {University of California at Berkeley, Department of EECS},
	YEAR = {1982}
}


@article{SS84,
  Author = "Schlichting, Richard D. and Fred B. Schneider",
  Title = "Using mesage passing for distributed programming: proof
                  rules and disciplines",
  Journal = toplas,
  Year = 1984,
  volume = 6,
  pages = "402--431"
  }


@article{SM94,
  Author = "Schwartz, R. and  Mattern, F.",
  Title = "Detecting causal relationships in distributed computations:
   In search of the holy grail",
  Journal = dc,
  Year = 1994,
  volume = 7,
  number = 3,
  pages = "149--174"
  }
@phdthesis{Sri86,
  Author = "T. K. Srikanth",
  Title = "Designing Fault-Tolerant Algorithms for Distributed Systems
  		Using Communication Primitives",
  School = cornell,
  month = feb,
  Year = 1986,
  note = "Department of Computer Science Technical Report 86-739"
  }

@article{ST87a,
  Author = "T. K. Srikanth and Sam Toueg",
  Title = "Optimal Clock Synchronization",
  Journal = jacm,
  month = jul,
  Year = 1987,
  volume = 34,
  number = 3,
  pages = "626--645"
  }

@article{ST87b,
  Author = "T. K. Srikanth and Sam Toueg",
  Title = "Simulating Authenticated Broadcasts to Derive
		Simple Fault-Tolerant Algorithms",
  Journal = dc,
  Year = 1987,
  volume = 2,
  number = 2,
  pages = "80--94"
  }

@inproceedings{SZ93,
  booktitle = proc # " 25th " # stoc,
  month = may,
  Year = 1993,
  confaddress = "San Diego, California",
  confeditor = "Alok Aggrawal",
  publisher = "ACM Press",
  Author = {Saks, Michael and Fotios Zaharoglou},
  Title = "Wait-Free $k$-Set Agreement is Impossible: The Topology of
Public Knowledge",
  pages = "101--110"
  }
  
%T

@article{SZ00,
  Author = {Saks, Michael  and Zaharoglou, Fotios},
  Title = "Wait-Free k-Set Agreement Is Impossible: The Topology of Public Knowledge",
  Journal = "SIAM J. on Computing",
  volume = 29,
  Year = 2000,
  pages = "1449--1483"
  }




@book{T91,
  Author = "Tel, G.",
  Title = "Topics in Distributed Algorithms",
  Publisher = "Cambridge University Press",
  Year = 1991
  }

@book{T94,
  Author = "Tel, G.",
  Title = "Introduction to Distributed Algorithms",
  Publisher = "Cambridge University Press",
  Year = 1994
  }


@book{Tan81,
  Author = "Tanenbaum, Andrew S.",
  Title = "Computer Networks",
  Publisher = "Prentice-Hall",
  Year = 1981
  }

@incollection{Tay89,
  crossref = "wdag89",
  Author = "Taylor, Kim",
  Title = "The Role of Inhibition in Asynchronous Consistent Cut Protocols",
  pages = "280--291"
  }

@phdthesis{Tay90,
  Author = "Taylor, Kimberly E.",
  Title = "Knowledge and Inhibition in Asynchronous Distributed Systems",
  School = cornell,
  month = jul,
  Year = 1990,
  note = "Department of Computer Science Technical Report 90-1139"
  }



@inproceedings{Tou84,
  crossref = "podc84",
  Author = "Toueg, Sam",
  Title = "Randomized {Byzantine} Agreements",
  pages = "163--178"
  }

@article{TPS87,
  Author = "Toueg, Sam and Kenneth J. Perry and T. K. Srikanth",
  Title = "Fast Distributed Agreement",
  Journal = sicomp,
  month = jun,
  Year = 1987,
  volume = 16,
  number = 3,
  pages = "445--457"
  }
%U
%V
@inproceedings{VA86,
Author={ P. Vitanyi and B. Awerbuch},
Title={ Atomic shared register access by asynchronous hardware},
booktitle={Proceedings of the IEEE Symp. om Foundations of Computer Science}, 
year=1986,
pages="233--243",
}
 
@article{vRBM96,
  Author = "van Renesse, R. and Birman, K.P. and Maffeis, S.",
  Title = "Horus: A flexible group communication system",
  Journal = cacm,
  month = apr,
  Year = "96",
  volume = 39,
  number = 4,
  pages = "76--83",

  }

@inproceedings{VMH98,
  author = "van Renesse, R. and  Minsky, Y.  and M. Hayden, M.",
  title = " A gossip-based failure detection service",
  booktitle = "Proceedings  of Middleware'98  ",
  year = 1998,
  month = sep,
}

@INPROCEEDINGS{VM90,
AUTHOR = "Ver\'{\i}ssimo, Paulo and Marques,Jos\'{e} A.",
TITLE = "Reliable Broadcast for Fault-Tolerance on Local Computer Networks",
BOOKTITLE  =  "Proceedings of the 9th Symp. on Reliable Distributed Systems",
publisher = "IEEE Computer Society Press",
YEAR = "1990",
MONTH=oct,
ADDRESS = "Huntsville, Alabama-USA"
}
%W
@MASTERSTHESIS{Web89,
        AUTHOR = {Weber, Samuel},
        TITLE = {Bounds on the message Complexity of {B}yzantine Agreement},
        SCHOOL = {University of Toronto},
        YEAR = {1989},
        MONTH = Oct
}

@article{Wel87,
  Author = "Welch, Jennifer Lundelius",
  Title = "Simulating Synchronous Processors",
  Journal = ic,
  month = aug,
  Year = 1987,
  volume = 74,
  number = 2,
  pages = "159--171"
  }

@article{WL88,
  Author = "Welch, Jennifer Lundelius and Nancy A. Lynch",
  Title = "A New Fault-Tolerant Algorithm for Clock Synchronization",
  Journal = ic,
  month = apr,
  Year = 1988,
  volume = 77,
  number = 1,
  pages = "1--36"
  }

@article{Wen78,
  Author = {Wensley, John H. and Leslie Lamport and Jack Goldberg and
Milton W. Green and
            Karl N. Levitt and P.M. Melliar-Smith and Robert E. Shostak
and Charles B. Weinstock},
  Title = "{SIFT}: Design and Analysis of a Fault-Tolerant Computer for
Aircraft Control",
  Journal = "Proceedings of the IEEE",
  month = oct,
  Year = 1978,
  volume = 66,
  number = 10,
  pages = "1240--1255"
  }


@inproceedings{WMK95,
author  = {Whetten, B. and Montgomery, T. and Kaplan, S., Robbert},
title = {A hight performance totally ordered multicast protocol},
booktitle = {Theory and Practice in Distributed Systems: International Workshop},
editor = {Birman, K. and Mattern,F. and Schipper, A. },
publisher = springer,
pages = {33-57},
year = 1995,
series= {LNCS 938},
}
@inproceedings{WS95,
author  = {Wilhelm, U. G. and Schiper, A.},
title = {A hierarchy of totally ordered multicasts },
crossref= "srds95",


}

@inproceedings{YNG98,
author={Yang, Jiong and Neiger, Gil and Gafni,Eli},

pages="297--306",

  booktitle = proc # " 17th " # podc,
 title={Structured Derivations of consensus Algorithms for Failure Detectors},
   Year = 1998,

  }
}


%-----------------------CROSSREF PODC

@proceedings{podc83,
  booktitle = proc # " 2nd " # podc,

  month = aug,
  Year = 1983,
  confaddress = "Montreal, Qu\'{e}bec",
  confeditor = "Nancy A. Lynch"
  }

@proceedings{podc84,
  booktitle = proc # " 3th " # podc,

  month = aug,
  Year = 1984,
  confaddress = "Vancouver, British Columbia",
  confeditor = "Jayadev Misra"
  }

@proceedings{podc85,
  booktitle = proc # " 4th " # podc,
  title = proc # " Fourth " # podc,
  month = aug,
  Year = 1985,
  confaddress = "Minaki, Ontario",
  confeditor = "Ray Strong"
  }

@proceedings{podc86,
  booktitle = proc # " 5th " # podc,

  month = aug,
  Year = 1986,
  confaddress = "Calgary, Alberta",
  confeditor = "Joseph Halpern"
  }

@proceedings{podc87,
  booktitle = proc # " 6th " # podc,

  month = aug,
  Year = 1987,
  confaddress = "Vancouver, British Columbia",
  confeditor = "Fred B. Schneider"
  }

@proceedings{podc88,
  booktitle = proc # " 7th " # podc,

  month = aug,
  Year = 1988,
  confaddress = "Toronto, Ontario",
  confeditor = "Danny Dolev"
  }

@proceedings{podc89,
  booktitle = proc # " 8th " # podc,

  month = aug,
  Year = 1989,
  confaddress = "Edmonton, Alberta",
  confeditor = "Michael Merritt"
  }

@proceedings{podc90,
  booktitle = proc # " 9th " # podc,

  month = aug,
  Year = 1990,
  confaddress = "Qu\'{e}bec City, Qu\'{e}bec",
  confeditor = "Cynthia Dwork"
  }

@proceedings{podc91,
  booktitle = proc # " 10th " # podc,

  month = aug,
  Year = 1991,
  confaddress = "Montreal, Qu\'{e}bec",
  confeditor = "Richard Ladner"
  }

@proceedings{podc92,
  booktitle = proc # " 11th " # podc,
  month = aug,
  Year = 1992,
  confaddress = "Vancouver, British Columbia",
  confeditor = "Maurice Herlihy"
  }

@proceedings{podc93,
  booktitle = proc # " 12th " # podc,
   month = aug,
  Year = 1993,
  confaddress = "Ithaca, New York",
  confeditor = "Sam Toueg"
  }
@proceedings{podc94,
  booktitle = proc # " 13th " # podc,
  month = aug,
  Year = 1994,
  confaddress = "?",
  confeditor = "",
  }
@proceedings{podc95,
  booktitle = proc # " 14th " # podc,
   month = aug,
  Year = 1995,
  confaddress = "?",
  confeditor = "",
  }
@proceedings{podc96,
  booktitle = proc # " 15th " # podc,
 
  Year = 1996,
  confaddress = "Philadelphia, Pennsylvania",
  confeditor = "Yoram Moses"
  }
  @proceedings{podc97,
  booktitle = proc # " 16th " # podc,
 
  Year = 1997,
  confaddress = "?",
  confeditor = "?"
  }
@proceedings{podc98,
  booktitle = proc # " 17th " # podc,
 
   Year = 1998,
  confaddress = "?",
  confeditor = "?"
  }
@proceedings{podc99,
  booktitle = proc # " 18th " # podc,
 
  Year = 1999,
  confaddress = "Atlanta",
  confeditor = ""
  }
@proceedings{podc00,
  booktitle = proc # " 19th " # podc,
 
  month = "aug",
  Year = 2000,
  confaddress = "Portland,Oregon",
  confeditor = ""
  }
@proceedings{podc01,
  booktitle = proc # " 20th " # podc,
 
  month = "aug",
  Year = 2001,
  confaddress = "",
  confeditor = ""
  }
@proceedings{podc02,
  booktitle = proc # " 21th " # podc,
 
  month = jul,
  Year = 2002,
  confaddress = "Monterey, California",
  confeditor = ""
  }

%-------------------CROSSREF FTCS-------------------------------

@proceedings{ftcs85,
  booktitle = proc # " Fifteenth " # ftcs,
 
  month = jun,
  Year = 1985,
  confaddress = "Ann Arbor, Michigan"
  }

@proceedings{ftcs86,
  booktitle = proc # " 16th " # ftcs,
 
  month = jul,
  Year = 1986,
  confaddress = "Vienna, Austria"
  }
  
@proceedings{ftcs87,
  booktitle = proc # " 17th " # ftcs,
 
  month = jul,
  Year = 1987,
  confaddress = "Pittsburgh, Pennsylvania",
  publisher = "IEEE Computer Society Press",
  confeditor = "Flaviu Cristian and Jack Goldberg"
  }

@proceedings{ftcs92,
  booktitle = proc # " 22th " # ftcs,
 
  month = jul,
  Year = 1992,
  publisher = "IEEE Computer Society Press",
  }
@proceedings{ftcs93,
booktitle = proc # "23th " # ftcs,

confaddress = {Toulouse},
month = jun,
Year= 1993,
 publisher = "IEEE Computer Society Press",
}


%----------------------CROSSREF FOCS
@proceedings{focs83,
  booktitle = proc # " 24th " # focs,

  month = nov,
  Year = 1983,
  confaddress = "Tucson, Arizona",
  publisher = "IEEE Computer Society Press",
  confeditor = "Lawrence Snyder"
  }

@proceedings{focs84,
  booktitle = proc # " 25th " # focs,

  month = oct,
  Year = 1984,
  publisher = "IEEE Computer Society Press",
  confaddress = "West Palm Beach, Florida"
  }

@proceedings{focs86,
  booktitle = proc # " 27th " # focs,

  month = oct,
  Year = 1986,
  publisher = "IEEE Computer Society Press",
  confaddress = "Toronto, Ontario"
  }

@proceedings{focs87,
  booktitle = proc # " 28th " # focs,

  month = oct,
  Year = 1987,
  publisher = "IEEE Computer Society Press",
  confaddress = "Los Angeles, California",
  confeditor = "Ashok Chandra"
  }

@proceedings{focs88,
  booktitle = proc # " Twenty-Ninth " # focs,

  month = oct,
  Year = 1988,
  confaddress = "White Plains, New York",
  publisher = "IEEE Computer Society Press",
  confeditor = "Dexter Kozen"
  }

@proceedings{focs89,
  booktitle = proc # " Thirtieth " # focs,

  month = oct,
  Year = 1989,
  confaddress = "Research Triangle Park, North Carolina",
  publisher = "IEEE Computer Society Press",
  confeditor = "Zvi Galil"
  }
@proceedings{focs93,
  booktitle = proc # " 34th " # focs,

  month = nov,
  Year = 1993,
  confaddress = "Palo Alto, California",
  publisher = "IEEE Computer Society Press",
    }
%___________________________CROSSREF STOC  
@proceedings{stoc85,
  booktitle = proc # " Seventeenth " # stoc,

  month = may,
  Year = 1985,
  confaddress = "Providence, Rhode Island",
  confeditor = "Nicholas Pippenger"
  }

@proceedings{stoc86,
  booktitle = proc # " Eighteenth " # stoc,

  month = may,
  Year = 1986,
  confaddress = "Berkeley, California"
  }

@proceedings{stoc88,
  booktitle = proc # " Twentieth " # stoc,

  month = may,
  Year = 1988,
  confaddress = "Chicago, Illinois",
  confeditor = "Jeff Ullman"
  }

@proceedings{stoc91,
  booktitle = proc # " Twenty third " # stoc,

  month = may,
  Year = 1991,
  confaddress = "New Orleans, Louisiana",
  confeditor = "Jeff Vitter"
  }

@proceedings{stoc93,
  booktitle = proc # " Twenty fifth " # stoc,
  month = may,
  Year = 1993,
  confaddress = "San Diego, California",
  confeditor = "Alok Aggrawal",
  publisher = "ACM Press"
  }
  
@proceedings{pods87,
  booktitle = proc # " Sixth " # pods,

  month = mar,
  Year = "1987",
  confaddress = "San Diego, California",
  publisher = "ACM Press"
  }
%------------------------------CROSSREF BONAS
@proceedings{bonas,
    booktitle = "Proceedings of the International Workshop on Parallel and
  		Distributed Algorithms",
  confaddress = "Ch\^{a}teau de Bonas, Gers, France",
  month = oct,
  Year = 1988,
  publisher = "North-Holland",
  editor = "Michel Cosnard and Patrice Quinton and Yves Robert
		and Michel Raynal",
  }

%---------------------CROSSREF WDAG--- CROSSREF DISC------------------

@proceedings{wdag89,
  booktitle = proc # " Third " # wdag,
  
  editor = "J.-C. Bermond and M. Raynal",
  confaddress = "La Colle-sur-Loup, France",
  series = {LNCS 392},
  month = sep,
  Year = 1989,
  publisher =  {Springer-Verlag}
  }

@proceedings{wdag90,
  booktitle = proc # " Fourth " # wdag,
  
  editor = "J. van Leeuwen and N. Santoro",
  confaddress = "Bari, Italy",
  series = {LNCS},
  month = sep,
  Year = 1990,
  publisher =  {Springer-Verlag},
  }

@proceedings{wdag91,
  booktitle = proc # " Fifth " # wdag,
  
  editor = "S. Toueg and P.G. Spirakis and L. Kirousis",
  confaddress = "Delphi, Greece",
  series = {LNCS},
  month = oct,
  Year = 1991,
  publisher = {Springer-Verlag},
  }

@proceedings{wdag92,
  booktitle = proc # " Sixth " # wdag,
  
  editor = "A. Segal and S. Zaks",
  confaddress = "Haifa, Israel",
  series = {LNCS},
  month = nov,
  Year = 1992,
  publisher =  {Springer-Verlag},
  }
	
@proceedings{wdag93,
  booktitle = proc # " Seventh " # wdag,
  
  editor = "",
  confaddress = "",
  series = {LNCS},
  month = nov,
  Year = 1993,
  publisher =  {Springer-Verlag},
  }
	
@proceedings{wdag94,
  booktitle = proc # " Heighth " # wdag,
  
  editor = "",
  confaddress = "",
  series = {LNCS 857},
  month = nov,
  Year = 1994,
  publisher = {Springer-Verlag},
  }
	
@proceedings{wdag95,
  booktitle = proc # " 9th  " # wdag,
  
  editor = "J.M Helary and M. Raynal",
  confaddress = "",
  series = {LNCS 972},
  month = nov,
  Year = 1995,
  publisher = {Springer-Verlag},
  }

@proceedings{wdag96,
  booktitle = proc # " 10th " # wdag,
  
  editor = "",
  confaddress = "",
  series = {LNCS},
  month = nov,
  Year = 1996,
  publisher = springer,
  }

@proceedings{disc97,
  booktitle = proc # " 11th " # disc,
  
  editor = "",
  confaddress = "",
  series = {LNCS 1320},
  month = nov,
  Year = 1997,
  publisher = springer,
  }


@proceedings{disc98,
  booktitle = proc # " 12th" # disc,
  
  editor = "",
  confaddress = "Andros, Greece",
  series = {LNCS},
  month = sep,
  Year = 1998,
  publisher =  springer,
  }

@proceedings{disc99,
  booktitle = proc # " 13th " # disc,
  
  editor = "",
  confaddress = "Bratislava, Slovaquia",
  series = {LNCS},
  month = oct,
  Year = 1999,
  publisher = "Springer-Verlag",
number= 1693,
  }
@proceedings{disc00,
  booktitle = proc # " Fourteenth " # disc,
  
  editor = "",
  confaddress = "Tolede, Spain",
  series = {LNCS},
  month = oct,
  Year = 2000,
  publisher = {Springer-Verlag},
  }
%-----------------------------------------------------------------------

%-------------------------CROSSREF SRDS-----------------------------
@proceedings{srds95,
  year =        {1995},
publisher = "IEEE Computer Society Press",
  booktitle =   proc # " 14th " # srds,
  month =       sep,
  
}
@proceedings{srds96,
  year =        {1996},
  confaddress =     {Niagara-on-the-Lake, Canada},
  booktitle =   proc # " 15th " # srds,
publisher = "IEEE Computer Society Press",
  month =       oct,
  
}
@proceedings{srds98,
  year =        {1998},
  confaddress =     {West Lafayette, Indiana},
  booktitle =   proc # " 17th " # srds,
publisher = "IEEE Computer Society Press",
  month =       oct,
}

@proceedings{srds00,
  year =        {2000},
  confaddress =     {N\"urnberg, Germany},
  booktitle =   proc # " 19th " # srds,
  publisher = "IEEE Computer Society Press",
  month =       oct,
  
}
%---------------------CROSSREF ICDCS----------------------------------------

@proceedings{icdcs88,
  booktitle = proc # " 8th " # icdcs,
  title = proc # " 8th " # icdcs,
  month = jun,
  Year = 1988,
  publisher = "IEEE Computer Society Press",
 confaddress = "San Jose, California" 
  }
@proceedings{icdcs89,
  booktitle = proc # " 9th" # icdcs,
  title = proc # " 9th " # icdcs,
  month = jun,
  Year = 1989,
publisher = "IEEE Computer Society Press",
  }
@proceedings{icdcs90,
 booktitle = proc #" 10th "# icdcs,
	publisher = "IEEE Computer Society Press",
  month = may,
  Year = 1990,
  confaddress = "Paris, France",
  
  }


@proceedings{icdcs91,
 booktitle = proc #" 11th "# icdcs,
publisher = "IEEE Computer Society Press",
   Year = 1991,
  month = may,
  address = {Arlington, TX},
 
  }

@proceedings{icdcs93,
 booktitle = proc #" 13th "# icdcs,
title = proc #" 13th"# icdcs,
publisher = "IEEE Computer Society Press",
   Year = 1993,
  month = may,
  address = "Pittsburgh ",
 
  }

@proceedings{icdcs94,
 booktitle = proc #" 14th "# icdcs,
publisher = "IEEE Computer Society Press",
   Year = 1994,
  month = " ",
  address = " ",
 
  }



@proceedings{icdcs96,
   booktitle = proc #" 16th "# icdcs,
  publisher = "IEEE Computer Society Press",
  month = " ",
  Year = 1996,
  confaddress = "",
  
  }
@proceedings{icdcs97,
 year =        {1997},
  address =     {Baltimore, USA},
   booktitle = proc #" 17th "# icdcs,
  publisher = "IEEE Computer Society Press",
  month =       may
}
@proceedings{icdcs98,
   booktitle = proc #" 18th "# icdcs,
    Year = 1998,
  confaddress = "",
month= may,
  publisher = "IEEE Computer Society Press",
  }


@proceedings{icdcs00,
   booktitle = proc #" 20th "# icdcs,
    month = apr,
  Year = 2000,
  confaddress = "",
  publisher = "IEEE Computer Society Press",
  }

@proceedings{icdcs01,
   booktitle = proc #" 21th "# icdcs,
  month = apr,
  Year = 2001,
  confaddress = "Mesa, Arizona",
publisher = "IEEE Computer Society Press",
 }





-----------------------------------------------------------------------------
		  
@InProceedings{WanZuc89,
        author =       "D. Wang and L. Zuck",
        title =        "Tight Bounds for the Sequence Transmission Problem",
        booktitle =     proc # " 8th " # podc,
        pages =         "73--83",
        month = aug,
        year =         "1989",
        confaddress = "Edmonton, Alb., Canada",
      }





@Article{CMT96,
        author =  "B. Charron-Bost and F. Mattern and G. Tel",
        title =  "Synchronous and Asynchronous Communications in Distributed
                  Computations",
        journal=  "Distributed Computing", 
        volume = "9",
        number = "4",
        year = "1996",
        pages = "173--191",
       }

@incollection{Dij72,
  Author = "Dijkstra, E.W.",
  Title = "Hierarchical Ordering of Sequential Processes",
  Booktitle = "Operating System Techniques",
  editor = "C.A.R. Hoare and R.H. Perrot",
  publisher = "Academic Press",
  Year = "1972",
  pages = "72--93"
  }

@incollection{LL90,
  Author = "Lamport, Leslie and Nancy A. Lynch",
  Title = "Distributing Computing: Models and Methods",
  Booktitle = "Handbook of Theoretical Computer Science",
  editor = "J. van Leeuwen",
  publisher = "Elsevier Science Publishers B. V.",
  Year = "1990",
  pages = "1158--1198"
  }

@article{LAA87,
  Author = "Loui, M. C. and Abu-Amara, H. A.",
  Title = "Memory requirements for agreement among unreliable
                  asynchronous processes ",
  Journal = "Advances in Computing Research",
  Editor = "Franco P. Preparata",
  Year = 1987,
  volume = 4,
  pages = "163--183"
  }


@Article{Fra80 ,
    Author = "N. Francez" ,
    Title = "Distributed Termination",
    Journal = toplas, 
    volume = 2 ,
    number = 1,
    Year = 1980 ,
    Pages = "42--55" 
         }

@Article{LY87,
    Author = "Lai, T.~H. and Yang, T.~H.",
    Title = "On distributed snapshots",
    Journal = ipl,
    volume = 25,
    Year = 1987,
    Pages = "153--158"
       }


@Article{Dij87,
    Author = "Dijkstra, E.~W.",
    Title = "Shmuel Safra's version of  termination detection",
    Journal = {EWD-Note},
    volume = 998,
    Year = 1987
       }
%PERSO-----------------------------------
}




@inproceedings{delporte09adversary,
  author    = {Carole Delporte-Gallet and
               Hugues Fauconnier and
               Rachid Guerraoui and
               Andreas Tielmann},
  title     = {The Disagreement Power of an Adversary},
  booktitle = {DISC},
  year      = {2009},
  pages     = {8-21}
}


@techreport{DF98,
 
  Title = "Synchronized Phase Systems",
  Author= "Carole Delporte-Gallet and Hugues Fauconnier",
  Institution = liafa,
  month = oct,
  Year = 1998,
  }


@inproceedings{DFG05-disc,
  author    = {Carole Delporte-Gallet and
               Hugues Fauconnier and
               Rachid Guerraoui},
  title     = {(Almost) All Objects Are Universal in Message Passing Systems.},
  booktitle = disc,
  year      = {2005},
  pages     = {184-198}
}
		  
# Conference international avec comite de lecture

% 
@Article{HHMRT00,
  author = 	 { Jean-Michel H\'{e}lary and  Michel Hurfin and  Achour Mostefaoui and Michel Raynal and Frdric
Tronel },
  title = 	 {Computing Global Functions in Asynchronous Distributed Systems with Perfect Failure
     Detectors},
  journal = 	 {IEEE Transactions on Parallel and Distributed Systems},
  year = 	 {2000 },
  volume = 	 {11},
  number = 	 {9},
pages= "897--909",
  month = 	 sep,
}

@InProceedings{G2000,
  author = 	 {Guerraoui, Rachid},
  title = 	 {Indulgent algorithms},
  booktitle = 	 {PODC' 00: Proceedings of the Nineteenth Annual ACM Symp. on Principles of Distributed Computing, Portland, Oregon, USA },
   pages = 	 {289-297},
  year = 	 {2000},
  month = 	 jul,
  organization = {ACM},
}

@InProceedings{QOS2000,
  author = 	 {Chen,W. and Toueg, S. and Aguilera, M. K.},
  title = 	 {On the Quality of Service of Failure Detectors},

  booktitle = 	{Proceedings of the 2000 International Conference on Dependable Systems and Networks (ICDSN/FTCS-30)},
  year = 	 {2000},
  month = 	 jun,
}


    
@Article{QOS2002,
  author = 	 {Chen,W. and Toueg, S. and Aguilera, M. K.},
  title = 	 {On the Quality of Service of Failure Detectors},
   journal = 	 {IEEE Transactions on computers},
  year = 	 {2002},
  volume = 	 {1},
  number = 	 {51},
  pages = 	 {13--32},
  month = 	 jan,

}

@Article{AT99,
  author = 	 {Aguilera, M. K. and Toueg, S.},
  title = 	 {A Simple Bivalency Proof that t-Resilient Consensus Requires t + 1 Round},
  journal = 	 {Information Processing Letters},
  year = 	 1999,
  volume =	 71,
  number =	 {3-4},
  pages =	 {155-158}
}


% genuine multicast

@inproceedings{GS97f,
  year =        {1997},
  address =     {Baltimore, USA},
  pages =       {578-585},
  title =       {Total order multicast to multiple groups},
  author =      {Guerraoui, R. and Schiper, A.},
  booktitle =   {Proceedings of the 17th International Conference on Distributed Computing Systems (ICDCS-17)},
  keywords =    {FT_principles},
  month =       may
}
@article{GS00,
  Author = "Guerraoui, R. and Schiper, A.",
  Title = "Genuine Atomic Multicast in Asynchronous Distributed Systems",
  Journal = tcs,
  Year = 2000,
volume = 254,
number= "1-2",
pages="297--316",

  } 


@article{GS01,
  Author = "Guerraoui, R. and Schiper, A.",
  Title = "Generic Consensus Service",
  Journal = "IEEE Transactions on Software Engineering",
  Year = 2001,
Volume =28,
number= 1,
pages= "29--41",
  
  }  

@inproceedings{DFGHKT04,
 author = {Carole Delporte-Gallet and Hugues Fauconnier and Rachid Guerraoui and Vassos Hadzilacos and Petr Koutnetzov and Sam Toueg},       
title = {The Weakest Failure Detectors to Solve Certain Fundamental Problems in Distributed Computing},
 booktitle   = {Proceedings of the 23th ACM Symp. on Principles of Distributed Computing},
  Year = {2004}
 }

@Unpublished{S85,
  Author = "D. Skeen",
  title = "unpublished communication",
  month = feb,
  Year = 1985,
  note= "The Skeen's algorithm",

  }

@InProceedings{MRT00,
  author = 	 {Mostefaoui, Achour and  Raynal, Michel and Tronel, Frederic },
  title = 	 {The Best of Both Worlds: A Hybrid Approach to Solve Consensus},
  booktitle = 	 {Proceedings of the International Conference on Dependable Systems and Networks},
  year = 	 {2000},
publisher = "IEEE Computer Society Press",

}

@inproceedings{MRT06,
  author    = {Achour Most{\'e}faoui and
               Michel Raynal and
               Corentin Travers},
  title     = {Exploring Gafni's Reduction Land: From {\it mega}$^{\mbox{{\it }}}$
               to Wait-Free Adaptive (2p-[p/k])-Renaming Via k-Set Agreement},
  booktitle = {DISC},
  year      = {2006},
  pages     = {1-15}
}



@InProceedings{Gaf98,
  author =       "Gafni, Eli",
  title =        "Round-by-Round Fault Detectors (extended abstract):
                 Unifying Synchrony and Asynchrony",
  booktitle = proc #    " 17th Symp. on Principles
                 of Distributed Computing",
  year =         "1998",
}


@InProceedings{Z06,
  author =       "Zieli\'nski, Piotr",
  title =        "Optimistically Terminating Consensus",
  booktitle = proc #    " IEEE International Symp. on Parallel and Distributed Computing ",
  year =         "2006",
}


@InProceedings{CBGS00,
  author =       "Bernadette Charron-Bost and Rachid Guerraoui and
                 {Andr\'e} Schiper",
  title =        "Synchronous System and Perfect Failure Detector:
                 Solvability and Efficiency Issues",
  booktitle =    "International Conference on Dependable Systems and
                 Networks (IEEE Computer Society)",
  year =         "2000",
  annote =       "Looks at the relation between the synchronous system
                 model and the asynchronous model augmented with perfect
                 failure detectors. They show that there are problems
                 which are solvable in synchronous systems but are
                 unsolvable in asynchronous systems with perfect failure
                 detectors. Hence, both models are not equivalent in
                 this respect. This is because failure detectors give no
                 information on the causal relation between the crash
                 event and other events on the crashed process. This
                 means that you cannot decide whether there is still a
                 message in transit coming from the crashed process or
                 not. If you want to base a decision on this fact you
                 have the same dilemma as in FLP
                 \cite{Fischer:1985:IDC}. But if it comes to consensus,
                 both models are ok because you can solve this problem
                 in both. However, in synchronous systems algorithms can
                 be constructed with a lower latency degree
                 \cite{Schiper:1997:ECA} so more efficient solutions are
                 possible in the synchronous model.",
}

@Article{DFN90,
  author       = {Delporte-Gallet, Carole and Fauconnier, Hugues and Nivat, Maurice},
  title        = {Paralllisation d'algorithmes avec un nombre fixe de processeurs},
  journal      = {rairo},
  pubtype      =  art_avec_comite,
  year         = {1990},
  volume       = {24},
  number       = {4},
  pages        = {353--386},
}                                                                              
@article{ChaDelFau95,
  author        = "Charron-Bost, Bernadette and Delporte-Gallet, Carole and Fauconnier, Hugues",
  title         = "Local and Temporal Predicates in Distributed System",
  journal       = "ACM TOPLAS",
  pubtype       =  art_avec_comite,
  month         = jan,
  year          = 1995,
  page          =  "157--179 ",
}
@inproceedings{DGF97a,
  author        = {Delporte-Gallet, Carole and Fauconnier, Hugues},
  title         = {Un algorithme de consensus r{\'e}sistant aux pannes d{\'e}finitives de processus et aux pertes de messages},
  pubtype       = coll_avec_comite,
  booktitle     = "Proceedings of RenPar'9 ",
  place         = {Lausanne,Swiss},
  year          = 1997,
}
 
@INPROCEEDINGS{phasedtm,
    author = {Yossi Lev and Mark Moir and Dan Nussbaum},
    title = {PhTM: Phased transactional memory},
    booktitle = {In Workshop on Transactional Computing (Transact), 2007. research.sun.com/scalable/pubs/ TRANSACT2007PhTM.pdf},
    year = {}
}

@inproceedings{DelFau99b,
  author        = {Delporte-Gallet, Carole and Fauconnier, Hugues},
  title         = {Synchronized phases systems },
  pubtype       = coll_avec_comite,
  booktitle     = proc # " 3th International Conference on Principles of Distributed Computing",
  year          = 1999,
  place         = {Hanoi,Vietnam}
 }
 
@inproceedings{DelFau99a,
  author        = "Delporte-Gallet, Carole and Fauconnier, Hugues",
  title         = "Real-Time fault Tolerant Atomic Broadcast",

  booktitle     = proc # " 18th " # "IEEE Symp. on Reliable Distributed Systems ",
  year          = 1999,
  pages         = "48-55",
  place         = "Lausanne,Swiss",
}                                                                                                            
@inproceedings{DelFau00,
  author        = {Delporte-Gallet, Carole and Fauconnier, Hugues},
  title         = {Fault-tolerant genuine atomic multicast to multiple groups},
  booktitle     = proc #  " 4th International Conference on Principles of Distributed Computing",
  year          = 2000,
  pages 	= "107--122",
  place         = {Paris, France},
 }  
 
@TechReport{GHKT04,
  author = 	 {Guerraoui, Rachid and Hadzilacos, Vassos and Koutnetzov, Petr and Toueg, Sam},
  title = 	 {The Weakest Failure Dectectors for Quittable Consensus and Non-Blocking Atomic Commit},
  institution =  {EPFL},
 
  year = 	 {2004},
 
}

@inproceedings{DGFHR02,
  author = 	 {Delporte-Gallet, Carole and Fauconnier, Hugues
and H\'{e}lary, Jean-Michel and Raynal, Michel},
  title = 	 {Early Stopping in Global Data Computing},
   crossref = "podc02",
    pages = "258",
  }


@Article{DGFHR03,
  author = 	 {Delporte-Gallet, Carole and Fauconnier, Hugues
and H\'{e}lary, Jean-Michel and Raynal, Michel},
  title = 	 {Early Stopping in Global Data Computing},
  journal =  {IEEE, Transactions On Parallel and Distributed Systems},
  year = 	 {2002},
  note = 	 {(to appear 2003},
}

@inproceedings{DelFau99c,
  author       = "Delporte-Gallet, Carole and Fauconnier, Hugues",
  title        = "Lower Bounds with Unreliable Failure Detector",
  booktitle    = proc # "13th" # " International Symp. on Distributed Computing, brief announcements", 
  year         = 1999,
  place        = "Bratislava,Slovacia",
}
		  
		  
#rapport ATR
@techreport{ATR1,
  author         = "AXLOG and  Dassault Aviation and  INRIA and LIAFA and  LIX
and  LMC-IMAG and  Thomson-CSF",
  title         = "Exemple de problmes applicatifs de type consensus ou de type diffusion atomique temps-rel,
spcification du problme tudi, Rapport tranche ferme contrat {ATR}",
  institution    = " DRET/MENESR/CNRS",
  pubtype        =  rapport,
  year		 = 1997,	  
		 
}



@techreport{ATR2,
		  
  author         = "Charron-Bost, Bernadette and Delporte, Carole and Fauconnier, Hugues and Le Lann, Gerard and Minet, Pascale",
  title          = "Rapport intermediaire 1.1",
  note           = "Rapport tranche ferme contrat ATR",
  institution    = " DRET/MENESR/CNRS",
  pubtype        =  ?,
  year		 = 1997,	  
		 
}
@techreport{ATR3,
		  
  author         = "Charron-Bost, Bernadette and Delporte, Carole and Fauconnier, Hugues and Le Lann, Gerard and Minet, Pascale",
  title          = "Rapport intermediaire 1.2A",
  note           = "Rapport tranche ferme contrat ATR",
  institution    = " DRET/MENESR/CNRS",
  year		 = 1997, 
  pubtype        =  rapport,
		 
}
@techreport{ATR4,
		  
  author         = "Charron-Bost, Bernadette and Delporte, Carole and Fauconnier, Hugues and Le Lann,Gerard and Minet, Pascale",
  title          = "Rapport final",
  note           = "Rapport tranche ferme contrat ATR", 
  institution    = " DRET/MENESR/CNRS",
  year		= 1997,	  
  pubtype        =  rapport,
		 
}
@techreport{ATR99,
		  
  author         = "AXLOG and  Dassault Aviation and  INRIA and LIAFA and 
 LIX and  LMC-IMAG and Thomson-CSF",
  title          = "Rapport final",
  note           = "Rapport tranche conditionnel  contrat ATR", 
  institution    = " DRET/MENESR/CNRS",
  year		= 1999,	  
  pubtype        =  rapport,
		 
}	
	 

 	  


@inproceedings{DelFau01,
  author        = {Delporte-Gallet, Carole and Fauconnier, Hugues},
  title         =  {An example of Real-Time Group Communication System},
  booktitle = proc # " 21th IEEE International Conference on Distributed Computing Systems Workshops",
  year          = 2001,
  place         = {Mesa, Arizona},
  pages         = {5--10},

}
		  



@InProceedings{DFG02,
  author = 	 {Delporte-Gallet, Carole and  Fauconnier, Hugues and Guerraoui, Rachid},
  title = 	 {A Realistic Look at Failure Detectors},
  booktitle = 	 {Proceedings of the 2002 International Conference on Dependable Systems and Networks  },
  year = 	 {2002},
  month = 	 jun,
place ={Washington, DC},
page={345--353}
}




@InProceedings{DFG02b,

  title = 	 {Failure Detection Lower Bounds on Registers and Consensus},
  year = 	 {2002},

  booktitle    = proc # " 16th International Symp. on Distributed Computing",
  series = {LNCS 2508},

    place={Toulouse, France},
  page={237--252},
  author = "Delporte-Gallet, Carole and  Fauconnier, Hugues and Guerraoui, Rachid", 
}




@TechReport{DFG05,
  author = 	 {Delporte-Gallet, Carole and  Fauconnier, Hugues and Guerraoui, Rachid},
  title = 	 {Implementing Atomic Objects in a Message Passing System},
  institution =  {EPFL Lausanne},
  year = 	 {2005}
}

@TechReport{DFG03,
  author = 	 {Delporte-Gallet, Carole and  Fauconnier, Hugues and Guerraoui, Rachid},
  title = 	 {Shared Memory vs Message Passing},
  institution =  {EPFL Lausanne},
  year = 	 {2003},
  number = 	 {200377},
}

@Article{DGFGK02a,
  author = 	 {Delporte-Gallet, Carole and  Fauconnier, Hugues and Guerraoui, Rachid and Kouztnetsov, Pietr },
  title = 	 {Mutual exclusion in asynchronous systems with
  failure detector},
  journal = 	 {Journal of Parallel and 
Distributed Computing},
  year = 	 {2005},
}

@article{JM07-cores,
  author    = {Flavio Junqueira and
               Keith Marzullo},
  title     = {A framework for the design of dependent-failure algorithms},
  journal   = {Concurrency and Computation: Practice and Experience},
  volume    = {19},
  number    = {17},
  year      = {2007},
  pages     = {2255-2269}
}


@article{GK10-arxiv,
  author    = {Eli Gafni and Petr Kuznetsov},
  title     = {{$L$-resilient adversaries and hitting sets}},
  journal   = {CoRR},
  volume    = {abs/1004.4701},
  year      = {2010},
  note = {http://arxiv.org/abs/1004.4701, to appear in ICDCN 2011},
  ee        = {http://arxiv.org/abs/1004.4701}
}


@article{GKR13-TR,
  author    = {Vincent Gramoli and
               Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {Optimistic Transactions vs. Pessimistic Locks },
  journal   = {CoRR},
  volume    = {abs/1203.4751},
  year      = {2012}
}


@InProceedings{HR10,
  author = 	 {Maurice Herlihy and Sergio Rajsbaum},
  title = 	 {The Topology of Shared-Memory Adversaries},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {PODC},
  OPTpages = 	 {},
  year = 	 {2010},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@inproceedings{IR09-rap,
  author    = {Damien Imbs and
               Michel Raynal},
  title     = {Visiting Gafni's Reduction Land: From the BG Simulation
               to the Extended BG Simulation},
  booktitle = {SSS},
  year      = {2009},
  pages     = {369-383}
}

@InProceedings{IRT10-asym,
  author = 	 {Damien Imbs and Michel Raynal and Gadi Taubenfeld},
  title = 	 {On asymmetric progress conditions},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {PODC},
  OPTpages = 	 {},
  year = 	 {2010},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}



@TechReport{GG09,
  author = 	 {Eli Gafni and Rachid Guerraoui},
  title = 	 {Simulating Few by Many: Limited Concurrency = Set Consensus},
  OPTinstitution =  {},
  year = 	 {2009},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTnumber = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Tau10,
  author = 	 {Gadi Taubenfeld},
  title = 	 {The computational structure of progress conditions},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {DISC},
  OPTpages = 	 {},
  year = 	 {2010},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTannote = 	 {}
}


@TechReport{GG10,
  author = 	 {Eli Gafni and Rachid Guerraoui},
  title = 	 {Generalizing State Machine Replication},
  institution =  {EPFL},
  year = 	 {2010},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTnumber = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  note = 	 {http://infoscience.epfl.ch/record/150307},
  OPTannote = 	 {}
}
@inproceedings{TM-theory,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {Transactional Memory: Glimmer of a Theory},
 booktitle = {Proceedings of the 21st International Conference on Computer Aided Verification},
 series = {CAV '09},
 year = {2009},
 isbn = {978-3-642-02657-7},
 location = {Grenoble, France},
 pages = {1--15},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-02658-4_1},
 doi = {http://dx.doi.org/10.1007/978-3-642-02658-4_1},
 acmid = {1575062},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 

@inproceedings{GK08-opacity,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {On the Correctness of Transactional Memory},
 booktitle = {Proceedings of the 13th ACM SIGPLAN Symp. on Principles and Practice of Parallel Programming},
 series = {PPoPP '08},
 year = {2008},
 isbn = {978-1-59593-795-7},
 location = {Salt Lake City, UT, USA},
 pages = {175--184},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1345206.1345233},
 doi = {10.1145/1345206.1345233},
 acmid = {1345233},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {correctness, lower bound, model, transactional memory},
} 



@inproceedings{GHS08-permissiveness,
  author    = {Rachid Guerraoui and
               Thomas A. Henzinger and
               Vasu Singh},
  title     = {Permissiveness in Transactional Memories},
  booktitle = {DISC},
  year      = {2008},
  pages     = {305-319}
}



@InProceedings{AGK11-popl,
  author = 	 {Hagit Attiya and Rachid Guerraoui and Danny Hendler and Petr Kuznetsov 
and Maged Michael and Martin Vechev},
  title = 	 {Laws of Order: Expensive Synchronization in Concurrent Algorithms Cannot be Eliminated},
  booktitle = 	 {POPL},
 year = 	 {2011},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {http://www.net.t-labs.tu-berlin.de/$\sim$petr/pubs/fences.pdf},
  OPTannote = 	 {},
  pages = {487-498},
}

@inproceedings{MS96,
  author    = {Maged M. Michael and
               Michael L. Scott},
  title     = {Simple, Fast, and Practical Non-Blocking and Blocking Concurrent
               Queue Algorithms},
  booktitle = {PODC},
  year      = {1996},
  pages     = {267-275},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}



@article{Lamport74-bakery,
  author    = {Leslie Lamport},
  title     = {{A New Solution of Dijkstra's Concurrent Programming Problem}},
  journal   = {Commun. ACM},
  volume    = {17},
  number    = {8},
  year      = {1974},
  pages     = {453-455}
}

@article{anderson-90-tpds,
  author    = {Thomas E. Anderson},
  title     = {The Performance of Spin Lock Alternatives for Shared-Memory
               Multiprocessors},
  journal   = {IEEE Trans. Parallel Distrib. Syst.},
  volume    = {1},
  number    = {1},
  year      = {1990},
  pages     = {6-16}
}

@article{GK09-progressiveness,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {The Semantics of Progress in Lock-based Transactional Memory},
 journal = {SIGPLAN Not.},
 issue_date = {January 2009},
 volume = {44},
 number = {1},
 month = jan,
 year = {2009},
 issn = {0362-1340},
 pages = {404--415},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/1594834.1480931},
 doi = {10.1145/1594834.1480931},
 acmid = {1480931},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {consensus number, impossibility, lock, lower bound, reduction, semantics, transactional memory, try-lock},
} 

@inproceedings{imbs-raynal,
 author = {Imbs, Damien and Raynal, Michel},
 title = {A Lock-Based STM Protocol That Satisfies Opacity and Progressiveness},
 booktitle = {Proceedings of the 12th International Conference on Principles of Distributed Systems},
 series = {OPODIS '08},
 year = {2008},
 isbn = {978-3-540-92220-9},
 location = {Luxor, Egypt},
 pages = {226--245},
 numpages = {20},
 url = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 doi = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 acmid = {1496328},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {Atomic operation, Commit/abort, Concurrency control, Consistent global state, Lock, Opacity, Progressiveness, Shared object, Software transactional memory, Transaction},
}

@inproceedings{mv-permissive,
 author = {Attiya, Hagit and Hillel, Eshcar},
 title = {Brief announcement: single-version permissive {STM}},
 booktitle = {Proceeding of the 29th ACM SIGACT-SIGOPS Symp. on Principles of distributed computing},
 series = {PODC '10},
 year = {2010},
 isbn = {978-1-60558-888-9},
 location = {Zurich, Switzerland},
 pages = {67--68},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/1835698.1835712},
 doi = {http://doi.acm.org/10.1145/1835698.1835712},
 acmid = {1835712},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {permissiveness, transactional memory},
} 
 

@BOOK(tm-book,
	AUTHOR		= "Guerraoui, Rachid and  Kapalka, Michal",
	TITLE		= "Principles of Transactional Memory,Synthesis Lectures on Distributed Computing Theory",
	PUBLISHER	= "Morgan and Claypool",
	YEAR		= "2010")

@article{jaytoueg,
 author = {Jayanti, Prasad and Tan, King and Toueg, Sam},
 title = {Time and Space Lower Bounds for Nonblocking Implementations},
 journal = {SIAM J. Comput.},
 volume = {30},
 issue = {2},
 month = {April},
 year = {2000},
 issn = {0097-5397},
 pages = {438--456},
 numpages = {19},
 url = {http://portal.acm.org/citation.cfm?id=586848.587007},
 doi = {10.1137/S0097539797317299},
 acmid = {587007},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 keywords = {asynchronous shared memory algorithms, lower bounds, nonblocking, randomized shared object implementations, space complexity, synchronization, time complexity, wait-free},
} 


@article{burnslynch,
 author = {Burns, James E. and Lynch, Nancy A.},
 title = {Bounds on shared memory for mutual exclusion},
 journal = {Inf. Comput.},
 volume = {107},
 issue = {2},
 month = {December},
 year = {1993},
 issn = {0890-5401},
 pages = {171--184},
 numpages = {14},
 url = {http://portal.acm.org/citation.cfm?id=175991.175992},
 doi = {10.1006/inco.1993.1065},
 acmid = {175992},
 publisher = {Academic Press, Inc.},
 address = {Duluth, MN, USA},
} 

@techreport{michel-permissive,
    HAL_ID = {inria-00533620},
    URL = {http://hal.inria.fr/inria-00533620/en/},
    title = { {R}ead invisibility, virtual world consistency and permissiveness are compatible},
    author = {{C}rain, {T}yler and {I}mbs, {D}amien and {R}aynal, {M}ichel},
    language = {{E}nglish},
    institution = {{ASAP} - {INRIA} - {IRISA} - {CNRS} : {UMR}6074 - {INRIA} - {I}nstitut {N}ational des {S}ciences {A}ppliqu{\'e}es de {R}ennes - {U}niversit{\'e} de {R}ennes {I} },
    pages = {21 },
    type = {{R}esearch {R}eport},
    month = {11},
    year = {2010},
    URL = {http://hal.inria.fr/inria-00533620/PDF/PI-1958.pdf},
}

@article{Pap79-serial,
 author = {Papadimitriou, Christos H.},
 title = {The serializability of concurrent database updates},
 journal = {J. ACM},
 volume = {26},
 issue = {4},
 year = {1979},
 issn = {0004-5411},
 pages = {631--653},
 numpages = {23},
 url = {http://doi.acm.org/10.1145/322154.322158},
 doi = {http://doi.acm.org/10.1145/322154.322158}, 
acmid = {322158},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{help15,
  author    = {Keren Censor{-}Hillel and
               Erez Petrank and
               Shahar Timnat},
  title     = {Help!},
  booktitle = {Proceedings of the 2015 {ACM} Symp. on Principles of Distributed
               Computing, {PODC} 2015, Donostia-San Sebasti{\'{a}}n, Spain,
               July 21 - 23, 2015},
  pages     = {241--250},
  year      = {2015},
  url       = {https://doi.org/10.1145/2767386.2767415},
  doi       = {10.1145/2767386.2767415},
  timestamp = {Tue, 06 Nov 2018 11:07:19 +0100},
  biburl    = {https://dblp.org/rec/conf/podc/Censor-HillelPT15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:jattiya-help,
  author    = {Hagit Attiya and
               Armando Casta{\~{n}}eda and
               Danny Hendler},
  title     = {Nontrivial and universal helping for wait-free queues and stacks},
  journal   = {J. Parallel Distributed Comput.},
  volume    = {121},
  pages     = {1--14},
  year      = {2018},
  url       = {https://doi.org/10.1016/j.jpdc.2018.06.004},
  doi       = {10.1016/j.jpdc.2018.06.004},
  timestamp = {Sat, 22 Feb 2020 19:35:43 +0100},
  biburl    = {https://dblp.org/rec/journals/jpdc/AttiyaCH18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{QueueFriedman18,
  author    = {Michal Friedman and
               Maurice Herlihy and
               Virendra J. Marathe and
               Erez Petrank},
  editor    = {Andreas Krall and
               Thomas R. Gross},
  title     = {A persistent lock-free queue for non-volatile memory},
  booktitle = {Proceedings of the 23rd {ACM} {SIGPLAN} Symp. on Principles and
               Practice of Parallel Programming, PPoPP 2018, Vienna, Austria, February
               24-28, 2018},
  pages     = {28--40},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3178487.3178490},
  doi       = {10.1145/3178487.3178490},
  timestamp = {Tue, 06 Nov 2018 16:57:28 +0100},
  biburl    = {https://dblp.org/rec/conf/ppopp/FriedmanHMP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{NestingSafe18,
  author    = {Hagit Attiya and
               Ohad Ben{-}Baruch and
               Danny Hendler},
  editor    = {Calvin Newport and
               Idit Keidar},
  title     = {Nesting-Safe Recoverable Linearizability: Modular Constructions for
               Non-Volatile Memory},
  booktitle = {Proceedings of the 2018 {ACM} Symp. on Principles of Distributed
               Computing, {PODC} 2018, Egham, United Kingdom, July 23-27, 2018},
  pages     = {7--16},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3212734.3212753},
  doi       = {10.1145/3212734.3212753},
  timestamp = {Mon, 16 Sep 2019 15:23:07 +0200},
  biburl    = {https://dblp.org/rec/conf/podc/AttiyaBH18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{AH13-inv,
   author = {Attiya, Hagit and Hillel, Eshcar},
  journal = {IEEE Trans. Computers},
  keywords = {dblp},
  number = 12,
  pages = {2531-2543},
  title = {The Cost of Privatization in Software Transactional Memory},
  volume = 62,
  year = 2013
}
@inproceedings{DS10-rwlock,
  author    = {David Dice and
               Nir Shavit},
  title     = {{TLRW:} return of the read-write lock},
  booktitle = {{SPAA}},
  pages     = {284--293},
  year      = {2010}
}

@inproceedings{israeli-disjoint,
 author = {Israeli, Amos and Rappoport, Lihu},
 title = {Disjoint-access-parallel implementations of strong shared memory primitives},
 booktitle = {PODC},
 year = {1994},
 pages = {151--160},
} 

@article{AHM09,
year={2011},
issn={1432-4350},
journal={Theory of Computing Systems},
volume={49},
number={4},
doi={10.1007/s00224-010-9304-5},
title={Inherent Limitations on Disjoint-Access Parallel Implementations of Transactional Memory},
url={http://dx.doi.org/10.1007/s00224-010-9304-5},
publisher={Springer-Verlag},
keywords={Transactional memory; Disjoint-access parallelism; Partial snapshots; Lower bound; Impossibility result},
author={Attiya, Hagit and Hillel, Eshcar and Milani, Alessia},
pages={698-719},
language={English}
}

@inproceedings{DStransaction06,
 author = {Dice, Dave and Shavit, Nir},
 title = {What really makes transactions fast?},
 booktitle = {Transact},
 year = {2006}
 
} 

@article{attiyaH13,
  added-at = {2014-01-22T00:00:00.000+0100},
  author = {Attiya, Hagit and Hillel, Eshcar},
  biburl = {http://www.bibsonomy.org/bibtex/2b4825fd9aba8c48baf75b7db390d1aff/dblp},
  ee = {http://doi.ieeecomputersociety.org/10.1109/TC.2012.159},
  interhash = {68c7a4e4558e3a0dc5bf9d981783f4c0},
  intrahash = {b4825fd9aba8c48baf75b7db390d1aff},
  journal = {IEEE Trans. Computers},
  keywords = {dblp},
  number = 12,
  pages = {2531-2543},
  timestamp = {2014-01-22T00:00:00.000+0100},
  title = {The Cost of Privatization in Software Transactional Memory.},
  url = {http://dblp.uni-trier.de/db/journals/tc/tc62.html#AttiyaH13},
  volume = 62,
  year = 2013
}

@inproceedings{AH11-perm,
  author    = {Hagit Attiya and
               Eshcar Hillel},
  title     = {Single-Version {STM}s Can Be Multi-version Permissive (Extended
               Abstract)},
  booktitle = {ICDCN},
  year      = {2011},
  pages     = {83-94}
}

@book{WV02-book,
  author    = {Gerhard Weikum and
               Gottfried Vossen},
  title     = {Transactional Information Systems: Theory, Algorithms, and
               the Practice of Concurrency Control and Recovery},
  publisher = {Morgan Kaufmann},
  year      = {2002},
  isbn      = {1-55860-508-8},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}



@article{AdveG96,
  title={Shared memory consistency models: A tutorial},
  author={Sarita V. Adve and Kourosh Gharachorloo},
  journal={IEEE Computer},
  volume={29},
  number={12},
  pages={66--76},
  year={1996}
}

@PHDTHESIS{Lee99,
  AUTHOR =       {Jaejin Lee},
  TITLE =        {Compilation Techniques for Explicitly Parallel Programs},
  SCHOOL =       {Department of Computer Science,
                    University of Illinois at Urbana-Champaign},
  YEAR =         1999,
}

@UNPUBLISHED{McKenney10,
  AUTHOR =       {Paul E. McKenney},
  TITLE =        {Memory Barriers: a Hardware View for Software Hackers},
  NOTE =         {Linux Technology Center, IBM Beaverton},
  year =         2010,
  month =        jun,
  source =       {http://www.rdrop.com/users/paulmck/scalability/paper/whymb.2010.06.07c.pdf},
}

@Book{Ray86,
  author = 	 {Michel Raynal},
  title = 	 {Algorithms for Mutual Exclusion},
  publisher = 	 {MIT Press},
  year = 	 {1986},
  OPTkey = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTedition = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@inproceedings{GK08-OFT,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {On obstruction-free transactions},
 booktitle = {Proceedings of the twentieth annual Symp. on Parallelism in algorithms and architectures},
 series = {SPAA '08},
 year = {2008},
 isbn = {978-1-59593-973-9},
 location = {Munich, Germany},
 pages = {304--313},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1378533.1378587},
 doi = {http://doi.acm.org/10.1145/1378533.1378587},
 acmid = {1378587},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {consensus number, impossibility, obstruction-freedom, transactional memory},
} 

@article{KR11-TR,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  journal   = {CoRR},
  volume    = {abs/1103.1302},
  year      = {2011},
  ee        = {http://arxiv.org/abs/1103.1302}
}

@article{icdcs-opacity,
author = {Hagit Attiya and Sandeep Hans and Petr Kuznetsov and Srivatsan Ravi},
title = {Safety of Deferred Update in Transactional Memory},
journal ={2013 IEEE 33rd International Conference on Distributed Computing Systems},
volume = {0},
issn = {1063-6927},
year = {2013},
pages = {601-610},
doi = {http://doi.ieeecomputersociety.org/10.1109/ICDCS.2013.57},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@inproceedings{KR11,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  booktitle = {OPODIS},
  year      = {2011},
  pages     = {112-127},
  note      = {full version: http://arxiv.org/abs/1103.1302}
}


@inproceedings{HendlerIST10,
  author    = {Danny Hendler and
               Itai Incze and
               Nir Shavit and
               Moran Tzafrir},
  title     = {Flat combining and the synchronization-parallelism tradeoff},
  booktitle = {SPAA},
  year      = {2010},
  pages     = {355-364},
  ee        = {http://doi.acm.org/10.1145/1810479.1810540}
}


@Article{LWN-mckenney,
  author = 	 {Paul McKenney},
  title = 	 {Concurrent code and expensive instructions},
  journal = 	 {Linux Weekly News},
  year = 	 {2011},
  OPTkey = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTpages = 	 {},
  month = 	 {January},
  note = 	 {http://lwn.net/Articles/423994/},
  OPTannote = 	 {}
}

@COMMENT{
   Vincent: Not sure it is the right format, but below are some related pointers.
}

@inproceedings{FML+11,
  author    = {Cesare Ferri and
               Andrea Marongiu and
               Benjamin Lipton and
               R. Iris Bahar and
               Tali Moreshet and
               Luca Benini and
               Maurice Herlihy},
  title     = {{S}o{C}-{TM}: integrated {HW/SW} support for transactional memory
               programming on embedded {MPSoCs}},
  booktitle = {Proceedings of the 9th International Conference on Hardware/Software
               Codesign and System Synthesis (CODES+ISSS)},
  year      = {2011},
  pages     = {39-48},
}

  @article{TMS,
year={2013},
issn={0934-5043},
journal={Formal Aspects of Computing},
volume={25},
number={5},
doi={10.1007/s00165-012-0225-8},
title={Towards formally specifying and verifying transactional memory},
url={http://dx.doi.org/10.1007/s00165-012-0225-8},
publisher={Springer London},
keywords={Transactional memory; Formal specification; Verification; I/O automation; Simulation proof; Refinement},
author={Doherty, Simon and Groves, Lindsay and Luchangco, Victor and Moir, Mark},
pages={769-799},
language={English}
}

@inproceedings{SAH+06,
 author = {Saha, Bratin and Adl-Tabatabai, Ali-Reza and Hudson, Richard L. and Minh, Chi Cao and Hertzberg, Benjamin},
 title = {Mc{RT}-{STM}: a high performance software transactional memory system for a multi-core runtime},
 booktitle = {PPoPP},
 year = {2006},
 pages = {187--197},
} 

@misc{USB09,
  title = {Adaptive Locks: Combining Transactions and Locks for Efficient Concurrency},
  author = {Takayuki Usui and Yannis Smaragdakis and Reimer Behrends},
  year = {2009},
  booktitle = {Transact},
}

@incollection{BS88,
 author = {R. Bayer and M. Schkolnick},
 title = {Concurrency of operations on {B}-trees},
 booktitle = {Readings in database systems},
 year = {1988},
 pages = {129--139},
 publisher = {Morgan Kaufmann Publishers Inc.},
}

@inproceedings{GG11b,
  author = {Vincent Gramoli and Rachid Guerraoui},
  title = {Democratizing Transactional Programming},
  booktitle = {Middleware},
  publisher = {Springer},
  address = {},
  editor = {},
  volume = {7049},
  series = {LNCS},
  year = {2011},
  month = {Dec},
  pages = {1--19},
  url = {http://lpd.epfl.ch/gramoli/doc/pubs/middleware2012-preprint.pdf},
  location = {},
} 

@inproceedings{HK08,
	title = {Transactional Boosting: A Methodology for Highly-Concurrent Transactional Objects},
	author = {Maurice Herlihy and Eric Koskinen},
	booktitle = {PPoPP},
	year = {2008},
	publisher = {ACM}, 
	address = {New York, NY, USA},
} 


@inproceedings{Mos06,
 author = {J. Eliot B. Moss}, 
 title = {Open Nested Transactions: Semantics and Support},
 booktitle = {WMPI}, 
 location = {Austin, TX} ,
 month = {February},
 year = {2006},
}

@article{Gar83,
 author = {Garcia-Molina, Hector},
 title = {Using semantic knowledge for transaction processing in a distributed database},
 journal = {ACM Trans. Database Syst.},
 volume = {8},
 issue = {2},
 month = {June},
 year = {1983},
 pages = {186--213},
} 

@article{Lyn83,
 author = {Lynch, Nancy A.},
 title = {Multilevel atomicity--a new correctness criterion for database concurrency control},
 journal = {ACM Trans. Database Syst.},
 volume = {8},
 issue = {4},
 month = {December},
 year = {1983},
 issn = {0362-5915},
 pages = {484--502},
} 
@inproceedings{HLM+03,
 author = {Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer,III, William N.},
 title = {Software Transactional Memory for Dynamic-sized Data Structures},
 booktitle = {Proceedings of the Twenty-second Annual Symp. on Principles of Distributed Computing},
 series = {PODC '03},
 year = {2003},
 isbn = {1-58113-708-7},
 location = {Boston, Massachusetts},
 pages = {92--101},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/872035.872048},
 doi = {10.1145/872035.872048},
 acmid = {872048},
 publisher = {ACM},
 address = {New York, NY, USA},
} 
 

@ARTICLE{rock,
author={Chaudhry, S. and Cypher, R. and Ekman, M. and Karlsson, M. and Landin, A. and Yip, S. and Zeffer, Håkan and Tremblay, M.},
journal={Micro, IEEE},
title={Rock: A High-Performance Sparc CMT Processor},
year={2009},
month={March},
volume={29},
number={2},
pages={6-16},
keywords={multi-threading;software architecture;aggressive dynamic hardware parallelization;automatic hardware;checkpoint-based architecture;high-performance Sparc CMT processor;sequential instruction stream;software threads;third-generation chip-multithreading processor;transactional memory;Bandwidth;Computer architecture;Control systems;Hardware;Out of order;Parallel processing;Random access memory;Retirement;Throughput;Yarn;integration and modeling;multicore/single-chip multiprocessors;multithreaded processors;parallel architectures;processor architectures;speculative multithreading;system architectures},
doi={10.1109/MM.2009.34},
ISSN={0272-1732},}

@inproceedings{Wei86,
 author = {Weikum, Gerhard},
 title = {A theoretical foundation of multi-level concurrency control},
 booktitle = {PODS},
 year = {1986},
 pages = {31--43},
 numpages = {13},
} 

@inproceedings{FFR08,
 author = {Felber, Pascal and Fetzer, Christof and Riegel, Torvald},
 title = {Dynamic performance tuning of word-based software transactional memory},
 booktitle = {PPoPP},
 year = {2008},
 pages = {237--246},
} 

@inproceedings{MSH+06,
  title = {Lowering the Overhead of Nonblocking Software Transactional Memory},
  author = {Virendra J. Marathe and Michael F. Spear and Christopher Heriot and Athul Acharya and David Eisenstat and William N. Scherer III and Michael L. Scott},
  booktitle = {Transact},
  year = {2006},
 }

@inproceedings{hybridnorec,
  added-at = {2011-03-10T00:00:00.000+0100},
  author = {Dalessandro, Luke and Carouge, François and White, Sean and Lev, Yossi and Moir, Mark and Scott, Michael L. and Spear, Michael F.},
  biburl = {http://www.bibsonomy.org/bibtex/2140e12213aa417d19daa223093dca41d/dblp},
  booktitle = {ASPLOS},
  editor = {Gupta, Rajiv and Mowry, Todd C.},
  ee = {http://doi.acm.org/10.1145/1950365.1950373},
  interhash = {bd7ab35fdfe569cd4699bcca42ef36c3},
  intrahash = {140e12213aa417d19daa223093dca41d},
  isbn = {978-1-4503-0266-1},
  keywords = {dblp},
  pages = {39-52},
  publisher = {ACM},
  timestamp = {2011-03-10T00:00:00.000+0100},
  title = {{Hybrid NOrec: a case study in the effectiveness of best effort hardware transactional memory}},
  url = {http://dblp.uni-trier.de/db/conf/asplos/asplos2011.html#DalessandroCWLMSS11},
  year = 2011
}

@article{norec,
 author = {Dalessandro, Luke and Spear, Michael F. and Scott, Michael L.},
 title = {NOrec: Streamlining STM by Abolishing Ownership Records},
 journal = {SIGPLAN Not.},
 issue_date = {May 2010},
 volume = {45},
 number = {5},
 month = jan,
 year = {2010},
 issn = {0362-1340},
 pages = {67--78},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/1837853.1693464},
 doi = {10.1145/1837853.1693464},
 acmid = {1693464},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {ownership records, software transactional memory, transactional memory, transactional memory models},
} 


 
 @inproceedings{RFF06,
	Author = {Torvald Riegel and Pascal Felber and Christof Fetzer},
	title = {A Lazy Snapshot Algorithm with Eager Validation},
	Booktitle = {DISC},
	Year = {2006},
}

@inproceedings{DSS06,
 author = {Dice, Dave and Shalev, Ori and Shavit, Nir},
 title = {Transactional Locking II},
 booktitle = {Proceedings of the 20th International Conference on Distributed Computing},
 series = {DISC'06},
 year = {2006},
 isbn = {3-540-44624-9, 978-3-540-44624-8},
 location = {Stockholm, Sweden},
 pages = {194--208},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/11864219_14},
 doi = {10.1007/11864219_14},
 acmid = {2136065},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@misc{Her05,
  author = {Maurice Herlihy},
  title = {{SXM}: C\# Software Transactional Memory},
  note = {www.cs.brown.edu/~mph/SXM/README.doc},
  year = {2005},
}

@misc{Rei12,
  author = {James Reinders},
  title = {{Transactional Synchronization in Haswell}},
  note = {\url{http://software.intel.com/en-us/blogs/2012/02/07/transactional-synchronization-in-haswell/}},
  year = {2012},
}



@Misc{bluegene,
  OPTkey = 	 {},
  author = 	 {Martin Ohmacht},
  title = 	 {{Memory Speculation of the Blue Gene/Q Compute Chip}},
  OPThowpublished = {},
  OPTmonth = 	 {},
  year = 	 {2011},
  note = 	 {\url{http://wands.cse.lehigh.edu/IBM_BQC_PACT2011.ppt}},
  OPTannote = 	 {}
}

@Misc{asf,
  OPTkey = 	 {},
  OPTauthor = 	 {},
  title = 	 {{Advanced Synchronization Facility Proposed Architectural Specification}},
  month = 	 {March},
  year = 	 {2009},
  note = 	 {\url{http://developer.amd.com/wordpress/media/2013/09/45432-ASF_Spec_2.1.pdf}},
  OPTannote = 	 {}
}

@inproceedings{Ennals-code,
  author = {Ennals, Robert},
  title = {The Lightweight Transaction library},
  note = {http://sourceforge.net/projects/libltx/files/},
  
}

@inproceedings{riegel-thesis,
  author = {Riegel, Torvald},
  title = {\href{http://www.qucosa.de/fileadmin/data/qucosa/documents/11559/Riegel_Diss_final.pdf}{Software Transactional Memory Building Blocks} },
  
  year = {2013} 
}

@inproceedings{lee-thesis,
  author = {Hyonho, Lee},
  title = {\href{http://www.cs.toronto.edu/pub/hlee/thesis.ps}
  {Local-spin mutual exclusion algorithms on the DSM model using fetch-and-store objects}} ,
  
  year = {2003} 
}

@inproceedings{PA11,
  author    = {Victor Pankratius and
               Ali-Reza Adl-Tabatabai},
  title     = {A study of transactional memory vs. locks in practice},
  booktitle = {SPAA},
  year      = {2011},
  pages     = {43-52},
}


@inproceedings{PFK10,
  author    = {Dmitri Perelman and
               Rui Fan and
               Idit Keidar},
  title     = {On maintaining multiple versions in {STM}},
  booktitle = {PODC},
  year      = {2010},
  pages     = {16-25},
}

@inproceedings{PBLK11,
  author    = {Dmitri Perelman and
               Anton Byshevsky and
               Oleg Litmanovich and
               Idit Keidar},
  title     = {{SMV}: Selective Multi-Versioning {STM}},
  booktitle = {DISC},
  year      = {2011},
  pages     = {125-140},
}


@article{GHF10,
  author = {Vincent Gramoli and Derin Harmanci and Pascal Felber},
  title = {On the Input Acceptance of Transactional Memory},
  journal = {Parallel Processing Letters},
  volume = {20},
  number = {1},
  year = {2010},
  pages = {31--50},
} 


@article{Her90,
 author = {Herlihy, M.},
 title = {Apologizing versus asking permission: optimistic concurrency control for abstract data types},
 journal = {ACM Trans. Database Syst.},
 volume = {15},
 number = {1},
 year = {1990},
 issn = {0362-5915},
 pages = {96--124},
} 

@article{Wei89,
 author = {Weihl, W. E.},
 title = {Local atomicity properties: modular concurrency control for abstract data types},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {11},
 number = {2},
 year = {1989},
 pages = {249--282},
} 

@article{Wei88,
 author = {Weihl, W. E.},
 title = {Commutativity-Based Concurrency Control for Abstract Data Types},
 journal = {IEEE Trans. Comput.},
 volume = {37},
 number = {12},
 year = {1988},
 pages = {1488--1505},
} 

@inproceedings{RMB+93,
 author = {Rastogi, Rajeev and Mehrotra, Sharad and Breitbart, Yuri and Korth, Henry F. and Silberschatz, Avi},
 title = {On correctness of non-serializable executions},
 booktitle = {Proceedings of the twelfth ACM SIGACT-SIGMOD-SIGART Symp. on Principles of database systems},
 year = {1993},
 isbn = {0-89791-593-3},
 pages = {97--108},
} 

@inproceedings{EFKMT12,
  author    = {Faith Ellen and
               Panagiota Fatourou and
               Eleftherios Kosmas and
               Alessia Milani and
               Corentin Travers},
  title     = {Universal constructions that ensure disjoint-access parallelism
               and wait-freedom},
  booktitle = {PODC},
  year      = {2012},
  pages     = {115-124},
}

@INPROCEEDINGS{astm,
    author = {Virendra J. Marathe and William N. Scherer Iii and Michael L. Scott},
    title = {Adaptive Software Transactional Memory},
    booktitle = {In Proc. of the 19th Intl. Symp. on Distributed Computing},
    year = {2005},
    pages = {354--368}
}

@inproceedings{CGLM06,
 author = {Colvin, Robert and Groves, Lindsay and Luchangco, Victor and Moir, Mark},
 title = {Formal verification of a lazy concurrent list-based set algorithm},
 booktitle = {Proceedings of the 18th international conference on Computer Aided Verification},
 year = {2006},
 isbn = {3-540-37406-X, 978-3-540-37406-0},
 pages = {475--488},
 numpages = {14},
} 

@inproceedings{ARR10,
 author = {Attiya, H. and Ramalingam, G. and Rinetzky, N.},
 title = {Sequential verification of serializability},
 booktitle = {Proceedings of the 37th annual ACM SIGPLAN-SIGACT Symp. on Principles of programming languages},
 year = {2010},
 isbn = {978-1-60558-479-9},
 pages = {31--42},
} 

@inproceedings{ORV+10,
 author = {O'Hearn, Peter W. and Rinetzky, Noam and Vechev, Martin T. and Yahav, Eran and Yorsh, Greta},
 title = {Verifying linearizability with hindsight},
 booktitle = {PODC},
 year = {2010},
 pages = {85--94},
} 

@inproceedings{KP79,
 author = {Kung, H. T. and Papadimitriou, C. H.},
 title = {An optimality theory of concurrency control for databases},
 booktitle = {SIGMOD},
 year = {1979},
 pages = {116--126},
} 

@article{Yan84,
 author = {Yannakakis, Mihalis},
 title = {Serializability by Locking},
 journal = {J. ACM},
 volume = {31},
 number = {2},
 year = {1984},
 pages = {227--244},
} 

@book{HLR10,
  author    = {Tim Harris and
               James R. Larus and
               Ravi Rajwar},
  title     = {Transactional Memory, 2nd edition},
  booktitle = {Transactional Memory (2.ed.)},
  publisher = {Morgan {\&} Claypool Publishers},
  series    = {Synthesis Lectures on Computer Architecture},
  year      = {2010},
}

@article{hammondhytm,
 author = {Hammond, Lance and Wong, Vicky and Chen, Mike and Carlstrom, Brian D. and Davis, John D. and Hertzberg, Ben and Prabhu, Manohar K. and Wijaya, Honggo and Kozyrakis, Christos and Olukotun, Kunle},
 title = {Transactional Memory Coherence and Consistency},
 journal = {SIGARCH Comput. Archit. News},
 issue_date = {March 2004},
 volume = {32},
 number = {2},
 month = mar,
 year = {2004},
 issn = {0163-5964},
 pages = {102--},
 url = {http://doi.acm.org/10.1145/1028176.1006711},
 doi = {10.1145/1028176.1006711},
 acmid = {1006711},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{kumarhytm,
 author = {Kumar, Sanjeev and Chu, Michael and Hughes, Christopher J. and Kundu, Partha and Nguyen, Anthony},
 title = {Hybrid Transactional Memory},
 booktitle = {Proceedings of the Eleventh ACM SIGPLAN Symp. on Principles and Practice of Parallel Programming},
 series = {PPoPP '06},
 year = {2006},
 isbn = {1-59593-189-9},
 location = {New York, New York, USA},
 pages = {209--220},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/1122971.1123003},
 doi = {10.1145/1122971.1123003},
 acmid = {1123003},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {architecture support, nonblocking, transactional memory, transactions},
} 

@article{damronhytm,
 author = {Damron, Peter and Fedorova, Alexandra and Lev, Yossi and Luchangco, Victor and Moir, Mark and Nussbaum, Daniel},
 title = {Hybrid Transactional Memory},
 journal = {SIGPLAN Not.},
 issue_date = {November 2006},
 volume = {41},
 number = {11},
 month = oct,
 year = {2006},
 issn = {0362-1340},
 pages = {336--346},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/1168918.1168900},
 doi = {10.1145/1168918.1168900},
 acmid = {1168900},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transactional memory},
} 

@inproceedings{unboundedhtm1,
 author = {Ananian, C. Scott and Asanovic, Krste and Kuszmaul, Bradley C. and Leiserson, Charles E. and Lie, Sean},
 title = {Unbounded Transactional Memory},
 booktitle = {Proceedings of the 11th International Symp. on High-Performance Computer Architecture},
 series = {HPCA '05},
 year = {2005},
 isbn = {0-7695-2275-0},
 pages = {316--327},
 numpages = {12},
 url = {http://dx.doi.org/10.1109/HPCA.2005.41},
 doi = {10.1109/HPCA.2005.41},
 acmid = {1043430},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 

@InProceedings{HM93,
	author = "Maurice Herlihy and J. Eliot B. Moss",
	title = "Transactional memory: architectural support for lock-free data structures",
	booktitle = "ISCA",
	year = "1993",
	pages = "289--300"
}

@article{AttiyaCH18,
  author    = {Hagit Attiya and
               Armando Casta{\~{n}}eda and
               Danny Hendler},
  title     = {Nontrivial and universal helping for wait-free queues and stacks},
  journal   = {J. Parallel Distrib. Comput.},
  volume    = {121},
  pages     = {1--14},
  year      = {2018},
  url       = {https://doi.org/10.1016/j.jpdc.2018.06.004},
  doi       = {10.1016/j.jpdc.2018.06.004},
  timestamp = {Fri, 02 Nov 2018 15:39:06 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/jpdc/AttiyaCH18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{golab15,
  author    = {Ryan Berryhill and
               Wojciech M. Golab and
               Mahesh Tripunitara},
  title     = {Robust Shared Objects for Non-Volatile Main Memory},
  booktitle = {19th International Conference on Principles of Distributed Systems,
               {OPODIS} 2015, December 14-17, 2015, Rennes, France},
  pages     = {20:1--20:17},
  year      = {2015},
  
  url       = {https://doi.org/10.4230/LIPIcs.OPODIS.2015.20},
  doi       = {10.4230/LIPIcs.OPODIS.2015.20},
  timestamp = {Thu, 02 May 2019 17:40:16 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/opodis/BerryhillGT15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{ST95,
	author = "NirShavit and Dan Touitou",
	title = "Software transactional memory",
	booktitle = "PODC",
	year = "1995",
	pages = "204--213"
}

@inproceedings{Att10,
  author    = {Hagit Attiya},
  title     = {The inherent complexity of transactional memory and what
               to do about it},
  booktitle = {PODC},
  year      = {2010},
  pages     = {1-5}
}

@inproceedings{HHL+05,
 author = {Heller, Steve and Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer, William N. and Shavit, Nir},
 title = {A lazy concurrent list-based set algorithm},
 booktitle = {OPODIS},
 year = {2006},
 pages = {3--16}, 
} 

@inproceedings{MS13,
  title={Reduced hardware transactions: a new approach to hybrid transactional memory},
  author={Matveev, Alexander and Shavit, Nir},
  booktitle={Proceedings of the 25th ACM Symp. on Parallelism in algorithms and architectures},
  pages={11--22},
  year={2013},
  organization={ACM}
}

@inproceedings{hynorecriegel,
  title={Optimizing hybrid transactional memory: The importance of nonspeculative operations},
  author={Riegel, Torvald and Marlier, Patrick and Nowack, Martin and Felber, Pascal and Fetzer, Christof},
  booktitle={Proceedings of the 23rd ACM Symp. on Parallelism in Algorithms and Architectures},
  pages={53--64},
  year={2011},
  organization={ACM}
}

@inproceedings{CTGM14,
  title={Improved single global lock
fallback for best-effort hardware transactional memory.},
  author={Calciu, Irina and Shpeisman, Tatiana and Pokam, Gilles and Herlihy, Maurice},
  booktitle={Transact 2014 Workshop},
  year={2014},
  organization={ACM}
}

@inproceedings{ALM14,
  title={Software-improved hardware lock elision.},
  author={Afek, Yehuda and Levy, Amir and Morrison, Adam},
  booktitle={PODC},
  year={2014},
  organization={ACM}
}

@inproceedings{Harris01,
  author    = {Timothy L. Harris},
  editor    = {Jennifer L. Welch},
  title     = {A Pragmatic Implementation of Non-blocking Linked-Lists},
  booktitle = {Distributed Computing, 15th International Conference, {DISC} 2001,
               Lisbon, Portugal, October 3-5, 2001, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {2180},
  pages     = {300--314},
  publisher = {Springer},
  year      = {2001},
  url       = {https://doi.org/10.1007/3-540-45414-4\_21},
  doi       = {10.1007/3-540-45414-4\_21},
  timestamp = {Tue, 14 May 2019 10:00:54 +0200},
  biburl    = {https://dblp.org/rec/conf/wdag/Harris01.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Herlihy91,
  author    = {Maurice Herlihy},
  title     = {Wait-Free Synchronization},
  journal   = {{ACM} Trans. Program. Lang. Syst.},
  volume    = {13},
  number    = {1},
  pages     = {124--149},
  year      = {1991},
  url       = {https://doi.org/10.1145/114005.102808},
  doi       = {10.1145/114005.102808},
  timestamp = {Wed, 14 Nov 2018 10:30:40 +0100},
  biburl    = {https://dblp.org/rec/journals/toplas/Herlihy91.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{flat-combining,
  author    = {Danny Hendler and
               Itai Incze and
               Nir Shavit and
               Moran Tzafrir},
  editor    = {Friedhelm Meyer auf der Heide and
               Cynthia A. Phillips},
  title     = {Flat combining and the synchronization-parallelism tradeoff},
  booktitle = {{SPAA} 2010: Proceedings of the 22nd Annual {ACM} Symp. on Parallelism
               in Algorithms and Architectures, Thira, Santorini, Greece, June 13-15,
               2010},
  pages     = {355--364},
  publisher = {{ACM}},
  year      = {2010},
  url       = {https://doi.org/10.1145/1810479.1810540},
  doi       = {10.1145/1810479.1810540},
  timestamp = {Wed, 21 Nov 2018 11:15:55 +0100},
  biburl    = {https://dblp.org/rec/conf/spaa/HendlerIST10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{zuriel2019efficient,
  title={Efficient lock-free durable sets},
  author={Zuriel, Yoav and Friedman, Michal and Sheffi, Gali and Cohen, Nachshon and Petrank, Erez},
  journal={Proceedings of the ACM on Programming Languages},
  volume={3},
  number={OOPSLA},
  pages={1--26},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@inproceedings{david2018log,
  title={Log-free concurrent data structures},
  author={David, Tudor and Dragojevic, Aleksandar and Guerraoui, Rachid and Zablotchi, Igor},
  booktitle={2018 $\{$USENIX$\}$ Annual Technical Conference ($\{$USENIX$\}$$\{$ATC$\}$ 18)},
  pages={373--386},
  year={2018}
}

@article{herlihy1990linearizability,
  title={Linearizability: A correctness condition for concurrent objects},
  author={Herlihy, Maurice P and Wing, Jeannette M},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={12},
  number={3},
  pages={463--492},
  year={1990},
  publisher={ACM New York, NY, USA}
}

@misc{intel_2016, 
    title={Intel® 64 and IA-32 Architectures Optimization Reference Manual},
    journal={Intel® 64 and IA-32 Architectures Optimization Reference Manual},
    publisher={Intel}, 
    author={Intel}, 
    year={2016}, 
    month={Jun}
}

@inproceedings{fomitchev2004lock,
  title={Lock-free linked lists and skip lists},
  author={Fomitchev, Mikhail and Ruppert, Eric},
  booktitle={Proceedings of the twenty-third annual ACM Symp. on Principles of distributed computing},
  pages={50--59},
  year={2004}
}

@inproceedings{cohen2018inherent,
  title={The inherent cost of remembering consistently},
  author={Cohen, Nachshon and Guerraoui, Rachid and Zablotchi, Igor},
  booktitle={Proceedings of the 30th on Symp. on Parallelism in Algorithms and Architectures},
  pages={259--269},
  year={2018}
}

@article{attiya2011laws,
  title={Laws of order: expensive synchronization in concurrent algorithms cannot be eliminated},
  author={Attiya, Hagit and Guerraoui, Rachid and Hendler, Danny and Kuznetsov, Petr and Michael, Maged M and Vechev, Martin},
  journal={ACM SIGPLAN Notices},
  volume={46},
  number={1},
  pages={487--498},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@inproceedings{izraelevitz2016linearizability,
  title={Linearizability of persistent memory objects under a full-system-crash failure model},
  author={Izraelevitz, Joseph and Mendes, Hammurabi and Scott, Michael L},
  booktitle={International Symp. on Distributed Computing},
  pages={313--327},
  year={2016},
  organization={Springer}
}

@article{cohen2017efficient,
  title={Efficient logging in non-volatile memory by exploiting coherency protocols},
  author={Cohen, Nachshon and Friedman, Michal and Larus, James R},
  journal={Proceedings of the ACM on Programming Languages},
  volume={1},
  number={OOPSLA},
  pages={1--24},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@article{izraelevitz2019basic,
  title={Basic performance measurements of the intel optane DC persistent memory module},
  author={Izraelevitz, Joseph and Yang, Jian and Zhang, Lu and Kim, Juno and Liu, Xiao and Memaripour, Amirsaman and Soh, Yun Joon and Wang, Zixuan and Xu, Yi and Dulloor, Subramanya R and Zhao, Jishen and  Swanson, Steven},
  journal={arXiv preprint arXiv:1903.05714},
  year={2019}
}

@article{david2015asynchronized,
  title={Asynchronized concurrency: The secret to scaling concurrent search data structures},
  author={David, Tudor and Guerraoui, Rachid and Trigonakis, Vasileios},
  journal={ACM SIGARCH Computer Architecture News},
  volume={43},
  number={1},
  pages={631--644},
  year={2015},
  publisher={ACM New York, NY, USA}
}


@inproceedings{friedman2020nvtraverse,
  title={Nvtraverse: in nvram data structures, the destination is more important than the journey},
  author={Friedman, Michal and Ben-David, Naama and Wei, Yuanhao and Blelloch, Guy E and Petrank, Erez},
  booktitle={Proceedings of the 41st ACM SIGPLAN Conf. on Programming Language Design and Impl.},
  pages={377--392},
  year={2020}
}

@inproceedings{friedman2021mirror,
  title={Mirror: making lock-free data structures persistent},
  author={Friedman, Michal and Petrank, Erez and Ramalhete, Pedro},
  booktitle={Proceedings of the 42nd ACM SIGPLAN International Conference on Programming Language Design and Implementation},
  pages={1218--1232},
  year={2021}
}

@inproceedings{peng2019system,
  title={System evaluation of the intel optane byte-addressable nvm},
  author={Peng, Ivy B and Gokhale, Maya B and Green, Eric W},
  booktitle={Proceedings of the International Symp. on Memory Systems},
  pages={304--315},
  year={2019}
}

@book{AW04,
    Author={ Hagit Attiya and Jennifer Welch},
    Title= {Distributed Computing. Fundamentals, Simulations, and Advanced Topics.},
    Publisher={John Wiley \& Sons},
    Year= "2004",
}

@inproceedings{wang2018easy,
  title={Easy lock-free indexing in non-volatile memory},
  author={Wang, Tianzheng and Levandoski, Justin and Larson, Per-Ake},
  booktitle={2018 IEEE 34th International Conference on Data Engineering (ICDE)},
  pages={461--472},
  year={2018},
  organization={IEEE}
}

@misc{optane,
  author={Intel Corporation},
  title={Intel Optane Persistent Memory},
  year={2017},
  howpublished = {Available at: \url{www.intel.com/content/www/us/en/architecture-and-technology/optane-dc-persistent-memory}},
  note = {[last accessed: Jan 25, 2022]}
}


@misc{libvmmalloc,
  author={Intel Corporation},
  title={PMDK: Libvmmalloc},
  year={2020},
  howpublished = {Available at: \url{pmem.io/pmdk/manpages/linux/v1.3/libvmmalloc.3}},
  note = {[last accessed: Jan 25, 2022]}
}

@inproceedings{correia2020persistent,
  title={Persistent memory and the rise of universal constructions},
  author={Correia, Andreia and Felber, Pascal and Ramalhete, Pedro},
  booktitle={Proceedings of the Fifteenth European Conference on Computer Systems},
  pages={1--15},
  year={2020}
}

@inproceedings{kolli2016high,
  title={High-performance transactions for persistent memories},
  author={Kolli, Aasheesh and Pelley, Steven and Saidi, Ali and Chen, Peter M and Wenisch, Thomas F},
  booktitle={Proceedings of the Twenty-First International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={399--411},
  year={2016}
}


@article{avni2016persistent,
  title={Persistent hybrid transactional memory for databases},
  author={Avni, Hillel and Brown, Trevor},
  journal={Proceedings of the VLDB Endowment},
  volume={10},
  number={4},
  pages={409--420},
  year={2016},
  publisher={VLDB Endowment}
}

@inproceedings{avni2015hardware,
  title={Hardware transactions in nonvolatile memory},
  author={Avni, Hillel and Levy, Eliezer and Mendelson, Avi},
  booktitle={International Symp. on Distributed Computing},
  pages={617--630},
  year={2015},
  organization={Springer}
}

@article{volos2011mnemosyne,
  title={Mnemosyne: Lightweight persistent memory},
  author={Volos, Haris and Tack, Andres Jaan and Swift, Michael M},
  journal={ACM SIGARCH Computer Architecture News},
  volume={39},
  number={1},
  pages={91--104},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{coburn2011nv,
  title={NV-Heaps: Making persistent objects fast and safe with next-generation, non-volatile memories},
  author={Coburn, Joel and Caulfield, Adrian M and Akel, Ameen and Grupp, Laura M and Gupta, Rajesh K and Jhala, Ranjit and Swanson, Steven},
  journal={ACM SIGARCH Computer Architecture News},
  volume={39},
  number={1},
  pages={105--118},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{wei2021flit,
  title={FliT: A Library for Simple and Efficient Persistent Algorithms},
  author={Wei, Yuanhao and Ben-David, Naama and Friedman, Michal and Blelloch, Guy E and Petrank, Erez},
  journal={arXiv preprint arXiv:2108.04202},
  year={2021}
}

@inproceedings{censor2015help,
  title={Help!},
  author={Censor-Hillel, Keren and Petrank, Erez and Timnat, Shahar},
  booktitle={Proceedings of the 2015 ACM Symp. on Principles of Distributed Computing},
  pages={241--250},
  year={2015}
}

@article{ben2020separation,
  title={Separation and Equivalence results for the Crash-stop and Crash-recovery Shared Memory Models},
  author={Ben-Baruch, Ohad and Ravi, Srivatsan},
  journal={arXiv preprint arXiv:2012.03692},
  year={2020}
}

@article{jayanti2000time,
  title={Time and space lower bounds for nonblocking implementations},
  author={Jayanti, Prasad and Tan, King and Toueg, Sam},
  journal={SIAM Journal on Computing},
  volume={30},
  number={2},
  pages={438--456},
  year={2000},
  publisher={SIAM}
}

@inproceedings{ramalhete2021efficient,
  title={Efficient algorithms for persistent transactional memory},
  author={Ramalhete, Pedro and Correia, Andreia and Felber, Pascal},
  booktitle={Proceedings of the 26th ACM SIGPLAN Symp. on Principles and Practice of Parallel Programming},
  pages={1--15},
  year={2021}
}
